Optimal Sequential Recommendations: Exploiting User and Item Structure

We consider an online model for recommendation systems, with each user being recommended an item at each time-step and providing 'like' or 'dislike' feedback. A latent variable model specifies the user preferences: both users and items are clustered into types. The model captures structure in both the item and user spaces, as used by item-item and user-user collaborative filtering algorithms. We study the situation in which the type preference matrix has i.i.d. entries. Our main contribution is an algorithm that simultaneously uses both item and user structures, proved to be near-optimal via corresponding information-theoretic lower bounds. In particular, our analysis highlights the sub-optimality of using only one of item or user structure (as is done in most collaborative filtering algorithms).

==> BADlowerBD.tex <==
\subsection{Lower bounding the number of bad recommendations}
\label{sec:JL-BAD-lowerBD}

Lemma~\ref{l:jl-bad-lower} lower bounds the expected number of ``bad'' recommendations as defined in~\eqref{eq:jl-def-bad}  for any recommendation algorithm. This section covers sthe statement of this lemma and its proof. 
Theorem~\ref{t:joint-L} is a direct consequence of Lemmas~\ref{l:jl-reg-lower} and~\ref{l:jl-bad-lower}.
  \MK{Update the previous paragraph and the next lemma and maybe the next paragraph}
\begin{lemma}\label{l:jl-bad-lower}
The expected number of bad recommendations defined in Equation~\eqref{eq:jl-def-bad} satisfies the following lower bound:
\begin{align*}
\Exp{\bad(T)} \geq \frac{1}{8} M(T)
+ \frac{T}{8}  \min\big\{\thrjil, \frac{N}{\Lambda }\big\}
\end{align*}
where $M(T)$ is defined in Equations~\eqref{eq:MdefLBRegime1} and~\eqref{eq:MdefLBRegime2}.
 The variable $\Lambda$ is defined in Equation~\eqref{eq:ThetaqIdef}. The parameters $\thrjul$ and $\thrjil$ are defined in Equations~\eqref{eq:jl-thru} and~\eqref{eq:jl-thri}.
\end{lemma}
%This lemma is proved in Section~\ref{sec:JL-BAD-lowerBD}. 
%Theorem~\ref{t:joint-L} is a direct consequence of Lemmas~\ref{l:jl-reg-lower} and~\ref{l:jl-bad-lower}.  

To prepare for the proof of this lemma, we introduce some new notations each of which summarizes an important property of the performance of algorithm such as total number of items seen by the algorithm by the end of time $T$ or number of users which have rated more than $\thrjul$ item types by the end of time $T$ (Definitions~\ref{def:jl-itemsF},~\ref{def:jl-usersH},~\ref{def:jl-gamma-U}, and~\ref{def:jl-minUser}). 
Note that since these quantities depend on the algorithm description and the preference model, they can take unknown (possibly random) values. 
We lower bound the number of bad recommendations as various functions of these parameters in Lemmas~\ref{l:BoundBad1},~\ref{l:BoundBad2},~\ref{l:BoundBad3}, and~\ref{l:BoundBad4}. 
Next,
looking into the preference model introduced in Section~\ref{sec:model} and some  concentration bounds relates these parameters to each other (Lemmas~\ref{l:BoundminUserSize} and~\ref{l:JL-bdGammaStarP}). 
Putting it together, in Section~\ref{sec:LBputtingitall}, we show that for any realization of these parameters with these relations, the number of bad recommendations is lower bounded. 

\subsubsection{Step 1}
\label{sec:LBStep1}
Heuristically, when $\Xi^T\in \rgl_{\thrjil,\eta}$, to partition a group of items, any algorithm needs to make $\thrjil$ explorative (bad) recommendations per item to compare any item with  all item types. 
Section~\ref{ss:comparison} presents this heuristic in the context of the algorithm design and the number of comparisons needed to partition items. \MK{The previous sentence is wrong. } Section~\ref{sec:LBthrParam} uses notion of row regularity to lower bound the number of explorative recommendations per item for any algorithm. 
In this section, we bound the number of bad recommendations in terms of number of explorative recommendations made in order to learn the item types.

Recall that $c_i^t$ (Definition~\ref{def:jl-cit}) is the number of user types which have rated item $i$ by the end of time $t-1$.

\begin{definition}\label{def:jl-itemsF} 
Let $\Fc^{(t)} = \{i: c_i^{t+1} \geq \thrjil\}$  be the set of items that have been rated by at least $\thrjil$ user types by the end of time $t$ and  
\begin{equation}
\label{eq:jl-fT}
f^{(t)} := |\Fc^{(t)}| =\sum_{i\in\mathbb{N}} \ident[c_{i}^{t+1}\geq \thrjil]\,.
\end{equation}
%
 Let $\Gc^{(t)} =  \{i: 0<c_i^{t+1} < \thrjil\}$ be the set items that have been rated by at least one and fewer than $\thrjil$ user types by the end of time $t$. Let $g^{(t)} $ be the number of times any item in $\Gc^{(t)}$  is recommended to a user type for the first time. 
\begin{equation}
\label{eq:jl-gT}
g^{(t)} := 
 \sum_{i\in\mathbb{N}} c_{i}^{t+1} \,\,\ident[0 < c_{i}^{t+1}< \thrjil].
\end{equation}
Let $\Nc^{(t)} = \Fc^{(t)} \cup \Gc^{(t)}$ be the set of all items that have been recommended to at least one user by the end of time $t$ and
\begin{equation}
\label{eq:jl-nT}
n^{(t)} := |\Nc^{(t)}|=
 \sum_{i\in\mathbb{N}} \ident[0 < c_{i}^{t+1}]\,.
\end{equation}
\end{definition}

Any item in $i\in\Fc^{(T)}$ (Definition \ref{def:jl-itemsF}) is recommended to at least $\thrjil$ user types by time $T$. So, for any $i\in\Fc^{(T)}$, there are $\thrjil$ recommendations in which $i$ is recommended to a user type for the first time while it has been rated by fewer than $\thrjil$ user types previously:
\begin{align}
\sum_{\substack{t\in [T] \\ u\in [N]} } \ident[c_i^t <\thrjil,  (\BBjul{u}{i}{t})^c, a_{u,t}=i]  = \thrjil, \quad \text{ for } i\in\Fc^{(T)}\,.
\label{eq:jl-boundcFc}
\end{align}
Any $i\in \Gc^{(T)}$ (Definition \ref{def:jl-itemsF}) is recommended to at least one user type, so for these items:
\begin{align}
\sum_{\substack{t\in [T] \\ u\in [N]} } \ident[c_i^t <\thrjil,  (\BBjul{u}{i}{t})^c, a_{u,t}=i]  
=
\sum_{\substack{t\in [T] \\ u\in [N]} } \ident[ (\BBjul{u}{i}{t})^c, a_{u,t}=i]  
= c_{i}^{T+1}, \quad \text{ for } i\in\Gc^{(T)}\,,
\label{eq:jl-boundcGc}
\end{align}
where the first equality holds since for any $ i\in\Gc^{(T)}$ and $t\leq T$ we have $c_i^t <\thrjil$.


The following claim bounds the number of bad recommendations up to time $T$ in terms of $f^{(T)}$ and $g^{(T)}$.
\begin{lemma}
\label{l:BoundBad1}
The  number of bad recommendations $\bad(T)$,  defined in Equation~\eqref{eq:jl-def-bad} satisfies 
\begin{equation}\label{eq:jl-bad-gT-fT}
\bad(T)\geq f^{(T)} \thrjil + g^{(T)} \,.
\end{equation}
which gives
\begin{equation}\label{eq:jl-bad-nT}
\bad(T)\geq n^{(T)} \,.
\end{equation}
\end{lemma}

\begin{proof}
Using the definition of bad recommendations in~\eqref{eq:jl-def-bad}:
\begin{align*}
\bad(T)
&
{\geq}
 \sum_{t=1}^T \sum_{u=1}^N\Bsf{1}(u,t) +\Bsf{2}(u,t)
 \\ 
 &
\overset{(a)}{\geq}
  \sum_{t=1}^T \sum_{u=1}^N\sum_{i\in\Fc_T \cup \Gc_T} \ident[c_i^t <\thrjil,  (\BBjul{u}{i}{t})^c, a_{u,t}=i] 
% \\&
\overset{(b)}{\geq}
 f^{(T)} \thrjil + g^{(T)} \geq n^{(T)} \,,
\end{align*}
where (a) uses the definitions in~\eqref{eq:jl-def-B1} and~\eqref{eq:jl-def-B2} and the fact that the recommended items by time $T$ are either in $\Fc^{(T)}$ or $\Gc^{(T)}$.
(b) uses~\eqref{eq:jl-boundcFc} and~\eqref{eq:jl-boundcGc} and definition of $f^{(T)}$ and $g^{(T)}$ in~\eqref{eq:jl-fT} and~\eqref{eq:jl-gT}. Note that for $i\in \Gc^{(T)}$, we have $c_i^{T+1}\geq 1$, hence $n^{(T)}= |\Fc^{(T)}|+|\Gc^{(T)}|\leq f^{(T)}+g^{(T)}$ which gives the last inequality.
\end{proof}

%%%%%%%%

\subsubsection{Step 2}
\label{sec:LBStep2}
Similar to Section~\ref{sec:LBStep1}, heuristically speaking, to partition a group of users, any algorithm needs to make at least $\thrjul$ explorative (bad) recommendations per user to compare any user with all the user types. 
In this section, we lower bound the number of bad recommendations in terms of number of explorative recommendations made to learn the user types.
Recall that $d_u^t$ (Definition~\ref{def:jl-dut}) is the number of distinct item types which have been recommended to user $u$ by the end of time $t-1$.


\begin{definition}\label{def:jl-usersH}
Let $\Wc_t\subseteq [N]$ be the set of users that have rated at least $\thrjul$ distinct item types by the end of time $t$. Let 
\begin{equation}\label{eq:jl-wT}
w_t:= \frac{1}{N}|\Wc_t|=\frac{1}{N}\sum_{u\in[N]}\ident[d_u^{t+1}\geq \thrjul]\,,
\end{equation} 
be the fraction of users in $\Wc_t$.
\end{definition} 

Note that since $d_u^t$ is nondecreasing in $t$, for any $u\notin\Wc_T$, we have $d_u^t<\thrjul$ for all $t\leq T+1$. 

%%%%%%%%%%%%%%%
\begin{lemma}
\label{l:BoundBad2}
The  number of bad recommendations $\bad(T)$,  defined in Equation~\eqref{eq:jl-def-bad} satisfies 
\begin{equation}\label{eq:jl-wT-N-rU}
\bad(T)\geq 
w_T N \thrjul
 \,.
\end{equation}

\end{lemma}
%
\begin{proof}
Any user in $u\in\Wc_T$ (Definition \ref{def:jl-usersH}) is recommended at least $\thrjul$ item types by time $T$. So, for any $u\in\Wc_T$, there are $\thrjul$ recommendations in which $u$ is recommended an item type for the first time while it has been rated fewer than $\thrjul$ item types previously:
\begin{align}
\sum_{\substack{t\in [T] } }\sum_{i} \ident[d_u^t <\thrjul,  (\BBjil{u}{i}{t})^c, a_{u,t}=i]  = \thrjul, \quad \text{ for } u\in\Wc_T\,.
\label{eq:jl-bounddWc}
\end{align}
Using the definition of bad recommendations in~\eqref{eq:jl-def-bad}:
\begin{align}
\bad(T)
&{\geq}
 \sum_{t=1}^T \sum_{u\in [N]}\Bsf{1}(u,t) +\Bsf{3}(u,t)
\notag\\ &
\overset{(a)}{\geq}
  \sum_{t=1}^T \sum_{u\in \Wc_T}\sum_{i} \ident[d_u^t <\thrjul,  (\BBjil{u}{i}{t})^c, a_{u,t}=i] 
\label{eq:jl-B1-B3}
\overset{(b)}{\geq}
w_T N \thrjul
\,.
\end{align}
where (a) uses the definitions in~\eqref{eq:jl-def-B1} and~\eqref{eq:jl-def-B3}.% and the fact that the users by time $T$ are either in $\Fc_T$ or $\Gc_T$.
(b) uses~\eqref{eq:jl-bounddWc}
% and~\eqref{eq:jl-boundcWcCom} 
and definition of $w_T$ in~\eqref{eq:jl-wT}.
\end{proof}
%%%%%%%%%%%%%%%
\subsubsection{Step 3}
Heuristically speaking, if the algorithm does not know the type of a user, any time this user is recommended a new item type, the outcome is uncertain. 
As a result, the number of bad recommendations is lower bounded by the number of times  a new item type is recommended to any user  with unknown user type. 
According to Definition~\ref{def:jl-usersH}, the algorithm cannot learn the type of  users $u\notin\Wc_T$ by the end of time $T$. To bound the number of item types recommended to these users for the first time, we define the following notation:

\begin{definition}\label{def:jl-gamma-U}
 Let $\Gamma_{u}^T$ be the set of item types that are rated by user $u$ by time $T$.
\[\Gamma_u^T=\bigg\{\ti\in[\qi]: \sum_{t\in[T], i:\tau_I(i)=\ti}\ident[a_{u,t}=i]\neq 0\bigg\}\]
Let $\gamma_u^T = |\Gamma_u^T|$ and  $\gamma_*^T := \min_{u} \gamma_u^T$.
\end{definition}

Looking at Definition~\ref{def:jl-dut}, we see that $\gamma_u^{t} = d_{u}^{t+1}$.
Note that for according to the definition of $\Wc_T$ (Definition~\ref{def:jl-usersH})
\begin{equation} \label{eq:jl-gamu -notin-W} 
u\in \Wc_T\text{ if and only if } \gamma_u^T \geq \thrjul\,.
\end{equation}

\begin{lemma}
\label{l:BoundBad3}
The  number of bad recommendations $\bad(T)$,  defined in Equation~\eqref{eq:jl-def-bad} satisfies 
\begin{align*}
\bad(T)
\geq
(1-w_T) N\gamma_*^T\,.
\end{align*}
\end{lemma}

\begin{proof}
For any $u\notin \Wc_T$, using Definition~\ref{def:jl-usersH}, $d_{u}^t < \thrjul$ for all $t\leq T$. 
Hence, as shown in Equation~\eqref{eq:jl-B1-B3}, for any $u\notin \Wc_T$
\begin{align*}
\Bsf{1}(u,t) +\Bsf{3}(u,t)
& \geq 
\sum_{i\in\mathbb{N}}\ident[ d_{u}^t < \thrjul, (\BBjil{u}{i}{t})^c, a_{u,t}=i]
\\
&\geq 
\sum_{i\in\mathbb{N}}\ident[(\BBjil{u}{i}{t})^c, a_{u,t}=i]
\end{align*}
Using Definition~\ref{def:jl-gamma-U},  user $u$ rates an item from a new item type (which has not been rated by $u$ before) for the first time $\gamma_u^T$ times by time $T$. So for 
any $u \notin \Wc_T$ we have 
\begin{align*}\label{eq:jl-B1-B3-gammaOneU}
\sum_{t=1}^T\Bsf{1}(u,t) +\Bsf{3}(u,t) \geq 
\gamma_u^T \geq \gamma_*^T\,.
\end{align*}
Taking the summation on $u\in[N]\setminus \Wc_T$ gives
\begin{equation*}
%\label{eq:jl-B1-B3-gammaOneU}
\bad(T) \geq 
\sum_{u\in [N]\setminus \Wc_T }\sum_{t=1}^T\Bsf{1}(u,t) +\Bsf{3}(u,t) 
\geq
(1-w_T)N\gamma_*^T\,.
%\qedhere
\end{equation*}
\end{proof}

%%%%%%%%%%
%%%%%%%%%%
\subsubsection{Step~4}
Heuristically speaking, any time a user type is recommended a new item type, the outcome of the recommendation is uncertain. In this section, we look at the group of users for which their type might be known by the end of time $T$ and bound the number of bad recommendations by the number of new item types recommended to each of these user types. To do so, we use the following definition.  
\begin{definition}\label{def:jl-minUser}
 Let $\minUser$ be the maximum number of users with a user type:
 \[\minUser = \max_{\tu\in[\qu]} \Big| \big\{u\in [N]: \tau_U(u)=\tu \big\} \Big|\,.\]
\end{definition}
Using this definition, we can  lower bound the number of user types with at least one user among all the users in $[N]$ by $\frac{N}{\minUser}$. 
%\begin{definition}\label{def:jl-NonEmptyUser}
% Let $\NonEmptyUser$ be the number of  user types with at least one user present in the system:
% \[
% \NonEmptyUser
%  := \big| \{
%  \tu\in [\qu] :\text{ there exists } 
%  u\in [N] \text{ such that } \tau_U(u)=\tu  
%  \}\big|\,.\]
%\end{definition}

\begin{lemma}
\label{l:BoundBad4}
The  number of bad recommendations is lower bounded as 
$
\bad(T)
\geq
\frac{N}{\minUser}\gamma_*^T\,.
$
\end{lemma}

%Proof of this lemma appears in Appendix~\ref{sec:Proofl:BoundBad4}.
\begin{proof}
Note that if no user from user type $\tau_U(u)$ has rated any item from item type $\tau_I(i)$, then obviously no user from user type $\tau_U(u)$ has rated item $i$: $\ident[(\BBjul{u}{i}{t})^c]\geq \ident[(\BBjjl{u}{i}{t})^c] $; and  no item with item type $\tau_I(i)$ has been rated by user $u$: $\ident[(\BBjil{u}{i}{t})^c]\geq \ident[(\BBjjl{u}{i}{t})^c] $. Hence,
\begin{align*}
\Bsf{1}(u,t)+\Bsf{2}(u,t)+\Bsf{3}(u,t) +\Bsf{4}(u,t)
 & \geq \ident[ (\BBjjl{u}{a_{u,t}}{t})^c]\,.
\end{align*}
So the number of bad recommendations is lower bounded as follows:
\begin{align*}
\bad(T)
&\geq 
\sum_{u\in [N]}
\sum_{t=1}^T\ident[ (\BBjjl{u}{a_{u,t}}{t})^c]
\geq
\frac{N}{\minUser}
    \gamma_*^T\,.
\end{align*}
The last inequality uses the definition of parameters $\gamma_*^T$ and $\minUser$.
According to  Definition~\ref{def:jl-minUser}, the number of user types with at least one user present among the $N$ users in the system is lower bounded by $\frac{N}{\minUser}$.

Any user $u$ is recommended an item with a new item type for the first time $\gamma_u^T$ times by time $T$. Hence, any user type $\tu$ is recommended an item with a new item type for the first time at least $\gamma_*^T= \min_u \gamma_u^T$ times by time $T$.
So the number of times an item type is recommended to a user type for the first time is lower bounded by $\frac{N}{\minUser}\gamma_*^T$.
\end{proof}

%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
\subsubsection{Step~5}
This step focuses on the fact that the total number of recommendations made by the algorithm by the end of time $T$ is $TN$ (one recommendation per user per unit of time). 
Also, the good recommendations (the ones which are not bad),  either include recommending items (in $\Fc_T$) that have been recommended to at least $\thrjil$ user types before, or recommending items ($i\in\Gc_T$) to users from types which have been previously  recommended item $i$ before. We give the details of this argument next.


\begin{lemma}
\label{l:BoundBad5}
The  number of bad recommendations $\bad(T)$,  defined in Equation~\eqref{eq:jl-def-bad} satisfies 
\[\bad(T) \geq TN- \Big[f_T (N-\thrjil) + g_T (\minUser-1)\Big]\,. \]
\end{lemma}


We bound the total number of recommendations made by the algorithm as follows:

\begin{align*}
TN  
\overset{(a)}= &
\sum_{u=1}^N
\sum_{t=1}^T
\sum_{i\in\Nc_T}
\ident[a_{u,t}=i]
\\
\overset{(b)}= &
\sum_{i\in\Nc_T}
\sum_{u=1}^N
\sum_{t=1}^T
\ident[a_{u,t}=i, c_i^t<\thrjil, (\BBjul{u}{i}{t})^c]
\\
&+
\sum_{i\in\Fc_T}
\sum_{u=1}^N
\sum_{t=1}^T
\ident[a_{u,t}=i] - \ident[a_{u,t}=i, c_i^t<\thrjil, (\BBjul{u}{i}{t})^c] 
\\
&+
\sum_{i\in\Gc_T}
\sum_{u=1}^N
\sum_{t=1}^T
\ident[a_{u,t}=i, c_i^t<\thrjil, \BBjul{u}{i}{t}]
\\
\overset{(c)}\leq &
\sum_{u=1}^N
\sum_{t=1}^T
[\Bsf{1}(u,t)+\Bsf{2}(u,t)]
+
\sum_{i\in\Fc_T}
(N-\thrjil)
+
\sum_{i\in \Gc_T}
c_i^{T+1}
\minUser
\\
 \overset{(d)}\leq&
 \bad(T)
+ 
\sum_{i\in \Fc_T}
(N-\thrjil)
+
g_T
(\minUser-1)
\,.
\end{align*}
In the above display equality (a) holds since according to the Definition~\ref{def:jl-itemsF}, by time $T$ items in $\Nc_T=\Fc_T\cup\Gc_T$ are recommended by the algorithm. In (b) the recommendations made from $\Fc_T$ and $\Gc_T$ are decomposed separately and for all items $i\in\Gc_T$ and $t\leq T$, we have $1\leq c_i^t<\thrjil$. \MK{Double check this one more time to make sure the onequality is strict}

According to~\eqref{eq:jl-def-B1} and~\eqref{eq:jl-def-B2}, 
$\sum_{i\in\Nc_T}
\ident[a_{u,t}=i, c_i^t<\thrjil, (\BBjul{u}{i}{t})^c] \leq \Bsf{1}(u,t)+\Bsf{2}(u,t)$. 
This gives the first term in (c). 
Each item can be recommended at most once to each user, hence $\sum_{u=1}^N
\sum_{t=1}^T
\ident[a_{u,t}=i]\leq N$ for each item $i\in\Fc_T$. This inequality and ~\eqref{eq:jl-boundcFc} give 
\[
\sum_{u=1}^N
\sum_{t=1}^T
\ident[a_{u,t}=i] - \ident[a_{u,t}=i, c_i^t<\thrjil, (\BBjul{u}{i}{t})^c] 
\leq N-\thrjil\]
 for any $i\in\Fc_T$.

Any item $i$ is recommended to $c_i^{T+1}$ user types by the end of time $T$. There are at most $\minUser$ users of any given user type present in the system. So the total number of times an item $i$ is recommended to a user $u$ such that $\BBjul{u}{i}{t}$ holds is upper bounded by $c_i^{T+1}(\minUser-1)$ (Remember that  under the event $\{a_{u,t}=i \text{ and } \BBjul{u}{i}{t}\}$ item $i$ is recommended to a user $u$ whereas $i$ has already been recommended to a different user with type $\tau_U(u)$ before). Hence, for any $i\in\Gc_T$
 \[
 \sum_{u=1}^N
\sum_{t=1}^T
\ident[a_{u,t}=i, c_i^t<\thrjil, \BBjul{u}{i}{t}]
\leq
 \sum_{u=1}^N
\sum_{t=1}^T
\ident[a_{u,t}=i, \BBjul{u}{i}{t}] \leq c_i^{T+1} (\minUser-1)\,.\]

 The statement of lemma is derived from the above display using~\eqref{eq:jl-def-bad} and the definitions $f_T = |\Fc_T|$ and $g_T=\sum_{i\in \Gc_T} c_i^{T+1}$.




\input{CombineLBd.tex}



==> CombineLBd.tex <==

\subsubsection{Combining Steps~1 -- 5}
Here we combine the statement of Lemmas~\ref{l:BoundBad1},~\ref{l:BoundBad2},~\ref{l:BoundBad3},~\ref{l:BoundBad4}, and ~\ref{l:BoundBad5}  to to get a minimax statement as a lower bound for number of bad recommendations.

Combining Lemmas~\ref{l:BoundBad2} and~\ref{l:BoundBad3} and some algebraic manipulation give
\begin{align*}
\bad(T)
&\geq
\max\Big\{
(1-w_T) N\gamma_*^T,\, 
w_T N \thrjul
\Big\}
\\
&\geq
\min_{0\leq w_T\leq 1}\max\Big\{
(1-w_T) N\gamma_*^T,\, 
w_T N \thrjul
\Big\}
\\
&=
N\,
\frac{\thrjul \gamma_*^T }{\thrjul+\gamma_*^T }
\geq
\frac{1}{2}N\,
\min\{\gamma_*^T,\, \thrjul\}
\,.
\end{align*}
%
%%%%%%%%%%
Lemmas~\ref{l:BoundBad1} and~\ref{l:BoundBad5}  give
the following bound  (which subsequently will be used in the asymptotic analysis of the regret lower bound)
\begin{align*}
\bad(T)
&\geq
\max\Big\{
f_T \thrjil + g_T ,\, 
TN- \big[f_T (N-\thrjil) + g_T (\minUser-1) \big]
\Big\}
\\
&\geq
\min_{f_T,g_T}
\max\Big\{
f_T \thrjil + g_T ,\, 
TN- \big[f_T (N-\thrjil) + g_T (\minUser-1) \big]
\Big\}
\\
&\geq
T \min\{\thrjil, \frac{N}{\minUser}\}
\,.
\end{align*}
%
Finally, Lemmas~\ref{l:BoundBad1} and~\ref{l:BoundBad4} give
\begin{equation}
\bad(T)\geq 
\max\big\{
n_T, \frac{N}{\minUser}\gamma_*^T
\big\}\,.
\end{equation}
Combining the above statements gives
\begin{align}
\label{eq:LBcombineSteps}
\bad(T)
&\geq
\max\left\{ n_T,\,
\frac{N}{\minUser}\gamma_*^T,\, 
\frac{1}{2}N
\min\{\gamma_*^T,\, \thrjul\}
,\,
 T \min\big\{\thrjil, \frac{N}{ \minUser}\big\}
\right\}\,.
\end{align}
To compute a bound for the right hand side of the above display, we should note that the variables $n_T$ and $\gamma_*^T$ are not independent of each other. Also, the parameter $\minUser$ depends on the total number of users and the number of user types. 
In next section, we characterize these dependencies on the events which occur with high probabilities. Next, we bound expected value of bad recommendations on these events.
%%%%%%%%%%
%%%%%%%%%%
\subsubsection{Events of interest}
\label{sec:LBEvents}
%
%\begin{lemma}
%\label{l:JL-bdminUserP}
%The parameter $\minUser$ defined in Definition~\ref{def:jl-minUser} satisfies the following bound
%\begin{align*}
%\Pr\big[\minUser \geq \Theta_{\qu}(N)\big ]\leq 1/2\,.
%\end{align*}
%\end{lemma}
%
%\MK{Do I want to prove this? Am I sure it's correct? It's almost impossible that it's not correct}
In this section, we introduce two events which bound the parameters $\gamma_*^T$%, $\NonEmptyUser$, 
and $\minUser$  (Definitions~\ref{def:jl-gamma-U}%,~\ref{def:jl-NonEmptyUser}, 
and~\ref{def:jl-minUser}) in terms of the parameters of the model $\qu, \qi$ and $N$ and the number of items seen by the algorithm seen by time $T$ ($n_T$ in Definition~\ref{def:jl-itemsF}).



\begin{definition}
Let the function $\Lambda_{\qu}(N)$ be
\begin{align}
\label{eq:ThetaqIdef}
\Lambda:=\Lambda_{\qu}(N) = \begin{cases} 
3N/\qu & \text{ if } \quad N\geq 2\qu\log\qu
\\
7\log \qu & \text{ if }\quad 2\qu\log\qu > N \geq \qu\,.
\end{cases}
\end{align}
\end{definition}
\begin{lemma}
\label{l:BoundminUserSize}
Using Definition~\ref{def:jl-minUser} of $\minUser$, with probability at least $3/4$ the following holds:
\begin{align}
\label{eq:BoundminUserSize}
\minUser <
\Lambda_{\qu}(N)\,.
\end{align}
\MK{The proof of the tighter bound should be double checked}
\end{lemma}
The proof of this lemma is based on standard analysis of the balls and bins problem. Using the preference model introduced in Section~\ref{sec:model}, the type of each user is independently uniformly distributed among $\qu$ user types. Hence, the parameter $\minUser$ is the size of largest bin when $N$ balls are thrown into $\qu$ bins uniformly independently at random. A simple application of the Chernoff bound (Lemma~\ref{l:Chernoff}) and a union bound over the total number of user types gives the statement of this lemma. 

%
%\begin{lemma}
%\label{l:BoundNonEmptyUser}
%Using Definition~\ref{def:jl-NonEmptyUser}, 
%$\NonEmptyUser \geq  \frac{\qu}{2}$  with probability at least $1/4$.
%\end{lemma}
%\begin{proof}
%Note that $\NonEmptyUser$ is the number of nonempty bins after throwing $N$ balls in $\qu$ bins.
%The number of empty bins is $\qu-\NonEmptyUser$ and its expected value is
%$\Ex[\qu-\NonEmptyUser]  = \qu (1-1/\qu)^N\leq  \qu\exp(-N/\qu) $. 
%Using Markov inequality, 
%\[\Pr\big[ \NonEmptyUser < \frac{\qu}{2}\big] 
%=
%\Pr\big[ \qu- \NonEmptyUser \geq \frac{\qu}{2}\big] 
%\leq  \frac{2}{\qu}\Ex[\qu - \NonEmptyUser] 
%\leq 2\exp(-N/\qu)\leq \frac{3}{4}\,, \]
%where the last inequality uses $N\geq \qu$.
%\end{proof}


To bound the parameter $\gamma_*^T$ in terms of  $n_T$ and the parameters of the model, we use the following definition. 
%%%% %% %% 
%%%% %% %% 
%%%% %% %% 
%%%% %% %% 
%% %% %% %% Redone from here:
%%%% %% %% 
%\begin{definition}
%Let the function $\Theta_q(k)$ be
%\begin{align}
%\label{eq:ThetaqIdef}
%\Theta_{q}(k) := \begin{cases} 
%2\,,
% \,\quad&
% \text{if }\, k< k_0:=\sqrt{q}/3\\
%  3\, \frac{\log q}{\log q- \log k}\,,
% \,\quad&
% \text{if }\, k_0\leq k< k_1:=q/2\\
%8\log q\,, 
%\,\quad&
%\text{if }\, k_1\leq k< k_2:=2q\log q
%\\
%{4k}/{q}\,, 
%\,\quad&
%\text{if }\, k_2\leq k\,. \end{cases}
%\end{align}
%\end{definition}
%
%\begin{lemma}
%\label{l:JL-bdGammaStarP}
%The parameters $\gamma_*^T$ and $n_T$ defined in Definitions~\ref{def:jl-gamma-U} and~\ref{def:jl-itemsF} satisfy the following bound with probability at least half:
%\begin{align}
%\label{eq:JL-bdGammaStarP}
%%\Pr\Big[\gamma_*^T > \frac{T}{\Theta_{\qi}(n_T)}\Big ]\geq 1/2\,.
%\gamma_*^T > \frac{T}{\Theta_{\qi}(n_T)}\,.
%\end{align}
%\end{lemma}
%This lemma bounds the minimum number of item types recommended to any user by time $T$ as a function of the total number of items seen by the algorithm, $n_T$. 
%Heuristically speaking, each of $n_T$ items has one of $\qi$ item types. So roughly speaking, there are $n_T/\qi$ items per item type. Each user is recommended $T$ items by time $T$. So the number of item types recommended to any user should be proportional to $T/(n_T/\qi)$. 
%But formalizing this argument and getting the correct bounds require some care
%%The proof of this lemma is more involved than Lemma~\ref{l:BoundminUserSize} 
%since the algorithm picks the items to recommend sequentially. Hence, whether or not a new item is recommended potentially depends on the preference and type of the previously recommended items. To prove this lemma rigorously, we use the following definition:
%
%\begin{definition} \label{def:JL-rjT}
%Let $r_{\ti}^T$ be the number of items with item type $j$ that have been rated by time $T$:
%\[r_{j}^T=|\{i: \tau_I(i)=j, a_{u,t}=i, u\in[N], t\leq T\}|.\]
%\end{definition}
%
%
%For any user $u$, $T$ items from $\Nc_T=\Fc_T\cup\Gc_T$ with types in $\Gamma_u^T$ (defined in  Definition \ref{def:jl-gamma-U}) are recommended by time $T$. Hence, $T\leq \sum_{\ti\in\Gamma_{u}^T} r_{\ti}^T\,.$
%This implies 
%\begin{equation}\label{eq:maxrjT}
%\gamma_*^T := \min_{u} \gamma_u^T \geq \frac{T}{\max_{j}r_{j}^T}\,.
%\end{equation}
%Lemma~\ref{l:JL-bdGammaStarP} is a direct consequence of the above property and the following lemma:
%\begin{lemma}
%\label{l:JL-bdRjTP}
%For $r_j^T$ in Definition~\eqref{def:JL-rjT}, 
%$\Pr
%\left[\, 
%\max_{\ti\in[\qi]}r_j^T 
%\geq 
%\Theta_{\qi}(n_T)
%\right]
%\leq 1/2$.
%\end{lemma}
%The proof of this lemma is exactly the same as the proof  of Claim 7.9. in~\cite{RS1}. We present the proof in Section~\ref{sec:lbdRjTPproof} for the sake of completeness.



%%%%%%%%%%%%
%%%%%%%%%%%%
%%%%%%%%%%%
%%%%%%%%%%%%
%%%%%%%%%%%%
%%%%%%%%%%%
%%%%%%%%%%% 
\begin{definition}
Let the function $\Theta_q(k)$ be
%\begin{align}
%\label{eq:ThetaqIdef}
%\Theta_{q}(k) := \begin{cases} 
%2\,,
% \,\quad&
% \text{if }\, k< k_0:=\sqrt{q}/3\\
%  3\, \frac{\log q}{\log q- \log k}\,,
% \,\quad&
% \text{if }\, k_0\leq k< k_1:=q/2\\
%8\log q\,, 
%\,\quad&
%\text{if }\, k_1\leq k< k_2:=2q\log q
%\\
%{4k}/{q}\,, 
%\,\quad&
%\text{if }\, k_2\leq k\,. \end{cases}
%\end{align}
\begin{align}
\label{eq:ThetaqIdef}
\Theta_{q}(k) := \begin{cases} 
1\,,
 \,\quad&
 \text{if }\, k\leq 8\log q
\\
k q /4\,, 
\,\quad&
\text{if }\, 8\log q< k \,. \end{cases}
\end{align}
\end{definition}

\begin{lemma}
\label{l:JL-bdGammaStarP}
The parameters $\gamma_*^T$ and $n_T$ defined in Definitions~\ref{def:jl-gamma-U} and~\ref{def:jl-itemsF} satisfy the following bound with probability at least half
\begin{align}
\label{eq:JL-bdGammaStarP}
n_T >  \Theta_{\qi}\left(\frac{T}{\gamma_*^T}\right)\,.
%\\
%%\Pr\Big[\gamma_*^T > \frac{T}{\Theta_{\qi}(n_T)}\Big ]\geq 1/2\,.
%\gamma_*^T > \frac{T}{\Theta_{\qi}(n_T)}\,.
\end{align}

\end{lemma}
This lemma bounds the minimum number of item types recommended to any user by time $T$ as a function of the total number of items seen by the algorithm, $n_T$. 
Heuristically speaking, each of $n_T$ items has one of $\qi$ item types. So roughly speaking, there are $n_T/\qi$ items per item type. Each user is recommended $T$ items by time $T$. So the number of item types recommended to any user should be proportional to $T/(n_T/\qi)$. 
But formalizing this argument and getting the correct bounds require some care
%The proof of this lemma is more involved than Lemma~\ref{l:BoundminUserSize} 
since the algorithm picks the items to recommend sequentially. Hence, whether or not a new item is recommended potentially depends on the preference and type of the previously recommended items. In appendix~\ref{sec:lbdRjTPproof}, we give a rigorous proof of this Lemma.


\begin{definition}
\label{def:JL-Event}
Define event $\mathsf{E}$ to be the event on which all the events on
Lemmas~\ref{l:BoundminUserSize}  and~\ref{l:JL-bdGammaStarP} hold:
\begin{align}
\label{eq:BoundminUserSize}
\mathsf{E} = 
\Big\{ \minUser <
\Lambda_{\qu}(N),
\text{ and }
n_T >  \Theta_{\qi}\left(\frac{T}{\gamma_*^T}\right)
\Big\}\,.
\end{align}
\end{definition}
Using a union bound and Lemmas~\ref{l:BoundminUserSize},  and~\ref{l:JL-bdGammaStarP}  the event $\mathsf{E}$ holds with probability at least $1/4$.

%%%%%%%%%%%%
%%%%%%%%%%%%
%%%%%%%%%%%

%%%%%%%%%%%%
%%%%%%%%%%%%
%%%%%%%%%%%

%%%%%%%%%%%%
%%%%%%%%%%%%
%%%%%%%%%%%
\subsubsection{Proof of Lemma~\ref{l:jl-bad-lower}}
\label{sec:LBputtingitall}
To lower bound the expected number of bad recommendations and prove Lemma~\ref{l:jl-bad-lower}, we bound the right hand side of Equation~\eqref{eq:LBcombineSteps} on the events described in Definition~\ref{def:JL-Event} (Equations~\eqref{eq:BoundminUserSize} and~\eqref{eq:JL-bdGammaStarP}
hold). 
Applying tower property of expectation, 
\begin{align*}
\Ex\big[&\bad(T)\big]
\geq
\Ex\big[\bad(T)\, | \, \mathsf{E}\big]\,\, \Pr[\mathsf{E}]
\\
&\stackrel{(a)}{\geq}
\frac{1}{4}\,\,
\min_{n_T, \gamma_*^T, \minUser}\,\,
\max\Big\{ n_T,\,
\frac{N\gamma_*^T}{\minUser},\, 
\frac{N}{2}\min\{\gamma_*^T,\,\thrjul\},\,
% \\ &\quad 
 T \min\{\thrjil, \frac{N}{ \minUser}\}
\Big\}
\\
&\quad\quad\quad\text{subject to } \quad
\minUser <
\Lambda_{\qu}(N) 
\,\,\text{ and } \quad
n_T >  \Theta_{\qi}\left(\frac{T}{\gamma_*^T}\right)
\\
&\stackrel{}{\geq}
\frac{1}{4}\,\,
\min_{\gamma_*^T\geq 1}\,\,
\max\Big\{ \Theta_{\qi}\left(\frac{T}{\gamma_*^T}\right),\,
\frac{N\gamma_*^T}{\Lambda_{\qu}(N)},\, 
\frac{N}{2}\min\{\gamma_*^T,\, \thrjul\},\,
T \min\{\thrjil, \frac{N}{\Lambda_{\qu}(N) }\}
\Big\}
\,.
\end{align*}
(a) uses the application of 
Lemmas~\ref{l:JL-bdGammaStarP} and~\ref{l:JL-bdRjTP} which implies $\Pr[\mathsf{E}]>1/4$. It also uses the fact that the bound in Equation~\eqref{eq:LBcombineSteps} holds for any value of the parameters $n_T, \gamma_*^T$ and $\minUser$. Hence, the number of bad recommendations is bounded by the minimum value of the right hand side of Equation~\eqref{eq:LBcombineSteps} over the parameters $n_T, \gamma_*^T$ and $\minUser$. Event $\mathsf{E}$ in Definition~\ref{def:JL-Event} induces some constraints over the minimization. 

The lower bound in right hand side of the above display is a minimax where the minimum is over the realization of the  variable $\gamma_*^T$. 
%\MK{update from here}
%Note that the maximum is taken over several terms which are nondecreasing  in $n_T$ and $\gamma_*^T$ and nonincreasing in $\minUser$. Also, according to the constraints of this optimization, $\gamma_*^T$ is lower bounded by a nonincreasing function of $n_T$ and $\minUser$ is upper bounded in terms of $\qu$ and $N$. 
%This behavior opens the door for finding a lower bound for the minimax optimization in terms of the parameters of the problem $\qi, \qu, N$ and $T$. But due to the discontinuity in the optimizer and the constraints of the optimization, the lower bound would also be discontinous. 
Due to the discontinuity in the optimizer and the constraints of the optimization, the lower bound would also be discontinuous. 
As an example, the lower bound takes different forms depending on whether $N\geq 2\qu \log \qu$ or $N< 2\qu \log \qu$ since the function on $\Lambda_{\qu}(N)$  has discontinuity here. 
From here on, we use the shorthand $\Lambda=\Lambda_{\qu}(N)$ and $\gamma = \gamma_*^T$ for the sake of brevity.
Define 
\begin{align}
f_1(\gamma) 
&=
\begin{cases}
T\qi / (4\gamma) & \text{ if } \gamma < T/(8\log \qi)
 \\
 1  & \text{ if } \gamma > T/(8\log \qi)
 \end{cases}
 \quad \quad
f_2(\gamma)= \max\big\{ \frac{N}{\Lambda} \gamma,\frac{N}{2}, \min\{\thrjul,\gamma\}\big\}
\notag
\\
f_3(\gamma)&=
T \min\big\{\thrjil, \frac{N}{\Lambda }\big\}\,.
\label{eq:deffgammaLB}
 \end{align}
Then, 
\begin{align*}
\Ex\big[\bad(T)\big]
\geq 
\frac{1}{4}
\min_{\gamma\geq 1}
\max\big\{
f_1(\gamma), f_2(\gamma), f_{3}(\gamma)\big\}\,.
\end{align*}
\begin{figure}[h]
\includegraphics[width=15cm]{figures/LBf}
\caption{The functions \MK{the figures and the caption should be updated.}}
\label{fig:LBfig}
\centering
\end{figure}
Note that the functions $f_1(\gamma), f_2(\gamma)$ and constant function $f_{3}(\gamma)$ are parameterized by the parameters of the system $\qu, \qi, N$ and $T$. So depending on the realization of these parameters, the above minimax takes different forms. 
To lower bound the minimax term, we observe that $f_{1}(\gamma)$ is a nonincreasing function of $\gamma$; $f_{2}(\gamma)$ is a nondecreasing function of $\gamma$; and $f_{3}(\gamma)$ is a constant function of $\gamma$ (Figure~\ref{fig:LBfig}). 
Claim~\ref{claim:LBMT} elminates variable $\gamma$ to compute $\min_{\gamma\geq 1}
\max\big\{
f_1(\gamma), f_2(\gamma)\big\}$. Note that $f_3(\gamma)$ is independent of $\gamma$. So, we have 
\[
\Ex\big[\bad(T)\big]
\geq 
\frac{1}{4}
\max\Big\{
M(T), T \min\big\{\thrjil, \frac{N}{\Lambda }\big\} \Big\}
\geq 
\frac{1}{8} M(T)
+ \frac{T}{8}  \min\big\{\thrjil, \frac{N}{\Lambda }\big\}
\,.
\]


\begin{claim} 
\label{claim:LBMT}
Define $M(T):=\min_{\gamma\geq 1}
\max\big\{
f_1(\gamma), f_2(\gamma)\big\}$ where $f_1(\gamma)$ and $f_2(\gamma)$ are defined in Eq.~\eqref{eq:deffgammaLB}. Then, 


\paragraph{When $ \thrjul \leq
  4\frac{\qi\, \log\qi }{N}$:}
\begin{align}
\label{eq:MdefLBRegime1}
M(T) = 
\begin{cases}
\frac{N}{2}\frac{T}{8\log \qi},
\quad & \text{ if }
T\leq 8\thrjul \log \qi \\\\
\frac{N}{2} \thrjul 
\quad & \text{ if }
 8\thrjul \log \qi < T \leq \frac{\Lambda}{2}  8\thrjul \log \qi 
 \\\\
  \frac{N}{\Lambda} \frac{T}{8\log \qi}
 \quad & \text{ if }
 \frac{\Lambda}{2}  8\thrjul \log \qi  < T \leq 
  \frac{\Lambda}{2} 32\frac{\qi\, (\log\qi)^2 }{N}
 \\\\
 \frac{1}{2}\sqrt{T\qi \frac{N}{\Lambda}}
 \quad & \text{ if }
  \frac{\Lambda}{2} 32\frac{\qi\, (\log\qi)^2 }{N} <T
\end{cases}
\end{align}

%%%%%%%%%%
%%%%%%%%%%
%%%%%%%%%%
\paragraph{
When $
 \thrjul 
 >
  4\frac{\qi\, \log\qi }{N}$:}
\begin{align}
\label{eq:MdefLBRegime2}
M(T) = 
\begin{cases}
\frac{N}{2}\frac{T}{8\log \qi},
\quad & \text{ if }
T\leq  32\frac{\qi\, (\log\qi)^2 }{N}\\\\
 \sqrt{\frac{T\qi N}{8}}
\quad & \text{ if }
  32\frac{\qi\, (\log\qi)^2 }{N}< T \leq \frac{2N}{\qi} \thrjul^2
 \\\\
  \frac{N}{2} \thrjul 
 \quad & \text{ if }
 \frac{2N}{\qi} \thrjul^2< T \leq 
  \frac{\Lambda}{2}  \frac{2N}{\qi} \thrjul^2
 \\\\
 \frac{1}{2}\sqrt{T\qi \frac{N}{\Lambda}}
 \quad & \text{ if }
  \frac{\Lambda}{2}  \frac{2N}{\qi} \thrjul^2<T
\end{cases}
\end{align}
\end{claim}

\begin{proof}

To find $M(T):=\min_{\gamma\geq 1}
\max\big\{
f_1(\gamma), f_2(\gamma)\big\}$, define
$$\gamma_1 : = \sqrt{\frac{T\qi}{2N}}, \quad \text{and} \quad 
\gamma_2 : = \sqrt{\frac{T\qi}{4} \frac{\Lambda}{N}}$$
to be the intersection of function $\frac{T\qi}{4\gamma}$ with the functions  $\frac{N}{2}\gamma$ and $\frac{N}{\Lambda}\gamma$  respectively.

\paragraph{Regime 1:}
$M(T) = \frac{N}{2}\frac{T}{8\log \qi}$. This happens when 
\[\frac{T}{8\log \qi} \leq \thrjul,
\quad 
\text{and }\quad 
\frac{T}{8\log \qi} \leq \gamma_1\,,\]
which occurs when
 \[T\leq 
 \min\big\{
 8\log \qi \thrjul, \, \, 32\frac{\qi\, (\log\qi)^2 }{N}
 \big\}.\]

\paragraph{Regime 2:}
$M(T) = \frac{T\qi}{4\gamma_1}  =  \sqrt{\frac{T\qi N}{8}}$. 
This happens when 
\[
\frac{T}{8\log \qi} > \gamma_1
\quad \text{ and }
\gamma_1 \leq \thrjul\,,
\]
which occurs when
\[ 32\frac{\qi\, (\log\qi)^2 }{N}
< T \leq 
\frac{2N}{\qi} \thrjul^2\,. \]


\paragraph{Regime 3:}
If none of the other regimes happen, we have $M(T) = \frac{N}{2} \thrjul$.
In particular, $M(T) = \frac{N}{2} \thrjul$ when 
\[f_1( \thrjul ) 
\geq \frac{N}{2} \thrjul  
> f_1(\frac{\Lambda}{2} \thrjul )\]

This happen when either of the following events happen: 
\[E_1 = \{  \thrjul \leq \frac{T}{8\log \qi} < \frac{\Lambda}{2} \thrjul
 \quad \text{ and } \quad
 \frac{T\qi}{4 \thrjul } \geq \frac{N}{2}  \thrjul 
\}\]

\[E_2 = \{  \thrjul \leq \frac{T}{8\log \qi} 
 \quad \text{ and } \quad
\frac{N \Lambda }{4}    >
 \frac{T\qi}{4 \thrjul } \geq \frac{N}{2}  \thrjul 
\}\] 

which happens when 

\[
\max\big\{ 
8\thrjul \log \qi , \,\, 2 \frac{N}{\qi} \thrjul^2\big\}
\leq
T
<
\frac{\Lambda }{2}
 \max\big\{ 
8\thrjul \log \qi , \,\, 2 \frac{N}{\qi} \thrjul^2\big\}
\]


\paragraph{Regime 4:}
$M(T) = \frac{N}{\Lambda} \frac{T}{8\log \qi}$.
This happens when 
\[  \frac{\Lambda}{2}\thrjul
<
\frac{T}{8\log \qi}
<\gamma_2
\]
which occurs when
\[  4\Lambda \thrjul \log \qi 
< T < 
16 \qi (\log \qi)^2 \frac{\Lambda}{N}
\]

\paragraph{Regime 5:}
$M(T) = \frac{T\qi}{4\gamma_2}  =  \frac{1}{2}\sqrt{T\qi \frac{N}{\Lambda}}$.
This happens when 
\[  \frac{\Lambda}{2}\thrjul
<\gamma_2 \leq 
\frac{T}{8\log \qi}
\]
which occurs when
\[
\max\big\{ 
N\Lambda \frac{\thrjul^2}{\qi},
16 \qi (\log \qi)^2 \frac{\Lambda}{N}
\big\}
< T\]

Putting it all together, we will have two different cases 
$ 8\log \qi \thrjul \leq  32\frac{\qi\, (\log\qi)^2 }{N}$
or
$ 8\log \qi \thrjul >  32\frac{\qi\, (\log\qi)^2 }{N}$.

Note that 
$ 8\log \qi \thrjul \leq  32\frac{\qi\, (\log\qi)^2 }{N}$ if and only if $ 8\log \qi \thrjul \geq \frac{2N}{\qi} \thrjul^2$. As a result, there are two different cases:

\paragraph{Case 1: 
($ \thrjul \leq
  4\frac{\qi\, \log\qi }{N}$)}

In this case ($  \frac{2N}{\qi} \thrjul^2\leq 8\thrjul \log \qi \leq  32\frac{\qi\, (\log\qi)^2 }{N}$) and Regime 2 does not appear, and $M(T)$ is as defined in Equation~\eqref{eq:MdefLBRegime1} in the statement of the claim.

%\begin{align*}
%M(T) = 
%\begin{cases}
%\frac{N}{2}\frac{T}{8\log \qi},
%\quad & \text{ if }
%T\leq 8\thrjul \log \qi \\\\
%\frac{N}{2} \thrjul 
%\quad & \text{ if }
% 8\thrjul \log \qi < T \leq \frac{\Lambda}{2}  8\thrjul \log \qi 
% \\\\
%  \frac{N}{\Lambda} \frac{T}{8\log \qi}
% \quad & \text{ if }
% \frac{\Lambda}{2}  8\thrjul \log \qi  < T \leq 
%  \frac{\Lambda}{2} 32\frac{\qi\, (\log\qi)^2 }{N}
% \\\\
% \frac{1}{2}\sqrt{T\qi \frac{N}{\Lambda}}
% \quad & \text{ if }
%  \frac{\Lambda}{2} 32\frac{\qi\, (\log\qi)^2 }{N} <T
%\end{cases}
%\end{align*}

%%%%%%%%%%
%%%%%%%%%%
%%%%%%%%%%
\paragraph{Case 2: 
($
 \thrjul 
 >
  4\frac{\qi\, \log\qi }{N}$ )}

In this case ($  \frac{2N}{\qi} \thrjul^2 >
 8\thrjul \log \qi 
 >
  32\frac{\qi\, (\log\qi)^2 }{N}$ ) and  Regime 4 does not appear, and $M(T)$ is as defined in Equation~\eqref{eq:MdefLBRegime2} in the statement of the claim.
%
%\begin{align*}
%M(T) = 
%\begin{cases}
%\frac{N}{2}\frac{T}{8\log \qi},
%\quad & \text{ if }
%T\leq  32\frac{\qi\, (\log\qi)^2 }{N}\\\\
% \sqrt{\frac{T\qi N}{8}}
%\quad & \text{ if }
%  32\frac{\qi\, (\log\qi)^2 }{N}< T \leq \frac{2N}{\qi} \thrjul^2
% \\\\
%  \frac{N}{2} \thrjul 
% \quad & \text{ if }
% \frac{2N}{\qi} \thrjul^2< T \leq 
%  \frac{\Lambda}{2}  \frac{2N}{\qi} \thrjul^2
% \\\\
% \frac{1}{2}\sqrt{T\qi \frac{N}{\Lambda}}
% \quad & \text{ if }
%  \frac{\Lambda}{2}  \frac{2N}{\qi} \thrjul^2<T
%\end{cases}
%\end{align*}

\end{proof}

\newpage


















%\input{minimax}

==> JLBadCount.tex <==
\subsection{Proof of Lemma~\ref{l:JL-marting-gammaBD}}
\label{sec:JL-proof-gammaBD}
We get a lower bound on $\gamma_*^T$ via an upper bound on $\max_{j}r_{j}^T$, which is in turn obtained via martingale concentration for each $r_{j}^T$. This is essentially just a question of bounding the fullest bin in a balls and bins scenario, with the added complication that the time-steps in which balls are thrown is a martingale. Thus the number of balls (i.e., $f_T + g_T$) is random, and the decision to throw a ball at a given time may depend on the configuration of balls in bins.
	
Let $r^t =(r_1^t,\dots, r_{\qi}^t)$. Any new item has type uniformly distributed on $[\qi]$, and it follows that the sequence $r_{j}^t - (f_t+g_t)/\qi$ is a martingale with respect to filtration $\Fc_t = \sigma(r^0,r^1,\dots, r^t)$, because $f_t+ g_t$ is incremented whenever a new item is recommended and this item contributes to $r^t_j$ with probability $1/\qi$.
%
It turns out to be easier to work with a different martingale that considers each user separately, so that the item counts are incremented by at most one at each step. Consider the lexicographical ordering on pairs $(t,u)$, where $(s,v)\leq(t,u)$ if either $s< t$ or $s=t$ and $v\leq u$ (the recommendation to user $v$ at time $s$ occurred before that of user $u$ at time $t$). Let $r^{t,u} = (r_1^{t,u} ,\dots, r_{\qi}^{t,u} )$, where for $j\in [\qi]$
$$
		r_{j}^{t,u}=\big|\big\{i: \tau_I(i)=j, a_{v,s}=i \text{ for some } (s,v)\leq (t,u)\big\}\big|,
$$
and $\rho^{t,u} = \sum_j	r_{j}^{t,u}$. 
	We now define a sequence of stopping times $Z_k \in \mathbb{N}\times [N]$, with $Z_0=(0,N)$ and
	$$
	Z_k = \min\big\{(t,u)> Z_{k-1}: \rho^{t,u} > \rho^{t,u-1}\big\}\,,
	$$
	where $(t,0)$ is interpreted as $(t-1,N)$. $Z_k$ is the first $(t,u)$ such that a new item is recommended by the algorithm for the $k$th time, so $\rho^{Z_k}=k$. The $Z_k$ are stopping times with respect to $(\rho^{t,u})$, and observe that $k^* = \max\{k: Z_k \leq (T,N)\} = \rho^{T,N} = f_T + g_T$ since $f_T+g_T$ is the total number of items recommended by the algorithm by the end of time $T$. Also, $\rho^{Z_{k^*}}=f_T+g_T$ and $r_j^{Z_{k^*}}=r_{\ti}^{(T,N)}$ for all $\ti\in[\qi]$.
	
	The sequence $M_{t,u}=r_j^{t,u} - \rho^{t,u}/\qi$ is a martingale w.r.t. $\Fc_{t,u}=\sigma(\rho^{1,1},\dots \rho^{t,u})$, and it follows that so is $\widetilde M_{k} = M_{(T,N)\wedge Z_k}$, this time with respect to $\widetilde\Fc_k:=\Fc_{(T,N)\wedge Z_k}$. Since $Z_{k^*}\leq (T,N)$, we have $\widetilde M_{k^*}=M_{Z_{k^*}}$ 
	We would like to apply martingale concentration (Lemma~\ref{l:martingaleBound}) to $\widetilde M_{k}$, and to this end observe that $\mathrm{Var}(\widetilde M_{k}|\widetilde\Fc_k) \leq 1/\qi$ and $|\widetilde M_{k} - \widetilde M_{k-1}|\leq 1$ almost surely. 
	
	
	For any $k\geq k_0:= 2\qi \log \qi$, Lemma~\ref{l:martingaleBound} gives
	\begin{align*}
\Pr\Big[\widetilde M_{k} \geq  \frac{3k}{\qi}\Big] \leq \exp\bigg(\frac{-9k^2/\qi^2}{2k/\qi + k/\qi}\bigg) = \exp\Big(-\frac{3k}{\qi}\Big)\,.
\end{align*}
By the union bound,
	\begin{align}
\Pr\Big[ \exists k\geq k_0\text{ s.t. }\widetilde M_{k} \geq  \frac{3k}{\qi}\Big]&\leq \sum_{k\geq k_0} \exp\Big(-\frac{3k}{\qi}\Big) 
=
 \frac{\exp\Big(-\frac{3k_0}{\qi}\Big)}{1-\exp(-3/\qi)} 
\leq \frac{1}{\qi^4}\,.\label{eq:IL-mart-k-large}
\end{align}
where the last inequality uses ${1-\exp(-3/\qi)}> \qi^{-2}$ (which is derived using $e^{-a}\leq 1-a+a^2/2$ and $\qi>1$). 

For $k< k_0$ we get 
\begin{align*}
	\Pr\Big[\widetilde M_{k} \geq  6\log \qi\Big] \leq \exp\bigg(\frac{-36\log^2\qi}{2k_0 +  2\log \qi}\bigg) \leq \frac{1}{\qi^6}\,.
\end{align*}
So 
\begin{align}\label{eq:IL-mart-k-small}
\Pr\Big[ \exists k< k_0\text{ s.t. }\widetilde M_{k} \geq   6\log \qi\Big]\leq \sum_{k<k_0} \frac{1}{\qi^6}= \frac{k_0}{\qi^6}\leq \frac{1}{\qi^4}\,.
\end{align}
Now
\begin{align}
&	\Pr\Big[ r_j^T \geq \max\Big\{8\log\qi, \frac{4(f_T+g_T)}{\qi}\Big\}\Big] \overset{(a)}{=	}\Pr\Big[ \widetilde M_{k^*} \geq \max\{8\log\qi, \frac{4k^*}{\qi}\}-\frac{k^*}{\qi}\Big] 
\nonumber
\\
	&= 
		\Pr\Big[ \widetilde M_{k^*} \geq \max\{8\log\qi-\frac{k^*}{\qi}, \frac{3k^*}{\qi}\},k^*\geq k_0\Big]
		+
			\Pr\Big[ \widetilde M_{k^*} \geq \max\{8\log\qi-\frac{k^*}{\qi}, \frac{3k^*}{\qi}\}, k*<k_0\Big] 
		\nonumber
		\\
&\overset{(b)}{=}\Pr\Big[\widetilde M_{k^*} \geq \frac{3k^*}{\qi},k^*\geq k_0\Big]+	\Pr\Big[ \widetilde M_{k^*} \geq 8\log\qi-\frac{k^*}{\qi}, k*<k_0\Big] 
\nonumber
\\		
&\overset{(c)}{\leq}\Pr\Big[\exists k\geq k_0 \text{ s.t. }\widetilde M_{k} \geq \frac{3k}{\qi}\Big]
+	\Pr\Big[ \exists k<k_0 \text{ s.t. }\widetilde M_{k} \geq 6\log\qi\Big] 
\overset{(d)}{\leq}
 \frac{2}{\qi^4}\,.\label{e:itemCount}
	\end{align}
	Here (a) follows by unpacking the definitions of $\widetilde M_k$ and $k^*$, (b) and (c) use the definition $k_0 =2\qi \log \qi$; (d) follows by~\eqref{eq:IL-mart-k-large} and~\eqref{eq:IL-mart-k-small}. 
	
	Equations~\eqref{e:itemCount} and~\eqref{eq:maxrjT} and the union bound for $j\in[\qi]$ imply that
\begin{align*}	
	\Pr\bigg[\gamma_*^T &\leq \min\left\{\frac{T}{8\log\qi},\frac{T\qi}{4(f_T+g_T)} \right\} \bigg] \\
	&\leq 
	\Pr\left[ \max_{\ti\in[\qi]}r_j^T \geq \max\left\{8\log\qi, \frac{4(f_T+g_T)}{\qi}\right\}\right] \leq \frac{2}{\qi^3}\leq \frac{1}{2}\,.%\qedhere
	\end{align*}

==> JU-exploit-errortemp.tex <==

\subsection{Probability of not finding enough exploitable items}
For any $u\in [N]$, $\R_u$ is the set of items exploitable by user $u$ in the algorithm \textsf{Exploit}.
%
The sets $\R_u$ are formed in Lines~\ref{Line:DefRu1} or~\ref{Line:DefRu2} of~ \textsc{Explore}  
 depending on whether $\ell\leq \thrjuu$ or $\ell>\thrjuu$. 
The parameter $\ell$ is determined in Equations~\eqref{eq:ParamChoice2ell} or~\eqref{eq:ParamChoice1} as a function of time horizon $T$. 

When $\ell\leq \thrjuu$,$\R_u=\bigcup_{j:L_{u,\rep_\ti}=+1} \S_j$ according to Lines~\ref{Line:defSj2} and~\ref{Line:DefRu1} of \textsc{Explore} where $\S_j$ contains the $j$-th item in $\Mcc{2}$ (i.e., $\rep_j$) and the set of items in $\Mcc{1}$ which are posited to have the same type as $\rep_j$.

When $\ell > \thrjuu$, users are grouped by the algorithm into partitions $\Pc_k$. 
According to Line~\ref{Line:DefRu2}, in this regime,  $\R_u=\bigcup_{u'\in\Pc_{\tu}} \bigcup_{j:L_{u',\rep_\ti}=+1} \S_j$ for each $u$ such that $\tauh(u)=k$. Here, $\S_j$ contains the $j$-th item in $\Mcc{3}$ (i.e., $\rep_j$) and the set of items in $\Mcc{1}$ which are posited to have the same type as $\rep_j$.

Lemmas~\ref{l:ju-exp-R-u} and~\ref{l:ju-exp-R-u2} in this Section upper bound 
$\Pr[|\R_u|< T]$ in two regimes specified in Sections~\ref{sec:UUparam} and~\ref{sec:IJparam}. 
These bounds are used in Equations~\eqref{eq:ju-bound-A2}  and~\eqref{eq:ju-bound-A2-UU}.


%%%%%%%%%%%%%%

\subsubsection{Bounding $\Pr[|\R_u|< T]$ in the regime specified in Section~\ref{sec:IJparam}}
\MK{I don't know if I want to keep this and the remark}
Lemma~\ref{l:ju-exp-R-u} in this section bounds $\Pr[|\R_u|< T]$ in the regime  specified in Section~\ref{sec:IJparam}.
%
 First, the following remark goes over the parameter values in this regime.  

\begin{remark}[Parameter values in the regime  specified in Section~\ref{sec:IJparam}]
\label{Rem:ParamLargequApp}
As a reminder,  according to~\eqref{eq:ParamChoice2} in Section~\ref{sss:params}, in this regime  $\qu \geq 9 \log(N\qi)$ and the parameters of the algorithm are chosen as follows: 
\begin{align*}
M_1 & = \left\lceil 15\frac{\qi}{\ell}T\right\rceil
,\quad 
M_2 =
\big\lceil 2\min\{ \ell,\thrjuu\}\big\rceil,
 \quad \text{ and }\quad
%\\&
 M_3
=
\begin{cases}
\lceil 2\ell \rceil, 
&
\text{ if } \ell\leq \frac{\qi}{8},
\\
\lceil\qi \log(N\qi) \rceil
& \text{ if } \ell >\frac{\qi}{8}\,.
 \end{cases}
%\label{eq:AppParamChoice2}
\end{align*}

We will use the following properties of the parameters
\begin{equation}
\label{eq:ParamAssumptionsLargequ}
 N\geq \qu,\quad 
  \qi\geq 25\log N,\quad  
  N>100, \quad 
\text{and}  \quad \thrjuu > 14\,.
 \end{equation}
\end{remark}

The first three inequalities in~\eqref{eq:ParamAssumptionsLargequ} are the assumptions throughout the paper specified in Section~\ref{ss:pref}. 
Equation~\eqref{eq:defthrjuu} defines $\thrjuu = \log (N\qu^2)$.
When  $\qu \geq 9 \log(N\qi)$, the assumption $N>100$ gives $\log N>4$, $\qu\geq 36$ and $\thrjuu = \log (N\qu^2)\geq \log N + 2\log 36\geq 14$. 
%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
\begin{lemma}\label{l:ju-exp-R-u}
 In the regime specified in Section~\ref{sec:IJparam},
for any user $u\in[N],$
\[\Pr[|\R_u|< T] \leq 
\exp(-T/5) +2 \exp(-\ell/8) + 2/N
\,.\]
And  for $T>5$
\[\Exp{(T- |\R_u |)_+}\leq 2+2 T\exp(-\ell/8) + 2T/N\,.
\]

\end{lemma}

\begin{proof}


The  number of items in $\Mcc{1}$ is 
$M_1=\left\lceil\frac{15\qi}{\ell}T \right\rceil$.
 Hence, there are about $\frac{15}{\ell}T$ items from each of the item types in $\Mcc{1}$.
Roughly speaking, any user $u$ likes about half of the  $\ell$ item types learned by the algorithm. 
The set $\R_u$ includes  the items in $\Mcc{1}$ which user $u$ is expected to like.  
 So, it is not surprising that with high probability $|\R_u|\geq T$. 
 Next, we go over the details of this high level argument. 

Let $\Lc$ be the set of item types learned by the algorithm after the exploration phase.
Hence,
\begin{align}
\label{e:defLc}
\Lc
& :=
\begin{cases}
\big\{ \ti\in[\qi]:
\exists i\in \Mcc{2}, \tau_I(i)=\ti
 \big\}, 
 \quad
& \text{ if }
 \ell\leq \thrjuu
\\
\\
\big\{ \ti\in[\qi]:
\exists i\in \Mcc{3}, \tau_I(i)=\ti
 \big\}, 
 \quad
& \text{ if }
 \ell > \thrjuu\,.
 \end{cases}
\end{align}
Note that, with this definition, $|\Lc|= \disi(\mathcal{M}_2)$ when $\ell \leq \thrjuu$ and $|\Lc|= \disi(\mathcal{M}_3)$ when $\ell > \thrjuu$.

For given user $u$, let $\Lc_u$ be the set of item types learned by the algorithm and liked by user $u$:
\begin{align}\label{eq:defLcu}
\Lc_u
&:=
\big\{
\ti\in \Lc: \xi_{\tau_U(u), \ti} = +1
\big\},
\quad 
\text{and } \quad
\ell_u := \big| \Lc_u\big|
\,.
\end{align}
%
Lemma~\ref{l:boundsizeLu} shows that with the choice of parameters made by the algorithm (Remark~\ref{Rem:ParamLargequApp}), 
\begin{equation*}
\Pr\big[\ell_u\leq \ell/8\big] \leq 2\exp\big( -\ell/8 \big) + \frac{1}{N}\,.
\end{equation*}
To bound the size of set $\R_u$, we apply total probability lemma to get
\begin{align}
\Pr&\Big[
|\R_u|\leq T 
\Big]
\leq 
\Pr\Big[
|\R_u|\leq T,\,\,  \ell_u\geq \ell/8,\,\,  \BB^c
\Big]
+
\Pr\Big[
\ell_u<\ell/8 
\Big]
+
\Pr\Big[
\BB\Big]\,,
\label{eq:BoundRudecompose}
\end{align}
where the event $\BB^c$, defined in~\eqref{e:ju-bcal},
holds when either no partitioning over the users happen (when $\ell\leq \thrjuu$) or the partitioning over the users is correct. 
%s the event under which the partitioning over the users made by the algorithm coincides with the partitioning over the users based on their types. 


Plugging in the Lemmas~\ref{l:ju-user-mis-pr},~\ref{l:boundsizeRuLuBc}, and~\ref{l:boundsizeLu} into~\eqref{eq:BoundRudecompose} 
gives
\begin{align*}
\Pr\Big[ 
|\R_u|<  T
\Big]
\leq
\exp( - T/5) + 2\exp(-\ell/8) + 2/N\,.
\end{align*}
Hence,
\begin{align*}
\Exp{(T- |\R_u |)_+}
& \leq 
T\exp( - T/5) + 2T\exp(-\ell/8) + 2T/N
\\
&\leq
2 +2 T\exp(-\ell/8) + 2T/N
\,,
\end{align*}
where we used $T\exp( - T/5)<2$ for $T>5$ in the last inequality.
%
\end{proof}




%%%%%%%%%%
%%%%%%%%%%
\begin{lemma}
Let $\Lc_u$ and $\ell_u=|\Lc_u|$ be defined in Equation~\eqref{eq:defLcu}. Then, 
\label{l:boundsizeRuLuBc}
\begin{align*}
\Pr\Big[ 
|\R_u|< T,\,\,  \ell_u\geq \ell/8,\,\,   \BB^c
\Big]
&\leq
\exp\big(-T/5\big)\,.
\end{align*}
\end{lemma}
\begin{proof}

For $\ti'\in[\qi]$, define 
\begin{align}\label{eq:UBdefRj}
\Rb(\ti')=
\big\{
i\in\Mcc{1}: \tau_I(i) = \ti'
\big\}\,,
\end{align}
to be the set of items in $\Mcc{1}$ with type $\ti'$. 
%
%Claim~\ref{c:Rbsubseteq} shows that 
Condition on event $\BB^c$, 
\begin{align}\label{eq:Rbsubseteq}
\bigcup_{\ti'\in\Lc_u} \Rb(\ti')
\subseteq 
\R_u 
\end{align}
where $\Lc_u$ is defined in~\eqref{eq:defLcu}.
To see this, %remember that event $\BB$ holds if and only if either no partitioning over the users happen (when $\ell\leq \thrjuu$) or the partitioning over the users is correct. 
remember that the set $\R_u$ in the algorithm is  the union of sets $\S_{\ti}$'s such that the representative $\rep_{\ti}$ is liked by user $u$ or a user in the same partition as $u$ (Line~\ref{Line:DefRu1} or~\ref{Line:DefRu2} of Alg. \textsc{Explore}). 
Condition on $\BB^c$, the partitioning made by the algorithm over the users coincides with their user types. 
Hence, condition on $\BB^c$,
the set $\R_u$ is the union of sets $\S_{\ti}$'s such that the representative $\rep_{\ti}$ is liked by all users of type $\tau_U(u)$: $\R_u = \bigcup_{\ti: L_{u,\rep_{\ti}}=+1} \S_{\ti}$.
Also, according to Remark~\ref{rem:partitionionuserserror}, the set $\S_{\ti}$ is a superset of items in $\Mcc{1}$ with the same type as representative $\rep_{\ti}$ (since items of similar types always fall into the same group): $\Rb(\tau_I(\rep_{\ti}))\subseteq \S_{\ti}$. 
So condition on $\BB^c$,~\eqref{eq:Rbsubseteq} holds.

Next, we will show that condition on the event $\BB^c$  and given the set $\Lc_u$ and $\ell_u = |\Lc_u|$, the size of the set $\R_u$ stochastically dominates a
 Binomial $(M_1, \ell_u/\qi)$ random variable.

Note that the event $\BB^c$ only depends on the choice items  in $\Mcc{2}$ and the preference of users for those items. The set $\Lc_u$ is also determined by the set of items in either $\Mcc{2}$ or $\Mcc{3}$ (depending on whether $\ell\leq \thrjuu$ or not) and their types.
 Whereas for fixed $\ti'$, $\Rb(\ti')$ (defined in~\eqref{eq:UBdefRj}) depends on the types of items in $\Mcc{1}$. 
 Since the items in $\Mcc{1}$ are chosen independently of $\Mcc{2}, \Mcc{3}$ and the feedback taken by the algorithm, the type of items in $\Mcc{1}$ are independent and uniformly distributed on $[\qi]$. Hence,  the
size of the set $\bigcup_{\ti'\in\Lc_u} \Rb({\ti'})$ is Binomial distributed with parameters $(M_1,\ell_u/\qi)$. 
We use this to get
\begin{align*}
\Pr\Big[ 
|\R_u|< T,\,\,  \ell_u\geq \ell/8,\,\,   \BB^c
\Big]
&\leq
\Pr\Big[
|\R_u|< T  \,\Big|  \ell_u\geq \ell/8,\,\, \BB 
\Big]
\\
&\stackrel{(a)}{\leq}
\Pr\Big[
\bigcup_{\ti\in\Lc_u} \big|\Rb({\ti})\big| < T  
\,\Big| \ell_u\geq \ell/8 ,\,\, \BB 
\Big]
\\
&\stackrel{(b)}{\leq}
\exp\big(-T/5\big)\,.
\end{align*}
where (a) uses~\eqref{eq:Rbsubseteq}.
(b)  uses an application of Chernoff bound in Lemma~\ref{l:Chernoff} on Binomial$(M_1,\ell/(8\qi))$ 
and the choice of $M_1 = \lceil 15 \frac{\qi}{\ell}T\rceil$.
\end{proof}
%%%%%%%%%%%%%
%%%%%%%%%%%%%
\begin{lemma}
\label{l:boundsizeLu}
Let $\Lc_u$ and $\ell_u=|\Lc_u|$ be defined in Equation~\eqref{eq:defLcu}. Then, 
\begin{align*}
\Pr\big[\ell_u\leq \ell/8\big] \leq 2\exp\big( -\ell/8 \big) + \frac{1}{N}
\,.
\end{align*}
\end{lemma}

\begin{proof}
\textbf{Bounding $|\Lc|$:}
First, we bound $|\Lc|$, defined in~\eqref{eq:boundsizeLc} to be the number of item types learned by the algorithm after the exploration phase. To do so, we look into the two different cases $\ell\leq \thrjuu$, $\thrjuu< \ell\leq \qi/8$ and $\qi/8 < \ell\leq \qi$ separately next.

\textbf{Case I ($\ell\leq \thrjuu$):} When $\ell\leq \thrjuu$, according to~\eqref{eq:boundsizeLc}, $\Lc$ is the set of  item types in $\Mcc{2}$. Hence, $|\Lc|= \disi(\Mcc{2})$ where $\disi(\Mcc{2})$ is the number of items with distinct item types in $\Mcc{2}$ according to Definition~\ref{def:distinct}.
The items in $\Mcc{2}$ are chosen independent of any feedback from the algorithm. So their types are independently uniformly distributed on $[\qi]$. 
%
Hence, $\disi(\Mcc{2})$,  is  the number of non-empty bins after throwing $M_2=\big\lceil 2\min\{ \ell,\thrjuu\}\big\rceil$ balls  in  $\qi$ bins in 
  a balls and bins argument (Section~\ref{sec:BallsBins}). 
  %
We can show $M_2\leq  \frac{4}{15} \qi$ using 
\[M_2 \leq 2\thrjuu +1=2\log(N\qu^2) +1\leq 6\log N+1 \leq \qi/4\,,\] 
under the assumptions $\qu\leq N,\, 25 \log N \leq \qi$ and $\log N>4$. (Remark~\ref{Rem:ParamLargequApp}).


An application of Lemma~\ref{l:ballsbins} gives
$\Pr\big[\disi(\Mcc{2}) \leq M_2/2 \big] \leq \exp(-M_2/2)$.
%
 When $\ell\leq \thrjuu$, we have $\ell \leq \lceil 2\ell\rceil /2 =M_2/2$.
  Hence, when $\ell\leq \thrjuu$, we have
 \[
 \Pr\big[\disi(\Mcc{2}) \leq \ell \big] 
 \leq 
 \Pr\big[\disi(\Mcc{2}) \leq M_2/2 \big] \leq \exp(-M_2/2)
 \leq \exp(-\ell) \,.\]


\textbf{Case II ($\thrjuu< \ell\leq \qi/8$):} When $ \thrjuu <\ell$, according to~\eqref{eq:boundsizeLc}, $\Lc$  is the set of  item types in  $\Mcc{3}$ and $|\Lc|= \disi(\Mcc{3})$.
 Similar argument as above shows that $\disi(\Mcc{3})$ is the number of non-empty bins after throwing $M_3$ balls  in  $\qi$ bins in 
 a balls and bins argument (Section~\ref{sec:BallsBins}). 

 When  $\thrjuu< \ell\leq \qi/8$,  we have $M_3=\big\lceil 2\ell\big\rceil$ which gives $2\ell\leq M_3\leq 2\ell+1 \leq \frac{4}{15}\qi$ (since $\qi\geq 100\log N\geq 60$). An application of Lemma~\ref{l:ballsbins}  gives 
 
% \MK{here I'm assuming $\ell>7$. I can assume this either by bounding $\log N>7$ or $\ell>16 \log T > 7$ . Or I could say that $\qu \geq 9\log N > 36$ . and hence $\thrjuu> \log N + \log 36 \geq 4+5$.}
 \[
 \Pr\big[\disi(\Mcc{3}) \leq \ell \big] 
 \leq 
 \Pr\big[\disi(\Mcc{3}) \leq M_3/2 \big] \leq \exp(-M_3/2)
 \leq \exp(-\ell)\leq \frac{1}{N} \,,\] 
 where we used $\ell>\thrjuu \geq \log N$ in the last inequality.
 
 \textbf{Case III ($\qi/8< \ell\leq \qi$):}
In this regime, $|\Lc|= \disi(\Mcc{3})$ and  $M_3=\big\lceil \qi \log(N \qi)\big\rceil$. An Application of Lemma~\ref{l:ballsbins3} gives
 \[
 \Pr\big[\disi(\Mcc{3}) \leq \ell \big] 
 \leq 
  \Pr\big[\disi(\Mcc{3}) \leq \qi \big] 
  \leq \frac{1}{N}\,.\]
  
  Overall, the above three cases show that for any $\ell$, we have 
\begin{align}\label{eq:boundsizeLc}
\Pr\big[|\Lc| \leq \ell \big] \leq \frac{1}{N}+\exp(-\ell)\,.
\end{align} 



\textbf{Bounding $\ell_u$:}
For given user $u$, using definition of $\ell_u$ in~\eqref{eq:defLcu},
\[\ell_u = \sum_{\ti\in\Lc} \ident[\xi_{\tau_U(u),\ti} = +1]\,.\]
The set $\Lc$ is a function of types of items in $\Mcc{2}$ or $\Mcc{3}$. Hence, $\Lc$ is independent of elements of matrix $\Xi$ and type of users. In particular, $\xi_{\tau_U(u),\ti}$ is independent of the set $\Lc$ and is uniformly distributed on $\{-1,+1\}$. 
%the set $\Lc_u$ is a function of the type of user $u$ and the elements of the matrix $\Xi$, which are independent of the item types in $\Mcc{2}$ and $\Mcc{3}$. So, we know that each item type $\ti\in\Lc$ is equally probable to be liked or disliked by a given user $u$ independent of other item types in $\Lc$. 
%Hence, the size of set $\Lc_u$ has Binomial distribution with parameters $\Lc$ and $1/2$. In particular, given fixed set of item types $\Lc$, by applying Chernoff bound in 
Application of Lemma~\ref{l:Chernoff} shows that for any realization of the set $\Lc$ and any $u\in [N]$
\begin{align*}
\Pr \big[ \ell_u< |\Lc|/8\,\,\big| \, \Lc \big]
&
\leq
\exp\big( -|\Lc|/8 \big)\,.
\end{align*}
Using this bound and Equations~\eqref{eq:boundsizeLc}, we get
\begin{align*}
\Pr \big[ \ell_u< \ell/8 \big]
&\leq 
\Pr \big[ \ell_u< \ell/8 \,\,\big| \, |\Lc|> \ell \big]
+
\Pr \big[|\Lc|\leq \ell \big]
\\
&
\leq
2\exp\big( -\ell/8 \big) + \frac{1}{N}\,.  \qedhere
\end{align*}
\end{proof}

%%%%%%%%%%%%%
%%%%%%%%%%%%%
%
%\begin{claim}
%\label{c:Rbsubseteq}
%Condition on  event $\BB$, 
%\begin{align}\label{eq:Rbsubseteq}
%\bigcup_{\ti\in\Lc_u} \Rb(\ti)
%\subseteq 
%\R_u 
%\end{align}
%where $\Lc_u$ is defined in~\eqref{eq:defLcu}.
%\end{claim}
%
%\begin{proof}
%To see this, remember that event $\BB$ holds if and only if either no partitioning over the users happen (when $\ell\leq \thrjuu$) or the partitioning over the users is correct. 
%
%The set $\R_u$ in the algorithm is defined to be the union of sets $\S_{\ti}$'s such that the representative $\rep_{\ti}$ is liked by user $u$ or a user in the same partition as $u$. 
%Condition on $\BB$, this means 
%the set $\R_u$ is the union of sets $\S_{\ti}$'s such that the representative $\rep_{\ti}$ is liked by users of type $\tau_U(u)$. So, condition on $\BB$, 
%$\R_u = \bigcup_{\ti\in\Lc_u} \S_{\ti}$.
%
%Remark~\ref{rem:partitionionitemserror} shows that condition on the event $\BB$, the set of items $\S_{\ti}$ is a superset of items in $\Mcc{1}$ with type $\tau_I(i)$: $\S_{\ti}\subseteq\Rb(\tau_I(\rep_{\ti}))$.
%%
%The above two statements give Equation~\eqref{eq:Rbsubseteq}.
%\end{proof}



\subsubsection{Bounding $\Pr[|\R_u|< T]$ in the Regime Specified in Section~\ref{sec:UUparam}}
In Remark~\ref{remark:II-Upper-TrivialAlg}, we explain that 
 the bound we focus on the proof of Theorem~\ref{th:Item-upper} in the regime $\reg(T)\leq Y(T)$ and $Y(T)\leq T/2$ since achieving the regret bound $T/2$ is trivial. 
 In particular, in the regime  specified in Section~\ref{sec:UUparam}, we are bounding regret for time horizon such that $T>\thrjuu$. For the horizon $T\leq\thrjuu$, we use the trivial bound $\reg(T)\leq T/2$. 
\begin{lemma}\label{l:ju-exp-R-u2}
In the regime specified in Section~\ref{sec:UUparam}, for any user $u\in[N],$
\[\Pr[|\R_u|\leq T] \leq  \frac{3}{N}\,.\]
And, 
\[\Exp{(T- |\R_u |)_+}\leq \frac{3T}{N}\,.\]
\end{lemma}

\begin{proof}

%Assume $\qu < 9 \log(N\qi)$, $T> \thrjuu$ and $M_3 = 16T$. Also, assume $\qi\geq 32 \thrjuu$ (which holds according to the discussion in Section~\ref{ss:pref}).

In this regime, we defined $\ell=T> \thrjuu$ and $\Mcc{1}=\varnothing$. Hence, the sets $\R_u$ (defined in Line~\ref{Line:DefRu2} of Algorithm \textsc{Explore}) are subset of set $\Mcc{3}$. 
In particular, for any $u\in [N]$, the set $\R_u$ is the items in $\Mcc{3}$ which are liked by any user in the same partition as $u$ after partitioning the  users in Line~\ref{line:user-partiotion}. 

According to Remark~\ref{rem:partitionionuserserror}, the users of the same type always end up in the same group after partitioning the users. So, 
\begin{align}
\label{eq:JU-BoundRuSubset}
\{i\in\Mcc{3}: \xi_{\tau_U(u), \tau_I(i)}=+1\}  \subseteq \R_u\,.
\end{align}
The above statement holds with equality for all $u$ when the partitioning made by the algorithm over users coincide with the partitioning of users according to their types.


Similar to~\eqref{e:defLc} and~\eqref{eq:defLcu}, we define
\begin{align*}
\Lc
& =
\big\{ \ti\in[\qi]:
\exists i\in \Mcc{3}, \tau_I(i)=\ti
 \big\}, 
 \\
 \Lc_u
&=
\big\{
\ti\in \Lc: \xi_{\tau_U(u), \ti} = +1
\big\},
\quad 
\ell_u = \big| \Lc_u\big|
\,,
\end{align*}
to be the set of item types appearing in $\Mcc{3}$ and the  set of item types appearing in $\Mcc{3}$ which are liked by user $u$ respectively. In particular, $|\Lc|= \disi(\Mcc{3})$.
 Since the items in $\Mcc{3}$ are chosen independently of the feedback, their types are uniform on $[\qi]$. 
 Hence, $ \disi(\Mcc{3})$ can be derived by using a balls and bins argument. In particular, $ \disi(\Mcc{3})$ is the number of non-empty bins after throwing $M_3$ balls into $\qi$ bins. Note that since $M_3 = 64T \geq 16\thrjuu$ and $\qi> 100\log N > 32\thrjuu$, we have  $ \disi(\Mcc{3})\geq 8 \thrjuu$ with probability at least $1-\exp(-8 \thrjuu)$ and
 $\Pr\big[\, |\Lc| < 8 \thrjuu \big] \leq \exp(-8 \thrjuu)$.
 
Also, for given user $u$, using definition of $\ell_u$,
\[\ell_u = \sum_{\ti\in\Lc} \ident[\xi_{\tau_U(u),\ti} = +1]\,.\]
The set $\Lc$ is a function of types of items in  $\Mcc{3}$. Hence, $\Lc$ is independent of elements of matrix $\Xi$ and type of users. In particular, $\xi_{\tau_U(u),\ti}$ is independent of the set $\Lc$ and is uniformly distributed on $\{-1,+1\}$. 
Application of Lemma~\ref{l:Chernoff} shows that for any realization of the set $\Lc$ and any $u\in [N]$
\begin{align*}
\Pr \big[ \ell_u< |\Lc|/8 \,\,\big| \, \Lc \big]
&
\leq
\exp\big( -|\Lc|/8 \big)\,.
\end{align*}
The total probability lemma gives
\begin{align*}
\Pr \big[ \ell_u/|\Lc|< 1/8 \big]
& \leq 
\Pr \big[ \ell_u< |\Lc|/8,\, |\Lc|\geq 8\thrjuu \big]
+\Pr \big[  |\Lc|<8 \thrjuu \big]
\\
&
\leq
\exp\big( -\thrjuu \big) + \exp(-8\thrjuu)\leq 2\exp(-\thrjuu)\,.
\end{align*}
Using~\eqref{eq:JU-BoundRuSubset}
\begin{align*}
|\R_u| 
&\geq
\sum_{i\in\Mcc{3}} \ident[\tau_I(i)\in\Lc_u]
\end{align*}
For any $i\in\Mcc{3}$, we have $\Pr[\tau_I(i)\in\Lc_u] = \frac{\ell_u}{|\Lc|}$.
Also, the variables $\ident[\tau_I(i)\in\Lc_u]$ are independent for all $i\in\Mcc{3}$.
Hence, when $\ell_u/|\Lc|\geq 1/8$, $|\R_u| $ stochastically dominates a Binomial random variable with parameters $(M_3, 1/8)$ with $M_3=32T$. Another application of Chernoff bound gives
\begin{align*}
\Pr [\R_u \leq T] 
& \leq 
\Pr [\R_u \leq T\, \big|\,  \ell_u/|\Lc|\geq 1/8 ]   + \Pr \big[ \ell_u/|\Lc|< 1/8 \big]
\\
& \leq 
\exp(-T) + 2\exp(-\thrjuu)
\leq 
3\exp(-\thrjuu)
< \frac{3}{N}\,.\qedhere
\end{align*}
\end{proof}
%%%%%%%%%%
%%%%%%%%%%%
%%%%%%%%%%%
%%%%%%%%%%%
%%%%%%%%%%
\subsection{Combining the bounds to get the upper bound}
\label{sec:UBcomb}
\subsubsection{Combining all the boundsin the regime specified in Section~\ref{sec:IJparam}}

We Plug in Equations~\eqref{eq:ju-bound-A1-ell-small},
 ~\eqref{eq:ju-bound-A1-ell-large},
 ~\eqref{eq:ju-bound-A2},
 \eqref{eq:ju-bound-A3},
 \eqref{eq:ju-bound-A4} and $\Asf{5} = 0$ into Equation~\eqref{eq:ju-reg-decomp}. 
%%
%\begin{align}
%\label{eq:ParamChoice2ell}
%\ell&=\begin{cases} 
%8\log T+ \sqrt{\frac{10\qi\thrjiu}{N}T}
%\quad  &\text{ if }\,\,
%T\leq 
%T_1
%\,,
%\\ 
%\sqrt{15\frac{\thrjiu \qi T}{\qu}} + 8\thrjuu, 
%& \text{ if }
% T_1
%<T 
%\leq  T_2
%\\
%\qi, 
%& \text{ if }  T_2< T\,.
%\end{cases}
%\end{align}
%
%
%
%\begin{align}
%\label{eq:ParamChoice2ell}
%\ell&=\begin{cases} 
%8\log T+ \sqrt{\frac{10\qi\thrjiu}{N}T}
%\quad  &\text{ if }\,\,
%8\log T+ \sqrt{\frac{10\qi\thrjiu}{N}T} 
%\leq \thrjuu
%\,,
%\\ 
%\sqrt{10\frac{\thrjiu \qi T}{\qu}} + 8\thrjuu, 
%& \text{ if }
%8\log T+ \sqrt{\frac{10\qi\thrjiu}{N}T}
%>\thrjuu
%\quad \text{and }
%\sqrt{10\frac{\thrjiu \qi T}{\qu}} + 8\thrjuu \leq \qi/2
%\\
%\qi, 
%& \text{ if } 
%8\log T+ \sqrt{\frac{10\qi\thrjiu}{N}T}>\thrjuu
%\quad \text{and }
%\sqrt{10\frac{\thrjiu \qi T}{\qu}} + 8\thrjuu >\qi/2
%\,.
%\end{cases}
%\end{align} 
% 
% %%%%%
%
%\begin{align}
%M_1 & = \left\lceil 15\frac{\qi}{\ell}T\right\rceil
%,\quad 
%M_2 =
%\big\lceil 2\min\{ \ell,\thrjuu\}\big\rceil,
% \quad \text{ and }\quad
%%\\&
% M_3
%=
%\begin{cases}
%\lceil 2\ell \rceil, 
%&\text{ if } \ell\leq \frac{\qi}{2}\,,
%\\
%\lceil \qi \log(N\qi)\rceil,
%& \text{ if } \ell >\frac{\qi}{2}
% \end{cases}
%\label{eq:ParamChoice2}
%\end{align}


\paragraph{ When $\ell\leq \thrjuu$:} First, we upper bound regret when the parameter $\ell$ is chosen such that $\ell\leq \thrjuu$. 
According to~\eqref{eq:ParamChoice2ell}, this holds when 
$T\leq
\min\big\{e^{\thrjuu/16}
, \,\,
\frac{N\thrjuu^2}{15\qi\thrjiu}\big\}$.
 Using Equations~\eqref{eq:ju-bound-A1-ell-small},
 ~\eqref{eq:ju-bound-A2},~\eqref{eq:ju-bound-A3},
 and~\eqref{eq:ju-bound-A4}, we get
\begin{align*}
N \reg(T) & \leq 
M_1 \thrjiu +M_2 N+ N 
+
N\log T + 2TNe^{-\ell/16} + 3T
+ 3M_1
\\
&{\leq}
 20 \frac{\qi}{\ell} \thrjiu T+ 2\ell N + N\log\log T+ 4N\,.
\end{align*}
The last inequality is 
based on the choice of parameters defined in~\eqref{eq:ParamChoice2} when $\qu \geq 9\log(N\qi)$ and parameter $\ell$ is chosen so that $\ell\leq \thrjiu$. In this regime, the following holds:
$M_2 = \lceil 2\ell\rceil$, $M_1=\lceil 15\frac{\qi}{\ell}T\rceil$ and $\ell$ is chosen so that $\ell\geq 16 \log T$. Hence $TN e^{-\ell/16}\leq N$.
Also, since $N>30$, we have $\thrjiu \geq 3$ which gives 
$M_1(\thrjiu+3)+ 3T\leq  20\frac{\qi}{\ell}\thrjiu T $ using $T\geq1$.

According to~\eqref{eq:ParamChoice2ell}, the parameter $\ell$ is chosen to be  \[\ell=\max\big\{16\log T, \sqrt{\frac{10\qi\thrjiu}{N}T}\big\}\] in this regime, which gives
\begin{align*}
\reg(T) & \leq 
4\ell + \log\log T + 4
\notag
\\
&\leq 
\max\{70\log T, \,\,14\sqrt{\frac{\qi\thrjiu}{N}T}\}\,.
\end{align*} 
%when $T\leq
%\min\big\{e^{\thrjuu/16}
%, \,\,
%\frac{N\thrjuu^2}{15\qi\thrjiu}\big\}$ (or $\ell\leq \thrjiu$). 
 %%%%%
 
\paragraph{ When $\ell> \thrjuu$:} Next, we upper bound regret when the parameter $\ell$ is chosen such that $\ell>  \thrjuu$. 
 Using Equations~\eqref{eq:ju-bound-A1-ell-large},~\eqref{eq:ju-bound-A2},~\eqref{eq:ju-bound-A3},~\eqref{eq:ju-bound-A4}, we get


\begin{align*}
N \reg(T) 
& \leq 
M_1\thrjiu + (M_2 +2)N + \qu M_3 
+
N\log \log T + 2TNe^{-\ell/16} + 3T
+ 3M_1
\end{align*}

\begin{align*}
 (M_2 +2 + \log \log T )N 
 &\leq 
  (2\thrjuu + 3 + \log \log T )N 
\\
\qu M_3
&\leq 
\begin{cases}
2\ell \qu + N, \quad \text{ when } \ell<\qi/2
\\
2\qi \qu \log(N\qi)+ N, \quad \text{ when }  \ell \geq\qi/2
\end{cases}
\\
M_1(\thrjiu  + 3 ) +2TNe^{-\ell/16} + 3T 
&\leq (15 \frac{\qi}{\ell}T + 1) (\thrjiu  + 3 ) +5T
\leq 
\frac{5}{4} \thrjiu(15 \frac{\qi}{\ell}T + 1) +5T
\\&\leq 
\frac{5}{4} \thrjiu (16 \frac{\qi}{\ell}T ) +5T 
\leq 20 \frac{\qi}{\ell}T \thrjiu+5T 
\leq 21 \frac{\qi}{\ell}T \thrjiu
\end{align*}

\paragraph{ When $ \thrjuu < \ell \leq \qi/2$:}

\begin{align*}
N \reg(T) 
& \leq 
  (2\thrjuu + 3 + \log \log T )N +
  2\ell \qu + N +
21 \frac{\qi}{\ell}T \thrjiu 
\\ & \leq 
  (2\thrjuu + 4+ \log \log T )N +
 2\qu \sqrt{10\frac{\thrjiu \qi T}{\qu}} + 32\qu\thrjuu +
21 \frac{\qi}{\ell}T \thrjiu 
%\\ & \leq 
%  (2\thrjuu + 4+ \log \log T )N   + 32\qu\thrjuu +
% \sqrt{40\thrjiu \qi \qu T}+
%\sqrt{ \frac{441}{10}\thrjiu \qi \qu T}
\\ & \leq 
  (34\thrjuu + 4+ \log \log T )N   + 
 13\sqrt{\thrjiu \qi \qu T}
 \end{align*}


\paragraph{ When $ \qi/2< \ell$:}


\begin{align*}
N \reg(T) 
& \leq 
  (2\thrjuu + 3 + \log \log T )N +
  2\qi \qu \log(N\qi) + N +
21 \frac{\qi}{\ell}T \thrjiu 
\\
& \leq 
  (2\thrjuu + 4 + \log \log T )N +
  2\qi \qu \log(N\qi) + 
21 T \thrjiu   
 \end{align*} 
 
 \MK{Old from here on}
 
\begin{align*}
&N \reg(T) 
\\& \leq 
M_1\thrjiu + (M_2 +2)N + \qu M_3 
+
N\log \log T + 2TNe^{-\ell/16} + 3T
+ 3M_1
\\
&\stackrel{(a)}{\leq}
 30 \frac{\qi}{\ell} \thrjiu T+ 2\thrjiu N + 5N+ N\log T+ 3T +\qu \min\{2\ell, \qi \}\log(N\qi) 
 \\
&\stackrel{(b)}{\leq}
 31 \frac{\qi}{\ell} \thrjiu T+ 3\thrjuu N + N\log T+\qu \min\{2\ell, \qi \}\log(N\qi) \,.
\end{align*}




The inequality (a) is 
based on the choice of parameters defined in Section~\ref{sec:IJparam} when $\ell> \thrjiu$. 

 In this regime, the following holds:
$M_1=\lceil 15\frac{\qi}{\ell}T\rceil$,
$M_2 =  \lceil 2\thrjuu\rceil$, 
$M_3=\big\lceil \min\{2\ell, \qi \}\log(N\qi)\big\rceil$ and $\ell$ is chosen so that $\ell\geq 16 \log T$. 

~\eqref{eq:ParamChoice2} when $\qu \geq 9\log(N\qi)$ and parameter $\ell$ is chosen so that $\ell> \thrjiu$. In this regime, the following holds:
$M_1=\lceil 15\frac{\qi}{\ell}T\rceil$,
$M_2 =  \lceil 2\thrjuu\rceil$, 
$M_3=\big\lceil \min\{2\ell, \qi \}\log(N\qi)\big\rceil$ and $\ell$ is chosen so that $\ell\geq 16 \log T$. Hence $2TN e^{-\ell/16}\leq 2N$.
Also, since $N>30$, we have $\thrjiu \geq 3$ which gives 
$M_1(\thrjiu+3) + 2T \leq 2M_1\thrjiu+2T\leq 31\frac{\qi}{\ell}\thrjiu T$. 
We also have $\qu M_3 \leq \qu \min\{2\ell, \qi \}\log(N\qi) + N$.
Inequality (b) uses $\thrjuu\geq 3$ to bound $2\thrjuu + 5\leq 3\thrjuu$.



The inequality (a) is 
based on the choice of parameters defined in~\eqref{eq:ParamChoice2} when $\qu \geq 9\log(N\qi)$ and parameter $\ell$ is chosen so that $\ell> \thrjiu$. In this regime, the following holds:
$M_1=\lceil 15\frac{\qi}{\ell}T\rceil$,
$M_2 =  \lceil 2\thrjuu\rceil$, 
$M_3=\big\lceil \min\{2\ell, \qi \}\log(N\qi)\big\rceil$ and $\ell$ is chosen so that $\ell\geq 16 \log T$. Hence $2TN e^{-\ell/16}\leq 2N$.
Also, since $N>30$, we have $\thrjiu \geq 3$ which gives 
$M_1(\thrjiu+3) + 2T \leq 2M_1\thrjiu+2T\leq 31\frac{\qi}{\ell}\thrjiu T$. 
We also have $\qu M_3 \leq \qu \min\{2\ell, \qi \}\log(N\qi) + N$.
Inequality (b) uses $\thrjuu\geq 3$ to bound $2\thrjuu + 5\leq 3\thrjuu$.

According to~\eqref{eq:ParamChoice2ell}, we have $\ell = \sqrt{15 \thrjiu \qi T/\qu}$ when $\min\big\{e^{\thrjuu/16} , \,\,
\frac{N\thrjuu^2}{15\qi\thrjiu}\big\}
<T 
\leq  \qi \qu/(15\thrjiu)$ (or $\thrjuu<\ell\leq \qi/2$) and we have $\ell = \qi$ when $T>\qi \qu/(15\thrjiu)$.

Hence, when $\min\big\{e^{\thrjuu/16} , \,\,
\frac{N\thrjuu^2}{15\qi\thrjiu}\big\}
<T 
\leq  \qi \qu/(15\thrjiu)$, we have 
\begin{align*}
\reg(T) & \leq 
3\thrjuu + \log T + 16 \frac{\log^2(N\qi)}{N} \sqrt{\qi \qu T}\,,
\end{align*}
and when $T>\qi \qu/(15\thrjiu)$, we have 
\begin{align*}
\reg(T) & \leq 
3\thrjuu + \log T + 2\frac{\qi \qu}{N} \log(N\qi) + 31 \frac{\thrjiu}{N}T\,,
\end{align*}
which is the asymptotic slope of the algorithm.

So, overall, when $\qu \geq 9\log(N\qi)$, we have 
\begin{align*}
&\reg(T) 
\\& \leq 
\begin{cases}
 17\max\Big\{\log T, \sqrt{\frac{\qi\thrjiu}{16 N}T}\Big\}\,,
 &
 \text{if } T\leq
T_0
\\\\
3\thrjuu + \log T + 16 \frac{\log^2(N\qi)}{N} \sqrt{\qi \qu T}\,,
 &
 \text{if } 
T_0
< T \leq \frac{\qi\qu}{15\thrjiu}
\\\\
3\thrjuu + \log T +2\frac{\qi \qu}{N} \log(N\qi) + 31 \frac{\thrjiu}{N}T\,,
 &
 \text{if } 
\frac{\qi\qu}{15\thrjiu} < T\,.
\end{cases}
\end{align*}  
 

%%%%%%%%%%%%
%%%%%%%%%%%%
%%%%%%%%%%%%
\subsubsection{Combining all the bounds in the regime specified in Section~\ref{sec:UUparam}}
We use the bound $\reg(T)\leq T/2$ 
for $T\leq  \thrjuu$
when $\qu < 9\log(N\qi)$.
For $T>\thrjuu$, according to~\eqref{eq:ParamChoice1}, we have $\ell=\thrjuu+1$. 
We use Equations~\eqref{eq:ju-bound-A1-ell-large},~\eqref{eq:ju-bound-A2-UU},~\eqref{eq:ju-bound-A3},
 and~\eqref{eq:ju-bound-A4} to get

For $T> \thrjuu$,
\begin{align*}
N \reg(T) & \leq 
M_1 \thrjiu +M_2 N+ 2N 
+
\qu M_3+ 4T
+ 3M_1
\\
&\overset{(a)}{\leq}
2\thrjuu N+ 3N 
+
10 \qu T + 4T\,.
\end{align*}
According to the choice of parameters in~\eqref{eq:ParamChoice1},  $M_1 = 0, M_2 = \lceil 2\thrjuu\rceil$ and $M_3 = 16T$. So, when $\qu<9\log(N\qi)$, 
\begin{align*}
 \reg(T) & \leq 
 \begin{cases}
T/2, 
 &\quad \text{ if } T\leq \thrjuu,
 \\
3 + 2\thrjuu
+
11 \frac{\qu}{N} T
 &\quad \text{ if } T> \thrjuu\,.
 \end{cases}
\end{align*}











==> MKdefRS.tex <==
%\usepackage{fullpage}
%% Packages
\RequirePackage{amsthm,amsmath,amsfonts,amssymb}
\RequirePackage[numbers]{natbib}
%\RequirePackage[authoryear]{natbib}%% uncomment this for author-year citations
% \RequirePackage[colorlinks,citecolor=blue,urlcolor=blue,]{hyperref}
% \usepackage[%dvips,
%             CJKbookmarks=true,
%             bookmarksnumbered=true,
%             bookmarksopen=true,
%             colorlinks=true,
%             citecolor=blue,
%             linkcolor=blue,
%             anchorcolor=red,
%             urlcolor=blue,
%             ]{hyperref}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage{sidecap}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{subfigure}
\usepackage{caption}
%\usepackage{subcaption}


\usepackage{fixltx2e}

\newcommand{\MK}[1]{\textcolor{blue}{Mina: #1}}
\newcommand{\guy}[1]{{\texttt{\textcolor{red}{Guy: #1}}}}

%\newcommand{\MK}[1]{}
%\newcommand{\guy}[1]{}

% \startlocaldefs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%% Uncomment next line to change            %%
%% the type of equation numbering           %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\numberwithin{equation}{section}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%% For Axiom, Claim, Corollary, Hypothesis, %%
%% Lemma, Theorem, Proposition              %%
%% use \theoremstyle{plain}                 %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{axiom}{Axiom}
\newtheorem{claim}[axiom]{Claim}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corr}[theorem]{Corollary}
\newtheorem{prop}[theorem]{Proposition}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark} %Mina: I added this myself. Does not look great.w
\newtheorem*{example}{Example}
\newtheorem*{fact}{Fact}


\newtheorem{lemmaalt}{Lemma}[theorem]
\usepackage{multirow}


%%To repeat the theorems and lemmas in the appendix with the same numering as in the body of the paper, we introduce a new theoremstyle.
\newtheoremstyle{TheoremNum}
        {\topsep}{\topsep}              %%% space between body and thm
        {\itshape}                      %%% Thm body font
        {}                              %%% Indent amount (empty = no indent)
        {\bfseries}                     %%% Thm head font
        {.}                             %%% Punctuation after thm head
        { }                             %%% Space after thm head
        {\thmname{#1}\thmnote{ \bfseries #3}}%%% Thm head spec
\theoremstyle{TheoremNum}
\newtheorem{thmn}{Theorem}
\newtheorem{lemman}{Lemma}
\newtheorem{propn}{Proposition}
\newtheorem{corn}{Corollary}



% % New environment
% \newenvironment{lemmap}[1]{
%   \renewcommand\thelemmaalt{#1}
%   \lemmaalt
% }{\endlemmaalt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Please put your definitions here:        %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\usepackage{dsfont}
\usepackage[T1]{fontenc}
\usepackage{color}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage{amssymb,amsmath,amsfonts}
\usepackage{mathtools} 
\usepackage{graphicx}
%\usepackage{graphicx,algorithm}
%\usepackage[noend]{algpseudocode}
\usepackage{hyperref}
\usepackage{amsbsy}
\usepackage{dsfont}
\usepackage{xcolor}


\RequirePackage{graphicx}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}


\usepackage[symbol]{footmisc}

\newcounter{daggerfootnote}
\newcommand*{\daggerfootnote}[1]{%
    \setcounter{daggerfootnote}{\value{footnote}}%

% \renewcommand*{\thefootnote}{\fnsymbol{footnote}}%
%    \footnote[2]{#1}%
%    \setcounter{footnote}{\value{daggerfootnote}}%
   \renewcommand*{\footnote}{\arabic{footnote}}%
    }
    \renewcommand{\thefootnote}{\arabic{footnote}}
    %%

%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\unif}{\mathsf{Unif}}


\newcommand{\ISstrong}{\mathcal{I}_{\mathsf{strong}}}
\newcommand{\ISweak}{\mathcal{I}_{\mathsf{weak}}}
\newcommand{\IStotal}{\mathcal{I}_{\mathsf{total}}}

\newcommand{\Istrong}{I_{\mathsf{strong}}}
\newcommand{\Iweak}{I_{\mathsf{weak}}}
\newcommand{\Itotal}{I_{\mathsf{total}}}



\renewcommand{\ell}{{\mathsf{k}_\mathrm{rep}}}
\renewcommand{\k}{\mathsf{k}}
\newcommand{\kI}{\mathsf{k}_\mathrm{Item}}
\newcommand{\kH}{\mathsf{k}_\mathrm{Hybrid}}
\newcommand{\kA}{\mathsf{k}_\mathrm{Asymp}}

\renewcommand{\Pr}{\mathbb{P}}

\newcommand{\minUser}{\pi_*}
\newcommand{\NonEmptyUser}{\mu}

\newcommand{\recsys}{\textsc{RecommendationSystem}}

\newcommand{\quadand}{\quad\text{and}\quad}
\newcommand{\ident}{\mathds{1}}
\renewcommand{\H}{\mathcal{H}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\St}{\widetilde{\mathcal{S}}}
\newcommand{\R}{\mathcal{R}}
\newcommand{\Tcal}{\mathcal{T}}

\newcommand{\Itypes}{\mathcal{T}}

\newcommand{\Lcrep}{\mathcal{T}_{\mathrm{rep}}^{u+}}
\newcommand{\ItypesR}{\mathcal{T}_{\mathrm{rep}}}

\newcommand{\Rb}{\overline{\R}}
\newcommand{\Rt}{\widetilde{\R}}
\newcommand{\M}{\mathbb{M}}

\newcommand{\BB}{\mathcal{B}}
\newcommand{\BBil}[3]{\BB^{{#3}}_{{#1},\tau_I({#2})}}
\newcommand{\BBul}[3]{\BB^{{#3}}_{\tau_U({#1}),{#2}}}

\newcommand{\CC}{\mathcal{C}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\EEb}{\bar{\mathcal{E}}}

\newcommand{\EEt}{\widetilde{\mathcal{E}}}

\newcommand{\USweak}{\mathcal{U}_\textsf{weak}}
\newcommand{\Uweak}{{U}_\textsf{weak}}

%\newcommand{\Mc}{\mathcal{M}} %the set of items to be partitioned in i-i
\newcommand{\Mcc}[1]{\mathcal{M}_{#1}} 
\newcommand{\IsetU}{\mathcal{I}_{\mathrm{usr}}}
\newcommand{\IsetR}{\mathcal{I}_{\mathrm{rep}}}
\newcommand{\IsetE}{\mathcal{I}_{\mathrm{exp}}}

\newcommand{\IU}{{I}_{\mathrm{usr}}}
\newcommand{\IR}{{I}_{\mathrm{rep}}}
\newcommand{\IE}{{I}_{\mathrm{exp}}}

\newcommand{\IRA}{{I}^{*,A}_{\mathrm{rep}}}
\newcommand{\IRB}{{I}^{*,B}_{\mathrm{rep}}}

\newcommand{\IRAi}{{I}^{*,1}_{\mathrm{rep}}}
\newcommand{\IRAii}{{I}^{*,2}_{\mathrm{rep}}}
\newcommand{\IRAiii}{{I}^{*,3}_{\mathrm{rep}}}
\newcommand{\IRAiv}{{I}^{*,4}_{\mathrm{rep}}}
\newcommand{\IRAv}{{I}^{*,5}_{\mathrm{rep}}}


%the set of items to be partitioned in i-i
\newcommand{\Fc}{\mathcal{F}} %the set of items to be partitioned in i-i
\newcommand{\Gc}{\mathcal{G}} %the set of items to be partitioned in i-i
\newcommand{\Nc}{\mathcal{N}} %the set of items to be partitioned in i-i


\newcommand{\Lc}{\mathcal{L}}
\newcommand{\Pc}{\mathcal{P}}%Partition of users 
\newcommand{\Uc}{\mathcal{U}}

\newcommand{\balls}{\mathsf{g}}

\newcommand{\EWtype}{\mathsf{E}_{W}}
\newcommand{\EFGtype}{\mathsf{E}_{FG}}

%\newcommand{\B}[0]{\mathcal{F}}

\newcommand{\qu}{\texttt{q}_U}
%number of user types
\newcommand{\tu}{w}
%counter for user type?

\newcommand{\qi}{\texttt{q}_I}
%number of item types
\newcommand{\ti}{\textit{j}} %counter for item type?

\newcommand{\tauh}{\widehat{\tau}}

\newcommand{\disi}{\Phi_{\texttt{I}} }%number of distinct types in a set of items
\newcommand{\disu}{\Phi_{\texttt{U}} }%number of distinct types in a set of users

\newcommand{\rep}{\textbf{\textmd{j}}} %representative of item type. 

\newcommand{\eps}{\epsilon}
\newcommand{\calS}{\mathcal{S}}

\newcommand{\reg}{\mathtt{regret}}
\newcommand{\Rtt}{\mathtt{R}}

\newcommand{\TupI}{\mathsf{T}_{Item}}
\newcommand{\TupU}{\mathsf{T}_{Hybrid}}

\newcommand{\rated}{\mathsf{rated}}
\newcommand{\ratedtype}{\mathsf{ratedcluster}}

\newcommand{\tIni}{\tau_I^{\sim i}}
\newcommand{\tUnu}{\tau_U^{\sim u}}
\newcommand{\tI}{\tau_I}
\newcommand{\tU}{\tau_U}

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\E}[2]{E_{#1,#2}}

\newcommand{\Tt}{\mathsf{T}}

\newcommand{\bw}{\mathbf{w}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bx}{\mathbf{x}}

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\TintCold}{\mathtt{T}_{\mathsf{Cold}}}
\newcommand{\TintItem}{\mathtt{T}_{\mathsf{Item}}}
\newcommand{\TintUser}{\mathtt{T}_{\mathsf{User}}}
\newcommand{\TintHyb}{\mathtt{T}_{\mathsf{Hybrid}}}
\newcommand{\TintAsym}{\mathtt{T}_{\mathsf{Asymptotic}}}
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\rgl}{\Omega}


\newcommand{\tiu}{\mathsf{r}_{I}}
\newcommand{\tuu}{\mathsf{r}_{U}}

\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\liked}[2]{{d^+_{#1}(#2)}} %The number of item types rated and likes by certain user type in the lower bound
\newcommand{\disliked}[2]{{d^-_{#1}(#2)}} %The number of item types rated and likes by certain user type in the lower bound


\newcommand{\til}{\mathsf{s}_{I}}
\newcommand{\tul}{\mathsf{s}_{U}}
\newcommand{\thril}{\mathsf{s}}

\newcommand{\BBjil}[3]{\mathcal{K}^{{#3}}_{{#1},\tau_I({#2})}}
\newcommand{\BBjul}[3]{\mathcal{K}^{{#3}}_{\tau_U({#1}),{#2}}}
\newcommand{\BBjjl}[3]{\mathcal{K}^{{#3}}_{\tau_U({#1}),\tau_I({#2})}}
\newcommand{\good}{\mathsf{good}}
\newcommand{\bad}{\mathsf{bad}}

\newcommand{\Wc}{\mathcal{W}}

\newcommand{\Bsf}[1]{\mathcal{B}^{#1}}
\newcommand{\Asf}[1]{\mathtt{A{#1}}}

%\newcommand{\hist}[1]{\mathsf{H}{#1}}
\newcommand{\hist}[1]{\mathsf{B_{#1}}}
\newcommand{\histE}[1]{\mathfrak{B}_{#1}}

%ep}{\rotatebox[origin=c]{90}{$\models$}}
\newcommand{\w}{\mathcal{W}}
\newcommand{\bvec}{\mathbf{b}}

\newcommand{\Exp}[1]{\mathbb{E}\left[ #1 \right]}
\newcommand{\thr}{\mathsf{r}}
%\newcommand{\thruu}{\mathsf{r}_{u,u}} %threshold for user-user-upper bound

%\newcommand{\thrul}{\mathsf{r}_{u,l}}
%threshold for user-user-lower bound

%\newcommand{\thriu}{\mathsf{r}_{i,u}}
%threshold for item-item-upper bound
%threshold for item-item-lower bound


\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\iuerr}{\mathsf{Err}}


%To be removed in thesis:
\newcommand{\Ex}{\mathbb{E}}
\newcommand{\EE}{\mathcal{E}}

\renewcommand{\Pr}{\mathbb{P}}

\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}



\usepackage{enumitem}

\newcommand{\Tu}{T_{\small{\textsc{Exp}}}}

\newcommand{\ind}[1]{\mathds{1}{\{#1\}}}
\newcommand{\indB}[1]{\mathds{1}{\B\{#1\B\}}}

\newcommand{\IRs}{\IR^*}
\newcommand{\IUs}{\IU^*}
\newcommand{\IEs}{\IE^*}

\newcommand{\ks}{\mathsf{k}^*_\mathrm{rep}}

\newcommand{\f}{\frac}
\newcommand{\B}{\Big}

\renewcommand{\b}{\big}

\newcommand{\inv}{^{-1}}

\newcommand{\rg}[1]{\mathsf{reg}_{#1}}

\newcommand{\bin}{\mathsf{Bin}}

%\newcommand{\sumTN}{\sum_{\substack{t\in [T]\\ u\in [N]}}}
\newcommand{\sumTN}{\sum_{t\in [T], u\in [N]}}


\newenvironment{oneshot}[1]{\@begintheorem{#1}{\unskip}}{\@endtheorem}
%%this is how you use this:
% \begin{oneshot}{Theorem~\ref{Th:wet}}
% Iberian precipitation primarily hits the flatlands.
% \end{oneshot}



% Alternative Assumption!

%%this is how you use it:
% \begin{assumption}\label{second}
% Second one
% \end{assumption}

% \begin{assumptionp}{\ref{second}$'$}
% Second one alternative
% \end{assumptionp}

% \begin{assumptionp}{\ref*{second}$'$}
% Second one alternative with no hyper link
% \end{assumptionp}

% \begin{assumptionp}{C}
% Custom One
% \end{assumptionp}

==> algorithmold.tex <==

\subsection{Choice of parameters}\label{sss:params}
We now specify the values of parameters  used in the algorithm pseudocode in this subsection. Let 
\begin{align}
\label{eq:defthrjuu}
\thrjuu &=
\log (N\qu^2), \quad\text{ and } \quad
\thrjiu = 
\big\lceil 2\log(N\qi)\big\rceil\,.
\end{align}

%%%%%
%%%%%
\subsubsection{User-User Regime} 
\label{sec:UUparam}
\begin{enumerate}
\item 
When $\qu<9\log (N\qi) $,   and $\max\big\{  \thrjuu, \, \frac{N\thrjuu^2}{\qi \thrjiu}  \big\} < T$.

\item 
When $\qu \geq 9\log (N\qi) $, and 
  $\max\big\{  \thrjuu, \, \frac{N\thrjuu^2}{\qi \thrjiu}  \big\} 
  < T\leq 
  \qi \frac{\thrjiu}{\qu}$.
%  \MK{There are constants missing in $ \frac{N\thrjuu^2}{\qi \thrjiu}$  and $  \qi \frac{\thrjiu}{\qu}$. As far as I have seen, the proof of the lemmas do not change. Maybe even the constants here don't really matter?!}
\end{enumerate}
%%%%%
\begin{align}
\label{eq:ParamChoice1}
\ell & = T,\quad 
M_1  = 0,\quad M_2 =\lceil 2\thrjuu\rceil, 
%\\&
\quad \text{ and }\quad M_3=27T\,.
\end{align}


%%%%%
%%%%%
\subsubsection{Hybrid and Item-Item regime}
\label{sec:IJparam}
When 
either  $T\leq  \max\big\{  1, \, \frac{N\thrjuu}{\qi \thrjiu}  \big\} \, \thrjuu$ or   $\qu \geq 9\log (N\qi) $ and  $T>\qi \frac{\thrjiu}{\qu}$.  % \MK{There are constants missing in $ \frac{N\thrjuu^2}{\qi \thrjiu}$  and $  \qi \frac{\thrjiu}{\qu}$. As far as I have seen, the proof of the lemmas do not change. Maybe even the constants here don't really matter?!}

In this regime, we define the parameter $\ell$ as follows: 


\begin{align}
\label{eq:ParamChoice2ell}
\ell&=\begin{cases} 
8\log T+ 3\sqrt{\frac{\qi\thrjiu}{N}T}
\quad  &\text{ if }\,\,
8\log T+ 3\sqrt{\frac{\qi\thrjiu}{N}T} 
\leq \thrjuu
\,,
\\ 
8\thrjuu + 3\sqrt{\frac{\thrjiu \qi T}{\qu}}, 
& \text{ if }
8\log T+ 3\sqrt{\frac{\qi\thrjiu}{N}T}
>\thrjuu
\quad \text{and }
8\thrjuu  + 3\sqrt{\frac{\thrjiu \qi T}{\qu}} \leq \frac{\qi}{3}
\\
\qi, 
& \text{ if } 
8\log T+3 \sqrt{\frac{\qi\thrjiu}{N}T}>\thrjuu
\quad \text{and }
8\thrjuu  + 3\sqrt{\frac{\thrjiu \qi T}{\qu}}  >\frac{\qi}{3}
\,.
\end{cases}
\end{align} 
The above discontiuities in the definition of parameter $\ell$ as a function of time horizon $T$ can be interpreted as follows: 
The parameter $\ell$ is an nondecreasing function of $T$ where for three different regimes $\ell\leq \thrjuu$, $\thrjuu< \ell \leq \qi/3$ and $\ell>\qi/3$ the parameter $\ell$ has different dependencies on $T$. 
Next, we define the remaining parameters of the algorithm in this regime:
\begin{align}
M_1 & = \left\lceil 15\frac{\qi}{\ell}T\right\rceil
,\quad 
M_2 =
\big\lceil 2\min\{ \ell,\thrjuu\}\big\rceil,
 \quad \text{ and }\quad
%\\&
 M_3
=
\begin{cases}
\lceil 3\ell \rceil, 
&\text{ if } \ell\leq \frac{\qi}{3}\,,
\\
\lceil \qi \log(N\qi)\rceil,
& \text{ if } \ell >\frac{\qi}{3}
 \end{cases}
\label{eq:ParamChoice2}
\end{align}
%\MK{Do I want $M_3 = \min\{2\ell,\qi\}\log(\qi N)$? Will this be fine?}
%
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%



\subsection{OLD Algorithm and guarantee}
\begin{theorem}\label{th:Item-upper}
Define the parameters $\thrjuu$  and $\thrjiu$ as in Equations~\eqref{eq:defthrjuu} and~\eqref{eq:defthrjiu}. Then the following bounds for regret of the \textsc{Hybrid} algorithm holds:
\[\reg(T)
\leq
 \min\Big\{ \frac{T}{2}, \,\,Y(T)\Big\}\]
where the function $Y(T)$ is defined as follows:
\begin{itemize}
\item
When either  $T\leq  \max\big\{  1, \, \frac{N\thrjuu}{\qi \thrjiu}  \big\} \, \thrjuu$ or   $\qu \geq 9\log (N\qi) $ and  $T>\qi \frac{\thrjiu}{\qu}$

\begin{align*}
Y(T)
&\leq
\begin{cases}
\vspace{.1in}
6 + 16 \log T +12 \sqrt{\frac{\qi \thrjiu}{N}T},
& \text{ if }
8\log T+ 3\sqrt{\frac{\qi\thrjiu}{N}T} \leq \thrjuu
\\ %%%
\vspace{.1in}
3 \thrjuu + 8\frac{\qu}{N}\thrjuu  + 12 \frac{1}{N} \sqrt{\qi\qu \thrjiu T},&
\text{ if }
8\log T+ 3\sqrt{\frac{\qi\thrjiu}{N}T}
>\thrjuu
\quad \text{and }
3\thrjuu  + 3\sqrt{\frac{\thrjiu \qi T}{\qu}} \leq \frac{\qi}{3}
\\  %%%
3\thrjuu  + \frac{\qu}{N} \qi \log(N\qi) +18 \frac{\thrjiu}{N} T,&
\text{ if }
8\log T+3 \sqrt{\frac{\qi\thrjiu}{N}T}>\thrjuu
\quad \text{and }
8\thrjuu  + 3\sqrt{\frac{\thrjiu \qi T}{\qu}}  >\frac{\qi}{3}
\,.
\end{cases}
\end{align*}



%
%\begin{align*}
%\begin{cases}
%17\max\big\{\log T, \sqrt{\frac{\qi\thrjiu}{16 N}T}\big\}
%  &\text{ when } \ell\leq \thrjuu\,,
%  \\
% 3\thrjuu + \log T + 
%  \max\big\{ \frac{2}{N}\sqrt{\qi \qu \log \qi \thrjiu T},\,62\,\frac{\thrjiu}{N} T\big\} 
%  &\text{ when } \ell>\thrjuu\,.
%\end{cases}
%\end{align*}
%\begin{align*}
% \reg(T) & \leq 
% \begin{cases}
% T/2, & \text{ for } T/2\leq 64\log T\\
% 64\log T
% , & \text{ for }4 \sqrt{26\frac{\qi\thrjiu}{N}T} \leq   64\log T \\
%4 \sqrt{26\frac{\qi\thrjiu}{N}T}
%, & \text{ for }
%  64\log T \leq 4 \sqrt{26\frac{\qi\thrjiu}{N}T}\leq \thrjuu/4 \text{ and }
%\\
%\frac{4 }{N}  \sqrt{25\qi \qu\thrjiu \log \qi T}
%, & \text{ for }
%\thrjuu/4  \leq 4 \sqrt{26\frac{\qi\thrjiu}{N}T}\text{ and }
%\sqrt{25 \frac{\qi \thrjiu}{\qu \log \qi}T}\leq \qi
%\\
%4\frac{\qu}{N}\qi \log\qi + 49 \frac{\thrjiu }{N} T
%, & \text{ for }
%\qi\leq \sqrt{25 \frac{\qi \thrjiu}{\qu \log \qi}T}
%\end{cases}
%\end{align*}


\item
When $\qu<9\log (N\qi) $,   and $\max\big\{  \thrjuu, \, \frac{N\thrjuu^2}{\qi \thrjiu}  \big\} < T$
or $\qu \geq 9\log (N\qi) $, and 
  $\max\big\{  \thrjuu, \, \frac{N\thrjuu^2}{\qi \thrjiu}  \big\} 
  < T\leq 
  \qi \frac{\thrjiu}{\qu}$.
%\begin{align*}
%Y(T)=
%3 + 2\thrjuu
%+
%11 \frac{\qu}{N} T\,.
%\end{align*}
\begin{align*}
 Y(T) & = 
 \begin{cases}
T/2, 
 &\quad \text{ if } T\leq \thrjuu,
 \\
3 + 2\thrjuu
+
27 \frac{\qu}{N} T
 &\quad \text{ if } T> \thrjuu\,.
 \end{cases}
\end{align*}
\end{itemize}
\end{theorem}


The simplified version of this theorem is stated in Section \ref{sec:mainresult}.
\begin{algorithm}
\caption{$\textsc{Hybrid}(\qi, \qu, N, T)$ (fixed time horizon)}
\label{alg:joint-fixed}
\begin{algorithmic}[1]
		\vspace{1mm}
\STATE Set algorithm parameters $\thrjuu, \thrjiu, M_1, M_2, M_3$, and $\ell$ as specified in Section~\ref{sss:params}.
\STATE $\Mcc{1} \gets M_1$  random items (exploitable items)
\STATE $\Mcc{2} \gets M_2$  new random items (items used in user-space exploration)
\STATE  $\Mcc{3} \gets M_3$  new random items (items used in item-space exploration)
		\vspace{1mm}
		\vspace{1mm}
\STATE $\{\R_u\}_{u\in [N]}\gets \textsc{Explore}(\Mcc{1}, \Mcc{2},\Mcc{3})$
		\vspace{1mm}
\STATE $\textsc{Exploit}(\{\R_u\}_{u\in[N]})$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
	\caption{$\textsc{Explore}(\Mcc{1}, \Mcc{2},\Mcc{3})$}\label{alg:joint-itemExplore}
	\begin{algorithmic}[1] 
\vspace{2mm}
		\STATEx \emph{Preliminary exploration of exploitable items in $\Mcc{1}$ }
\STATE Recommend each item in $\Mcc{1}$ to $\thrjiu$ random users 
(details specified in Remark~\ref{r:usersToItems})
\label{Line:exploreM1}
	\STATE $U_i \gets \rated(i)$ for each $i\in \Mcc 1$ ($U_i$ is the set of witness users to be used to put $i\in\Mcc{1}$ in clusters) 
		\vspace{2mm}
		\STATEx \emph{ Explorations to learn user preferences for item representatives}
%		\State Let $\Mcc {2} = \{\rep_1,\dots, \rep_{M_2}\}$
		\STATE Recommend all items in $\Mcc 2$ to all users \label{Line:RecommM2}
%		\For{$\ti=1,\cdots, M_2$} 
%%		\State $\rep_\ti \gets$ $j$-th item in $\Mcc{2}$ (representative item)
%		\State $a_{u,t}\gets \rep_\ti$ 
		%if $u\notin\rated_t(\rep_{\ti})$, otherwise a random item  from $\Mcc{2}$. 
		\label{line:self-item-explore}
%		\EndFor
	\vspace{1mm}
	%%
	\Statex \emph{Ignoring user structure, construct bag of exploitable items for each user based on item structure}

\IF{$\ell\leq \thrjuu$} \label{Line:smallellbegin}
	\FOR{$\ti=1,\cdots, M_2$} 
		\STATE $\rep_{\ti}  \gets \ti$-th item in $\Mcc{2}$ (representative item)
		\STATE $\S_{\ti}\gets  \{ \rep_{\ti} \}\cup\{i\in \Mcc{1}:  L_{U_i, i} = L_{U_i,\rep_\ti}\}$ \; (users in $U_i$ agree on $i$ vs. $\rep_{\ti}$)	\label{Line:defSj1} 
	\ENDFOR
				\STATE $\R_u \gets \bigcup_{j:L_{u,\rep_\ti}=+1} \S_j$ \; for each $u\in [N]$
				\label{Line:DefRu1} 
\ENDIF
	
	\vspace{1mm}
	\Statex \emph{Using user structure, construct set of exploitable items for each user}

\IF{$\ell>\thrjuu$}\label{Line:largeellbegin}
%	\Statex \emph{Partition users and learn item types (joint exploration utilizing user structure)}
	\State Partition users into fewest possible groups such that users in each group agree on all items in $\Mcc{2}$.  Let $\tauh_U(u)\in [\qu]$ be the label of user $u$'s partition. \label{line:user-partiotion}
	\State $\Pc_{\tu}\gets \{u\in[N]:\tauh_U(u)=\tu\},$ for all $\tu\in[\qu]$
%%
	\vspace{1mm}
	
	%	\Statex \emph{Learn $\ell$ item types jointly between users of the same partition}
\FOR{$\ti=1,\cdots, M_3$} 
		\State $\rep_\ti \gets$ $j$-th item in $\Mcc{3}$ (representative item)
		\State \label{line:joint-item-explore} $a_{u,t}\gets \rep_\ti$
for one user $u$ in each partition which has not rated $\rep_\ti$ yet 
		\State $\S_{\ti}\gets \{ \rep_{\ti} \}\cup \{i\in \Mcc{1}: V = \ratedtype(i)%\cap\ratedtype(\rep_{\ti})
		, L_{V, i} = L_{V,\rep_\ti}\}$
		\MK{add a remark. Notation and what happens if the cluster don't agree with each other over $i$. This could happen since partitioning is based on $\Mcc{2}$. Add a remark}
		\label{Line:defSj2}
\ENDFOR
\vspace{.1cm}
\For{$k \in [\qu]$}
\State $\R_u \gets
		\bigcup_{u'\in\Pc_{\tu}} \bigcup_{j:L_{u',\rep_\ti}=+1} \S_j$ for each $u$ such that $\tauh(u)=k$ \MK{explain}
\label{Line:DefRu2}
\ENDFOR
\ENDIF
		\Return $\{\R_u\}_{u\in [N]}$
	\end{algorithmic}
\end{algorithm}


\begin{algorithm}
	\caption{$\textsc{Exploit}\big( \{\R_u\}_{u\in [N]}\big)$}\label{alg:jointExploit}
	\begin{algorithmic}[1]
\FOR{ remaining $ t \leq T $}
\FOR{$u\in [N]$}
\IF{there is an item $i \in\R_u$ such that $u\notin \rated(i)$,} 
\STATE $a_{u,t}\gets i$ 
\ELSE  { } $a_{u,t} \gets$ a random item not yet rated by $u$.
\ENDIF
\ENDFOR
\ENDFOR
	\end{algorithmic}
\end{algorithm}

\begin{remark} \label{r:usersToItems}
Assignment of users to items in Line~\ref{Line:exploreM1} of {\sc Explore}: Recommending each item in $\Mcc{1}$ to $\thrjiu$ random users  is done over $\lceil{M_1\thrjiu}/{N}\rceil$ time-steps, with additional $N \lceil{M_1\thrjiu}/{N}\rceil -M_1\thrjiu$ recommendations being random new items. The main requirement in assigning users to items is to make Lemma~\ref{l:PrErrItemClass}  (which bounds the probability of mis-classification of each item in $\Mcc{1}$) hold.
 Since the claim addresses each item separately, we may introduce dependencies between sets of users for different items. What is important is that the set of users assigned to each specific item is uniform at random among all sets of users (or at least contains a random subset with size $\thrjiu$). For example, one can choose a random permutation over the users, repeat this list $\lceil{M_1 \thrjiu}/{N}\rceil$ times, and then assign each item in $\Mcc{1}$ to a block of $\thrjiu$ users.
\end{remark}

\begin{remark}
\label{r:timingExplore}
The time it takes to finish the exploration phase of the algorithm may be different for distinct users $u\in[N]$.
The recommendations made in Lines~\ref{Line:exploreM1} and~\ref{Line:RecommM2} of {\sc Explore} takes the same amount of time for all users. 
But if $\ell>\thrjuu$, the users are partitioned in Line~\ref{line:user-partiotion} according to the feedback taken so far and then the items in $\Mcc{3}$ is recommended to one user per partition in Line~\ref{line:joint-item-explore}. 
The more populated partitions of the users can explore many more items of $\Mcc{3}$ per unit of time, so the recommendations made in Line 14 of {\sc Explore}  takes less time for more populated partitions of users. 
As soon as a group of users finish rating items in $\Mcc{3}$, they are done with the exploration phase and enter the exploitation phase according to {\sc Exploit}, Alg.~\ref{alg:jointExploit}.% \MK{Double check to see if you want to edit this remark}
\end{remark}

\begin{remark}
\label{rem:partitionionuserserror} 
According to the model, users of the same type have identical ratings. Hence, users of the same type are always in the same group after partitioning. 
However, due to random sampling of the items in $\Mcc{2}$ (which are used to partition users), users with different types can have identical ratings for all the items in $\Mcc{2}$ in which case they will end up in the same partition. 
It follows that the total number of groups in the user partition is at most $\qu$.

 The labeling of user groups in the partitioning step is arbitrary (and may be different from the similarly arbitrary labeling of user types).

Similarly,  when in  Lines~\ref{Line:defSj1}  or~\ref{Line:defSj2} the items are grouped together, the items of similar type always fall into the same groups. 
But due to error, items of different types might fall into the same groups as well by mistake. 
Hence, the set of items $\S_{\ti}$ is a superset of items in $\Mcc{1}$ with type $\tau_I(\rep_{\ti})$. 
\end{remark}

%\begin{remark}
%\label{rem:partitionionitemserror} 
%condition on $\BB^c$
%\MK{edit this}
%\end{remark}







\begin{remark}[Trivial bound of $\reg(T)\leq T/2$]
\label{remark:II-Upper-TrivialAlg}
The regret bound we get for the algorithm is actually $\reg(T)\leq Y(T)$. One can obtain $T/2$ by a trivial algorithm which recommends random items independent of feedback to all users. This trivial algorithm  improves on our bound for 
the parameter range  in which $T/2 < Y(T)$. Thus in our analysis we focus on the parameter range where $Y(T)\leq T/2$;
 one consequence is that if $\qu\geq 9\log(N\qi)$, we focus on the regime in which 
 $\ell < T$. Also, if $\qu< 9\log(N\qi)$, we only bound regret for the time horizon $T>\thrjuu$. \MK{double check the constant.}
 \MK{Connect to cold-start time.}
\end{remark}


==> joint-lower.tex <==
\newpage
\section{General lower bound}
In this section, we provide the lower bound for the joint model introduced in Section \ref{sec:model}.


\begin{thm}\label{t:joint-L}
In the joint structure model, given $N>3\qu\log(2\qu)$, there are numerical constants $c_1, c_2, c_3$ and $C$ such that any recommendation algorithm must incur regret
\[\reg(T)\geq -1+C \begin{cases} \sqrt{\frac{T\qi}N}, \quad &\text{ if } T\leq c_1\frac{N(\log \qu)^2}{\qi}\\
\frac{\sqrt{T\qi \qu}}{N} , \quad &\text{ if } c_1\frac{N(\log \qu)^2}{\qi}\leq T\leq c_2\frac{\qi \qu}{(\log \qu)^2}\\
T\frac{\thrjil}{N}, \quad &\text{ if } c_2\frac{\qi \qu}{(\log \qu)^2}\leq T\,.
\end{cases}\]
\end{thm}

The strategy of the proof is very similar to the lower bounds of regret for user-user model and item-item model. First, we will show certain recommendations (defined in Equation~\eqref{eq:jl-def-bad}) are \textit{bad} recommendations in the sense that the probability of them being successful is at best close to half. We will represent regret defined in Equation~\eqref{eq:regdef} as the expected number of bad recommendation. Then, using a careful counting argument, we can find a lower bound for the number of bad recommendations in any algorithm which gives the lower bound for regret. The proof of this statement is a straightforward consequence of Lemmas \ref{l:jl-reg-lower}  and \ref{l:jl-bad-lower}.

In this section we use the following notations: $\tau_I(\cdot)=\{\tau_I(i'): i'\in\mathbb{N}\}$ denotes the sequence of item types for all items. $\tau_I(\cdot\setminus\{i\})=\{\tau_I(i'): i'\in\mathbb{N}, i'\neq i \}$ denotes the sequence of items types for all items excluding item $i$. The notations $\tau_U(\cdot)$ and $\tau_U(\cdot\setminus\{u\})$ are defined similarly.

$\Xi_{\cdot\setminus\{\tu,\ti\}}=\{\xi_{\tu',\ti'}:(\tu',\ti')\in[\qu]\times[\qi], (\tu',\ti')\neq (\tu,\ti)\}$ denotes all the elements in matrix $\Xi$ except $\xi_{\tu,\ti}$.

%%%%%%%%%%%
Throughout the proof we use Definition \ref{def:ul-reg} for $(t,\epsilon)$-column regularity repeated here:
	Let $A\in \{-1,+1\}^{m \times n}$. 
	For ordered tuple of distinct (column) indices $w=(i_1,\dots,i_t)\in [n]^t$, let $M=(A_{\cdot i})_{i\in w}\in  \{-1,+1\}^{m \times t}$ be the matrix formed by concatenating columns of $A$ indexed by $w$.
	For given row vector $b\in\{-1,+1\}^t$, let $K_{b,w}(A)\subseteq [m]$ be the set of rows in $M=(A_{\cdot i})_{i\in w}$ which are identical to the row $b$ . The cardinality of $K_{b,w}(A)$ is denoted by $k_{b,w}(A)$. 
	$A$ is said to be \emph{$(t,\epsilon)$-column regular} if 
	\[\max_{w,b}\Big|k_{b,w}(A)-\frac{m}{2^{t}}\Big| \leq \epsilon \frac{m}{2^{t}}\,,\]
	where the maximum is over tuples $w$ of $t$ columns and $\pm 1$ vectors $b$ of size $t$.	 We define $\rgl_{t,\epsilon}$ to be the set of $(t,\epsilon)$- column regular matrices. 
	
	According to the Definition \ref{def:row-reg}, matrix $A$ is $(t,\epsilon)$-row regular (denoted by $A^T\in\Omega_{t,\epsilon}$) if its transpose is $(t,\epsilon)-$ column regular.
		
Claim \ref{cl:ul-smalltregular} shows that if a matrix $A\in\{-1,+1\}^{m\times n}$ is \emph{$(t,\epsilon)$-column regular}, then it is also \emph{$(s,\epsilon)$-column regular} for all $s<t.$

In Lemma \ref{l:ul-regularity} it is proved that for matrix $A\in\{-1,+1\}^{m \times n}$ with i.i.d. $\mathrm{Bern}(1/2)$ entries is $(t,\epsilon)$-column regular with probability at least $$1-2(2n)^t  \max\Big\{\exp\left( - \frac{\epsilon^2}{3}\frac{m}{2^{t}}\right), \exp\left( - \frac{\epsilon}{2}\frac{m}{2^{t}}\right)\Big\}\,.$$

%%%%%%%%%%%%


\begin{definition} \label{def:jl-cit}
Let $c_i^t$ be the number of user types from which a user has rated item $i$ by time $t-1\,:$
\[c_i^t := |\{\tu\in[\qu]: \text{there exists user } u\in[N] \text{with user type } \tau_U(u)=\tu,\, \text{ s.t. }\, a_{u,s}=i \text{ for some } s<t \}|\,. \]
\end{definition}

For any $t\leq T$ and any constant $\thrjil,$
\begin{equation}
\ident[c_i^t \geq \thrjil] \leq \ident[c_i^T \geq \thrjil]\,.
\end{equation}


\begin{definition}\label{def:jl-dut}
Let $d_u^t$ be the number of distinct item types that were rated by user $u$ up to time $t-1\,:$
\[d_u^t := |\{\ti\in[\qi]:  \text{there exists item } i\in\mathbb{N} \text{with item type } \tau_I(i)=\ti,\, \text{ s.t. }\,  a_{u,s}=i \text{ for some } s<t \}|\,. \]
\end{definition}
For any $t\leq T$ and any constant $\thrjul,$
\begin{equation}
\ident[d_u^t \geq \thrjul] \leq \ident[d_u^T \geq \thrjul]\,.
\end{equation}


Throughout this section, let
\begin{equation}\label{eq:jl-eps-thr}
\epsilon=\frac{1}{\log N}, \quad \thrjil = \log \qi - 5\log\log N, \quad \thrjul = \log \qu - 5\log\log N\,.
\end{equation}



\begin{claim}\label{cl:jl-bdA1}
For any user $u\in[N],$ and item $i$  recommended to $u$ at time $t$, 
\[\Pr[L_{u,i}=+1 \,\big|\, a_{u,t}=i, c_i^t <\thrjil, d_u^t <\thrjul, \Xi^T \in \rgl_{\thrjil,\epsilon} \,,\Xi \in \rgl_{\thrjul,\epsilon}] \leq \frac{1+4\epsilon}{2}.\]
\end{claim}
\begin{proof}
We are going to show that given a preference matrix, there are many item types that are consistent with the history of an item $i$ which has been rated by less than $\thrjil$ user types. Similarly, there are many user types consistent with the history of a user that has rated less than $\thrjul$ item types. The row regularity and the column regularity of the preference matrix implies that uncertainty in types of item and user results in uncertainty of outcome of recommending $i$ to $u$. 

Given $\Xi$,  $\tau_{I}(.\setminus\{i\})$ $\tau_{U}(.\setminus\{u\})$ and $\H_{t-1}$ let $w_i=\{\tu\in[\qu]: a_{u',s}=i , \tau_U(u')=\tu , s<t\}$ be the set of user types that were recommended item $i$ up to time $t-1\,,$ and let $b_i$ be the vector of feedback from users of types in $w_i$ about item $i$ (for user type $\tu\in w_i$, the corresponding element in $b_i$ is $L_{u,i}$ for some user $u'$ with $\tau_U(u')=\tu$). Note that since $a_{u,t}=i$ and each user is recommended an item only once, we know that user $u$ was not recommended item $i$ by time $t-1\,.$ Hence conditioning on $\tau_U(.\setminus\{u\})$ (not knowing the type of user $u$) does not make the definition of $w_i$ ambiguous.

Using the notation in Definition \ref{def:ul-reg}, if $M$ is the matrix formed by concatenating the rows of $\Xi$ indexed by $w_i, $ then $K_{b_i,w_i}(\Xi^T)$ would be the set of columns (corresponding to the item types) which are identical. We claim that conditional on matrix $\Xi\,,$ vectors $b_i$ and $w_i\,,$ the type $\tau_I(i)$ of item $i$ at the end of time instant $t-1$ is uniformly distributed over the set of item types $K_{b_i,w_i}(\Xi^T)$ consistent with this data. This can be derived by applying Bayes rule considering that the prior distribution of type of each item is uniform over $[\qi]$. 

Very similarly,  given $\Xi$,  $\tau_{I}(.\setminus\{i\})$ $\tau_{U}(.\setminus\{u\})$ and $\H_{t-1}$ let $w_u=\{\ti\in[\qi]: a_{u,s}=i' , \tau_I(i')=\ti , s<t\}$ be the set of item types that were recommended to user $u$ up to time $t-1\,,$ and let $b_u$ be the vector of feedback from recommending items of types in $w_u$ to user $u$ (for item type $\ti\in w_u$, the corresponding element in $b_u$ is $L_{u,i'}$ for some user $i'$ with $\tau_I(i')=\ti$). 
%Note that since $a_{u,t}=i$ and each user is recommended an item only once, we know that user $u$ was not recommended item $i$ by time $t-1\,.$ Hence 
By a similar argument as above, conditioning on $\tau_I(.\setminus\{i\})$ %(not knowing the type of item $i$) 
does not make the definition of $w_u$ ambiguous.

As before, using the notation in Definition \ref{def:ul-reg}, conditional on matrix $\Xi,$ vector $b_u$ and $w_u$, the type $\tau_U(u)$ of user $u$ at the end of time instant $t-1$ is uniformly distributed over the set of user types $K_{b_u,w_u}(\Xi)\,.$

So, conditioning on $\Xi,\tau_{I}(.\setminus\{i\}),\tau_{U}(.\setminus\{u\})$ and $\H_{t-1}$ implies conditioning on $$\{\tau_U(u)\in K_{b_u,w_u}(\Xi),\tau_I(i)\in K_{b_i,w_i}(\Xi^T)\}$$ and $\Xi$ for the corresponding $b_u,w_u, b_i$ and $w_i\,.$ On the other hand conditioning on $ c_i^t <\thrjil$ and $d_u^t <\thrjul$ implies $w_i<\thrjil$ and $w_u<\thrjul\,.$

The event $\{L_{u,i}= +1\}$ is equivalent to the event $$\{\exists\ti\in[\qi], \tu\in[\qu], \xi_{\tu,\ti}=+1, \tau_U(u)=\tu, \tau_I(i)=\ti\}\,.$$


Using total probability lemma,
\begin{align*}
\Pr[L_{u,i}&= +1|\Xi,\tau_{I}(.\setminus\{i\}),\tau_{U}(.\setminus\{u\}),\H_{t-1}=\H]\\
& \overset{(a)}{=}  \sum_{\ti\in K_{b_i,w_i}(\Xi^T)}\Pr[\tau_I(i)=\ti, \,\tau_U(u)\in K_{b_u^+,\{w_u,\ti\}}(\Xi)|\tau_U(u)\in K_{b_u,w_u}(\Xi), \, \tau_I(i)\in K_{b_i,w_i}(\Xi^T)]\\
 &\overset{(b)}{=}  \sum_{\ti\in K_{b_i,w_i}(\Xi^T)} \frac{1}{k_{b_i,w_i}(\Xi^T)}\frac{k_{b_u^+,\{w_u,\ti\}}(\Xi)}{k_{b_u,w_u}(\Xi)}\\
\end{align*}
here equality (a) is application of total probability lemma on the type of item $i\,.$  Equality (b) uses the fact that, condition on variables specified above at time $t-1$: i)type of item $i$ is uniform over $K_{b_i,w_i}(\Xi^T)$; ii)type of user $u$ is uniform over $K_{b_u,w_u}(\Xi)$; iii) For given $\ti\in K_{b_i,w_i}(\Xi^T)\,,$ the probability of type of user $u$ being in $K_{b_u^+,\{w_u,\ti\}}(\Xi)$ is uniform proportional to the size of this set.

Using tower property of expectation on the above gives:
\begin{align*}
\Pr[L_{u,i}=+1 &\,\big|\, a_{u,t}=i, c_i^t <\thrjil, d_u^t <\thrjul, \Xi^T \in \rgl_{\thrjil,\epsilon} \,,\Xi \in \rgl_{\thrjul,\epsilon}] \\
 &\overset{(b)}{=}  \sum_{\ti\in K_{b_i,w_i}(\Xi^T)} \frac{1}{k_{b_i,w_i}(\Xi^T)}\frac{k_{b_u^+,\{w_u,\ti\}}(\Xi)}{k_{b_u,w_u}(\Xi)}\\
&\overset{(c)}{\leq}  \frac{\frac{\qu}{2^{|w_u|+1}}(1+\epsilon)}{\frac{\qu}{2^{|w_u|}}(1-\epsilon)} \overset{(d)}{\leq} \frac{1}{2}(1+4\epsilon)
\end{align*}
The last inequality is the result of the fact that: i)$k_{b_i,w_i}(\Xi^T)>1$ since $|w_i|<\thrjil\,;$ ii)$|w_u|\leq \thrjul\,;$ iii)The preference matrix $\Xi$ in $(\thrjul,\epsilon)-$ column regular: for $|w_u|<\thrjul,,$ $k_{b_u^+,\{w_u,\ti\}}(\Xi)< \frac{\qu}{2^{|w_u|+1}}(1+\epsilon)$ and  $k_{b_u,w_u}(\Xi)>\frac{\qu}{2^{|w_u|}}(1-\epsilon)\,.$ Finally, inequality (d) uses $\epsilon<\frac{1}{\log N}\,.$
\end{proof}

\begin{cor}\label{cor:jl-bdA1}
Given $(\thrjul,\epsilon)$-column regular and $(\thrjil,\epsilon)$-row regular preference matrix $\Xi$, recommending an item that has been rated by less than $\thrjil$ user types to a user that has rated less than $\thrjul$ item types gives uncertain outcome (these are among bad recommendations made by the algorithm):
\begin{align*}
\Asf{1} := \Pr[L_{u,a_{u,t}}=+1, c_{a_{u,t}}^t < \thrjil, d_{u}^t < \thrjul,  \Xi^T \in \rgl_{\thrjil,\epsilon} \,,\Xi \in \rgl_{\thrjul,\epsilon}]\\
 \leq \frac{1+4\epsilon}{2}\,\Pr[c_{a_{u,t}}^t < \thrjil, d_{u}^t < \thrjul,  \Xi^T \in \rgl_{\thrjil,\epsilon} \,,\Xi \in \rgl_{\thrjul,\epsilon}]\,.  
\end{align*}
\end{cor}

\begin{proof}
Multiplying the statement of Claim \ref{cl:jl-bdA1} by $\Pr[ a_{u,t}=i, c_i^t <\thrjil, d_u^t <\thrjul, \Xi^T \in \rgl_{\thrjil,\epsilon} \,,\Xi \in \rgl_{\thrjul,\epsilon}]$ and taking summation over $i$ gives the corollary.
\end{proof}

%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\begin{definition} \label{def:jl-B-tauU-i} Let $\BBjul{u}{i}{t}$ be  the event that a user with type $\tau_U(u)$ has rated item $i$ by time $t-1$, i.e.,
\[\BBjul{u}{i}{t} = \{{\exists u'\in[N]: a_{u',s}=i} \text{ for some } s< t \text{ with } \tau_U(u) = \tau_U(u')\}\,.\]
\end{definition}

\begin{claim}\label{cl:jl-bdA2}
Given $(\thrjil,\epsilon)$-row regular preference matrix $\Xi$, if the number of user types that have rated item $i$ is less than $\thrjil$, and no user of type $\tau_U(u)$ has rated $i$, then the outcome of recommending item $i$ to user $u$ is uncertain:
\[\Pr[L_{u,i}=+1 | a_{u,t}=i, c_i^t <\thrjil, d_u^t \geq\thrjul, (\BBjul{u}{i}{t})^c, \Xi^T \in \rgl_{\thrjil,\epsilon}] \leq \frac{1+4\epsilon}{2}\,.\]
\end{claim}


\begin{proof}
Conditional on $\Xi, \tau_U(.), \tau_I(.\setminus\{i\})$ and $\H_{t-1}$ similar to the proof of Claim \ref{cl:jl-bdA1}, define $w_i, b_i$ and $K_{b_i,w_i}(\Xi^T)\,.$
We will show that if the event $(\BBjul{u}{i}{t})^c$ holds,  conditional on $\Xi, \tau_U(.), \tau_I(.\setminus\{i\})$ and vectors $b_i$ and $w_i\,,$ the random variable $L_{u,i}$ is statistically independent of $\H_{t-1}\,:$

\[L_{u,i}\indep\H_{t-1} \big| (\BBjul{u}{i}{t})^c, \Xi, \tau_U(\cdot), \tau_I(\cdot\setminus\{i\}), \tau_I(i)\in K_{b_i,w_i}(\Xi^T)\,.\]

To see this, note that for all the history which $(\BBjul{u}{i}{t})^c$ holds, all the past recommendations of item $i$ are a function of $\Xi$,  $b_i$ and $w_i$. Past recommendations of other items are also function of $\tau_I(\cdot)$ and $\Xi.$

Using this and the fact that i) $\BBjul{u}{i}{t}$ is a deterministic function of $\H_{t-1}$ and $\tau_U(.);$ ii) $b_i$ and $w_i$ are deterministic functions of $\H_{t-1},\tau_U(.)$ and preference matrix $\Xi$, one can show that
\begin{align*}
\Pr&[L_{u,i}=+1 | a_{u,t}=i, \H_{t-1}, (\BBjul{u}{i}{t})^c, \Xi, \tau_U(\cdot), \tau_I(\cdot\setminus\{i\}), \tau_I(i)\in K_{b_i,w_i}(\Xi^T)] \\
& = \Pr[L_{u,i}=+1 | \Xi, \tau_U(\cdot), \tau_I(\cdot\setminus\{i\}), \tau_I(i)\in K_{b_i,w_i}(\Xi^T)]\\
& \overset{(a)}{=} \Pr[\tau_I(i)\in K_{b^{+}_i,\{w_i,\tau_U(u)\}}(\Xi^T)|\Xi, \tau_U(\cdot), \tau_I(\cdot\setminus\{i\}), \tau_I(i)\in K_{b_i,w_i}(\Xi^T)]\\
&\leq \frac{k_{b^{+}_i,\{w_i,\tau_U(u)\}}(\Xi^T)}{k_{b_i,w_i}(\Xi^T)}
\end{align*}
where in (a) we are using the fact that condition on the event $(\BBjul{u}{i}{t})^c$, it is guaranteed that $\tau_U(u)\notin w_i$.
\begin{align*}
\Pr[L_{u,i}=+1 | a_{u,t}=i, &c_i^t <\thrjil, d_u^t \geq\thrjul, (\BBjul{u}{i}{t})^c, \Xi^T \in \rgl_{\thrjil,\epsilon}]\\
&\leq \Exp{\frac{k_{b^{+}_i,\{w_i,\tau_U(u)\}}(\Xi^T)}{k_{b_i,w_i}(\Xi^T)} |\Xi^T \in \rgl_{\thrjil,\epsilon} }
\leq \frac{1}{2}\frac{1+\epsilon}{1-\epsilon}\leq \frac{1+4\epsilon}{2}
\end{align*}
where we used the definition of row regularity and the assumption $\epsilon<1/2\,.$
\end{proof}


\begin{cor}\label{cor:jl-bdA2}
For $\Asf{2}$ defined below, the following upper bound holds:
\begin{align*}
\Asf{2} := \Pr[L_{u,a_{u,t}}=+1, c_{a_{u,t}}^t < \thrjil, d_{u}^t \geq \thrjul, (\BBjul{u}{i}{t})^c, \Xi^T \in \rgl_{\thrjil,\epsilon} ]\\
 \leq \frac{1+4\epsilon}{2}\,\Pr[c_{a_{u,t}}^t < \thrjil, d_{u}^t \geq \thrjul, (\BBjul{u}{i}{t})^c, \Xi^T \in \rgl_{\thrjil,\epsilon} ]\,.
\end{align*}
\end{cor}
\begin{proof}
Multiplying the statement of Claim \ref{cl:jl-bdA2} by $\Pr[ a_{u,t}=i, c_i^t <\thrjil, d_u^t \geq\thrjul, (\BBjul{u}{i}{t})^c, \Xi^T \in \rgl_{\thrjil,\epsilon}]$ and summing over $i$ gives the statement of the corollary. 
\end{proof}

%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\begin{definition} \label{def:jl-B-u-tauI} Let $\BBjil{u}{i}{t}$ be  the event that user $u$ has rated an item of the same item type as item $i$ by time $t-1$, i.e.,
\[\BBjil{u}{i}{t} = \{{\exists i'\in\mathbb{N}: a_{u,s}=i'} \text{ for some } s< t \text{ with } \tau_I(i) = \tau_I(i')\}\,.\]
\end{definition}


\begin{claim}\label{cl:jl-bdA3}
 If user $u$ has not rated any item with the same type as $i$ by time $t-1\,,$ and user $u$ has rated less than $\thrjul$ distinct item types by time $t$, then the outcome of recommending  $i$ to $u$ at time $t$ is uncertain:
\[\Pr[L_{u,i}=+1 | a_{u,t}=i, c_i^t \geq\thrjil, d_u^t <\thrjul, (\BBjil{u}{i}{t})^c, \Xi \in \rgl_{\thrjul,\epsilon}] \leq \frac{1+4\epsilon}{2}\]\,.
\end{claim}
\begin{proof}
The proof is very similar to the proof of Claim \ref{cl:jl-bdA2}. Conditional on $\Xi, \tau_I(\cdot), \tau_U(\cdot,\setminus\{u\})$ and $\H_{t-1}$, define $w_u, b_u$ and $K_{b_u,w_u}(\Xi)$. Note that if event $(\BBjil{u}{i}{t})^c$ holds, then $\tau_I(i)\notin w_u\,.$ We will show that
\[L_{u,i}\indep\H_{t-1} \big| (\BBjil{u}{i}{t})^c, \Xi, \tau_U(\cdot\setminus\{u\}), \tau_I(\cdot), \tau_I(i)\in K_{b_u,w_u}(\Xi)\,.\]
To see this, note that for all the history which $ (\BBjil{u}{i}{t})^c$ holds, the outcome of all the past recommendations to user $u$ are a function of $\Xi,\tau_I(\cdot)$, $b_u$ and $w_u$. Past recommendations to other users are also function $\tau_U(\cdot\setminus\{u\}), \tau_I(\cdot)$ and $\Xi\,.$
\begin{align*}
\Pr[L_{u,i}=+1 \, &\big|\, a_{u,t}=i, \H_{t-1}, (\BBjil{u}{i}{t})^c, \Xi, \tau_U(\cdot\setminus\{u\}), \tau_I(\cdot), \tau_I(i)\in K_{b_u,w_u}(\Xi)]\\
& = \Pr[L_{u,i}=+1 \, \big|\, \Xi, \tau_U(\cdot\setminus\{u\}), \tau_I(\cdot), \tau_I(i)\in K_{b_u,w_u}(\Xi)]\\
& \overset{(a)}{=} \Pr[\tau_U(u)\in K_{b^{+}_u,\{w_u,\tau_I(i)\}}(\Xi)|\Xi, \tau_I(\cdot), \tau_U(\cdot\setminus\{u\}), \tau_U(u)\in K_{b_u,w_u}(\Xi)]\\
&\leq \frac{k_{b^{+}_u,\{w_u,\tau_I(i)\}}(\Xi)}{k_{b_u,w_u}(\Xi)}
\end{align*}
where in (a) we are using the fact that condition on the event $(\BBjil{u}{i}{t})^c$, it is guaranteed that $\tau_I(i)\notin w_u$.
\begin{align*}
\Pr[L_{u,i}=+1 | a_{u,t}=i, &c_i^t \geq\thrjil, d_u^t <\thrjul, (\BBjil{u}{i}{t})^c, \Xi \in \rgl_{\thrjul,\epsilon}]\\
&\leq \Exp{\frac{k_{b^{+}_u,\{w_u,\tau_I(i)\}}(\Xi)}{k_{b_u,w_u}(\Xi)} |\Xi \in \rgl_{\thrjul,\epsilon} }\\
&\leq \frac{1}{2}\frac{1+\epsilon}{1-\epsilon}\leq \frac{1+4\epsilon}{2}\,,
\end{align*}
where we used the definition of column regularity and the assumption $\epsilon<1/2\,.$
\end{proof}
\begin{cor}\label{cor:jl-bdA3}
For $\Asf{3}$ defined below, the following upper bound holds:
\begin{align*}
\Asf{3} & := \Pr[L_{u,a_{u,t}}=+1, c_{a_{u,t}}^t \geq\thrjil, d_u^t <\thrjul, (\BBjil{u}{a_{u,t}}{t})^c, \Xi \in \rgl_{\thrjul,\epsilon}]\\
& \leq \frac{1+4\epsilon}{2} \Pr[c_{a_{u,t}}^t \geq\thrjil, d_u^t <\thrjul, (\BBjil{u}{a_{u,t}}{t})^c, \Xi \in \rgl_{\thrjul,\epsilon}]\,.
\end{align*}
\end{cor}
\begin{proof}
Multiplying the statement of Claim \ref{cl:jl-bdA3} by $\Pr[ a_{u,t}=i, c_i^t \geq\thrjil, d_u^t <\thrjul, (\BBjil{u}{i}{t})^c, \Xi \in \rgl_{\thrjul,\epsilon}]$ and summing over $i$ gives the statement of the corollary. 
\end{proof}


%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\begin{definition} \label{def:jl-B-tauU-tauI} Let $\BBjjl{u}{i}{t}$ be  the event that a user with type $\tau_U(u)$ has rated an item with type $\tau_I(i)$ by time $t-1$, i.e.,
\[\BBjjl{u}{i}{t} = \{{\exists i'\in\mathbb{N}, u'\in[N]: a_{u',s}=i'} \text{ for some } s< t \text{ with } \tau_I(i') = \tau_I(i), \tau_U(u')=\tau_U(u)\}\,.\]
\end{definition}

\begin{claim}\label{cl:jl-bdA4}
Recommending item $i$ to user $u$ gives uncertain outcome if no user with the same type as $u$ has rated any item with the same type as $i$:
\[\Pr[L_{u,i}=+1 | a_{u,t}=i, c_i^t \geq\thrjil, d_u^t \geq\thrjul, (\BBjjl{u}{i}{t})^c] = \frac{1}{2}\]
\end{claim}
\begin{proof}
We can show that 
\[L_{u,i}\indep\H_{t-1} \big| (\BBjjl{u}{i}{t})^c, \Xi_{\cdot\setminus\{\tau_U(u),\tau_I(i)\}}, \tau_U(\cdot), \tau_I(\cdot)\,.\]
The above property holds because for all history $\H_{t-1}$ such that $(\BBjjl{u}{i}{t})^c$ holds, the outcome of all the past recommendations are function of $\Xi_{\cdot\setminus\{\tau_U(u),\tau_I(i)\}}$ and $\tau_U(\cdot)$. Also, condition on $\tau_U(\cdot)$ and $ \tau_I(\cdot)$, we have $L_{u,i}=\xi_{\tau_U(u),\tau_I(i)}$. Hence
\begin{align*}
\Pr[L_{u,i}=+1 &\, \big|\, a_{u,t}=i, \H_{t-1}, (\BBjjl{u}{i}{t})^c, \Xi_{\cdot\setminus\{\tau_U(u),\tau_I(i)\}}, \tau_U(\cdot), \tau_I(\cdot)]\\
& = \Pr[\xi_{\tau_U(u),\tau_I(i)}=+1\, \big|\,  (\BBjjl{u}{i}{t})^c, \Xi_{\cdot\setminus\{\tau_U(u),\tau_I(i)\}}, \tau_U(\cdot), \tau_I(\cdot)]\\
&= \frac{1}{2}
\end{align*}
Hence, using tower property of expectation,
\[\Pr[L_{u,i}=+1 | a_{u,t}=i, c_i^t \geq\thrjil, d_u^t \geq\thrjul, (\BBjjl{u}{i}{t})^c]= \frac{1}{2}\]
\end{proof}

\begin{cor}\label{cor:jl-bdA4}
For $\Asf{4}$ defined below, the following upper bound holds:
\begin{align*}
\Asf{4} := \Pr[L_{u,a_{u,t}}=+1,& c_{a_{u,t}}^t \geq\thrjil, d_{u}^t \geq \thrjul, (\BBjjl{u}{a_{u,t}}{t})^c ]\\
& = \frac{1}{2}\,\Pr[c_{a_{u,t}}^t \geq\thrjil, d_{u}^t \geq \thrjul, (\BBjjl{u}{a_{u,t}}{t})^c ]\,.
\end{align*}
\end{cor}
\begin{proof}
Multiplying the statement of Claim \ref{cl:jl-bdA4} by $\Pr[ a_{u,t}=i, c_i^t \geq\thrjil, d_u^t \geq\thrjul, (\BBjjl{u}{i}{t})^c]$ and summing over $i$ gives the statement of the corollary. 
\end{proof}
\newpage
Let
\begin{align}
\Bsf{1}(u,t) &:=\ident[c_{a_{u,t}}^t < \thrjil, d_{u}^t < \thrjul]\label{eq:jl-def-B1}\\
\Bsf{2}(u,t) &:=\ident[c_{a_{u,t}}^t < \thrjil, d_{u}^t \geq \thrjul, (\BBjul{u}{
a_{u,t}}{t})^c]\label{eq:jl-def-B2}\\
\Bsf{3}(u,t) &:=\ident[c_{a_{u,t}}^t \geq \thrjil, d_{u}^t < \thrjul, (\BBjil{u}{a_{u,t}}{t})^c]\label{eq:jl-def-B3}\\
\Bsf{4}(u,t) &:= \ident[c_{a_{u,t}}^t \geq\thrjil, d_{u}^t \geq \thrjul, (\BBjjl{u}{a_{u,t}}{t})^c]\,.\label{eq:jl-def-B4}
\end{align}
Next, define the set of bad recommendations up until time $T$ to be:
\begin{align}\label{eq:jl-def-bad}
\bad(T)& := \sum_{t=1}^T \sum_{u=1}^N\Exp{\Bsf{1}(u,t)+\Bsf{2}(u,t)+\Bsf{3}(u,t)+\Bsf{4}(u,t)} \,.
\end{align}
\begin{lemma}\label{l:jl-reg-lower}
For the set of bad recommendations defined in Equation~\eqref{eq:jl-def-bad}, the following lower bound for regret holds:
\[N\reg(T)\geq  \frac{1-4\epsilon}{2} \bad(T)- 4\,.\]
\end{lemma}
\begin{proof}
We decompose the set of recommendations made up until time $T$ according to: i) the preference matrix $\Xi$ is $(\thrjil,\epsilon)-$row regular or not; ii) the preference matrix $\Xi$ is $(\thrjul,\epsilon)-$column regular or not; iii) the user been has recommended items from more than $\thrjul$ distinct item types; iv) The recommended item has been recommended to users from more than $\thrjil$ distinct user types or not; v) user $u$ or users with similar type has rated item $i$ or any item with the similar item type before. 
\newpage We use the Definitions \ref{def:jl-cit}, \ref{def:jl-dut}, \ref{def:jl-B-tauU-i},\ref{def:jl-B-u-tauI} and  \ref{def:jl-B-tauU-tauI}.
\begin{align}
N(T-\reg(T)) & = \sum_{t=1}^T \sum_{u=1}^N \ident[L_{u,a_{u,t}}=+1]\notag\\
& \leq \Asf{1} + \Asf{2} + \Asf{3} + \Asf{4}\notag \quad+ 2 \Pr[\Xi \notin \rgl_{\thrjul,\epsilon}] + 2 \Pr[\Xi^T \notin \rgl_{\thrjil,\epsilon}]\notag\\
& \quad + \Pr[c_{a_{u,t}}^t \geq \thrjil, d_{u}^t < \thrjul, \BBjil{u}{i}{t}]\notag+ \Pr[c_{a_{u,t}}^t < \thrjil, d_{u}^t \geq \thrjul, \BBjul{u}{i}{t}]\notag\\
&  \quad+ \Pr[c_{a_{u,t}}^t \geq\thrjil, d_{u}^t \geq \thrjul, \BBjjl{u}{a_{u,t}}{t}]\notag\\
& \overset{\text{(a)}}{\leq}  
 \frac{1+4\epsilon}{2}\,\Pr[c_{a_{u,t}}^t < \thrjil, d_{u}^t < \thrjul] \notag\\
&\quad+ \frac{1+4\epsilon}{2}\,\Pr[c_{a_{u,t}}^t < \thrjil, d_{u}^t \geq \thrjul, (\BBjul{u}{i}{t})^c ] \notag\\
&\quad + \frac{1+4\epsilon}{2} \Pr[c_{a_{u,t}}^t \geq\thrjil, d_u^t <\thrjul, (\BBjil{u}{a_{u,t}}{t})^c]\notag \\
&\quad+\frac{1}{2}\,\Pr[c_{a_{u,t}}^t \geq\thrjil, d_{u}^t \geq \thrjul, (\BBjjl{u}{a_{u,t}}{t})^c ]\notag\\
&\quad+ \frac{4}{N}\notag
 + \Pr[c_{a_{u,t}}^t \geq \thrjil, d_{u}^t < \thrjul, \BBjil{u}{i}{t}]\notag\\
&  \quad+ \Pr[c_{a_{u,t}}^t < \thrjil, d_{u}^t \geq \thrjul, \BBjul{u}{i}{t}]\notag\\
&  \quad+ \Pr[c_{a_{u,t}}^t \geq\thrjil, d_{u}^t \geq \thrjul, \BBjjl{u}{a_{u,t}}{t}]\notag\\
& \leq  NT - \frac{1-4\epsilon}{2} \bad(T) + \frac{4}{N} \label{eq:jl-reg-bd1}
\end{align}
where in inequality (a) we used the statement of Claims ,\ref{cl:jl-bdA1}, \ref{cl:jl-bdA2}, \ref{cl:jl-bdA3} and \ref{cl:jl-bdA4}.

Using statement of Lemma \ref{l:ul-regularity}, $ \Pr[\Xi \notin \rgl_{\thrjul,\epsilon}]<\frac{1}{N}$ and $\Pr[\Xi^T \notin \rgl_{\thrjil,\epsilon}]<\frac{1}N$ with the choice of parameters given in Equation~\eqref{eq:jl-eps-thr}.
\end{proof}

Next, we will represent find several lower bounds for the total number of bad recommendations defined in Equation~\eqref{eq:jl-def-bad} as a function of parameters of the algorithm. Later, we will show that for any choice of these parameters, there is some lower bound for $\bad(T)$.

%
%We are going to use \MK{Are we?}
%\begin{align*}
%\good(T) &= \sum_{t=1}^T\sum_{u\in\Wc_T} \Exp{\B{1}(u,t)+\B{2}(u,t)+\B{3}(u,t)} \\
%&+\sum_{t=1}^T\sum_{u\in[N]\setminus\Wc_T} \Exp{\B{1}(u,t)}\,.
%\end{align*}
%
%
\begin{definition}\label{def:jl-itemsF} Let $\Fc_T$   be the items that have been rated by more than $\thrjil$ user types by time $T$ and 
\begin{equation}
\label{eq:jl-fT}
f_T := |\Fc_T| =\sum_{i\in\mathbb{N}} \ident[c_{i}^{T}\geq \thrjil].
\end{equation}
\end{definition}

\begin{definition}\label{def:jl-itemsG} Let $\Gc_T$ to be the items that have been rated by less than $\thrjil$ user types by time $T$ and 
\begin{equation}
\label{eq:jl-gT}
g_T := |\Gc_T|=
 \sum_{i\in\mathbb{N}} \ident[0 < c_{i}^{T}< \thrjil].
\end{equation}
\end{definition}

\begin{claim}
The expected number of bad recommendations defined in Equation~\eqref{eq:jl-def-bad} satisfies the following lower bound: 
\begin{equation}\label{eq:jl-bad-gT-fT}
\bad(T)\geq f_T (\thrjil-1) + g_T \,.
\end{equation}
\end{claim}

\begin{proof}
Using Equations~\eqref{eq:jl-def-B1} and~\eqref{eq:jl-def-B2}:
\begin{align*}
\Bsf{1}(u,t) +\Bsf{2}(u,t) &=
\ident[c_{a_{u,t}}^t < \thrjil, d_{u}^t < \thrjul,\BBjul{u}{a_{u,t}}{t}]\\
&\quad + \ident[c_{a_{u,t}}^t < \thrjil, d_{u}^t < \thrjul,(\BBjul{u}{a_{u,t}}{t})^c]\\
&\quad +\ident[c_{a_{u,t}}^t < \thrjil, d_{u}^t \geq \thrjul, (\BBjul{u}{a_{u,t}}{t})^c]\\
& \geq \ident[c_{a_{u,t}}^t < \thrjil, (\BBjul{u}{a_{u,t}}{t})^c]\,.
\end{align*}
According to Definition \ref{def:jl-itemsF} the items in $\Fc_T$  are rated by at least $\thrjil$ distinct user types by time $T$. So, each item  $i\in\Fc_T$, there are recommended at least $\thrjil-1$  times in which $\ident[c_{i}^t < \thrjil, (\BBjul{u}{i}{t})^c]$ holds. The items in $\Gc_T$ are recommended to at least one user by time $T$. Hence, all items $i\in\Gc_T$ are recommended at least once when $\ident[c_{i}^t < \thrjil, (\BBjul{u}{i}{t})^c]$ holds. Hence, 
\begin{align*}
%\label{eq:jl-B1B2-fg}
 \sum_{t=1}^T \sum_{u=1}\Bsf{1}(u,t) +\Bsf{2}(u,t) & \geq f_T (\thrjil-1) + g_T  \,.
\end{align*}
\end{proof}

\begin{claim}The expected number of bad recommendations defined in Equation~\eqref{eq:jl-def-bad} satisfies the following lower bound:
\begin{equation}\label{eq:jl-asympt}
\bad(T)\geq T(\thrjil-1)\,.
\end{equation}
\end{claim}
\begin{proof}
The total number of recommendations made to all the users by the end of time $T$ is $TN$. The items in $\Fc_T$ can be recommended at most $N$ times. According to the definition given in Equation ~\eqref{eq:jl-gT}, the items in $\Gc_T$ are recommended at most $\thrjil$ times. Hence, 
\[TN\leq f_T N + g_T (\thrjil-1)\,.\]
Plugging this into Equation~\eqref{eq:jl-bad-gT-fT} gives
\[\bad(T)> T(\thrjil- 1)+ g_T(1-\frac{(\thrjil-1)^2}{N}).\]
Note that for $N$ large enough, ${(\thrjil-1)^2}<{N}$ which gives the statement of the claim.
\end{proof}


\begin{definition}\label{def:jl-usersH}
Let $\Wc_T\subseteq [N]$ be the set of users that have rated more than $\thrjul$ distinct item types by time $T\,.$ Let \begin{equation}\label{eq:jl-wT}
w_T:= \frac{1}{N}|\Wc_T|=\frac{1}{N}\sum_{u\in[N]}\ident[d_u^T\geq \thrjul]\,.
\end{equation} 
\end{definition} 

Note $u\notin\Wc_T,$ for all $t\in[T],$ we have $d_u^t<\thrjil\,.$

%%%%%%%%%%%%%%%
\begin{claim}
The expected number of bad recommendations defined in Equation~\eqref{eq:jl-def-bad} satisfies the following lower bound:
\begin{equation}\label{eq:jl-wT-N-rU}
\bad(T)\geq w_T N (\thrjul-1)\,.
\end{equation}
\end{claim}
\begin{proof}
Using Equations~\eqref{eq:jl-def-B1} and~\eqref{eq:jl-def-B3}:
\begin{align}
\Bsf{1}(u,t) +\Bsf{3}(u,t) & = 
\ident[c_{a_{u,t}}^t < \thrjil, d_{u}^t < \thrjul, 
\BBjil{u}{a_{u,t}}{t}] \notag\\
&\quad + \ident[c_{a_{u,t}}^t < \thrjil, d_{u}^t < \thrjul, (\BBjil{u}{a_{u,t}}{t})^c]\notag\\
& \quad +\ident[c_{a_{u,t}}^t \geq \thrjil, d_{u}^t < \thrjul, (\BBjil{u}{a_{u,t}}{t})^c]\notag\\
&\geq 
\ident[ d_{u}^t < \thrjul, (\BBjil{u}{i}{t})^c]\label{eq:jl-B1-B3}
\end{align}
According to Definition \ref{def:jl-usersH} the users in $\Wc_T$  have rated  at least $\thrjul$ distinct item types by time $T$. So, each user  $u\in\Wc_T$,  are recommended at least $\thrjul-1$  times in which $\ident[d_{u}^t < \thrjul, (\BBjil{u}{i}{t})^c]$ holds. The users in $[N]\setminus\Wc_T$ are recommended at least one item by time $T$. Hence, all users $u\in[N]\setminus\Wc_T$ are recommended at least once when $\ident[d_{u}^t < \thrjul, (\BBjul{i}{i}{t})^c]$ holds. Hence, 
\begin{align*}
 \sum_{t=1}^T \sum_{u\in \Wc_T}\Bsf{1}(u,t) +\Bsf{3}(u,t) & \geq w_T N  (\thrjul-1)
\end{align*}
\end{proof}
%%%%%%%%%%%%%%%

\begin{definition}\label{def:jl-gamma-U}
 Let $\Gamma_{u}^T$ be the set of item types that are rated by user $u$ by time $T$.
\[\Gamma_u^T=\{\ti\in[\qi]: \sum_{t\in[T], i:\tau_I(i)=\ti}\ident[a_{u,t}=i]\neq 0\}\]
Let $\gamma_u^T = |\Gamma_u^T|$.
\end{definition}

Note that for according to the definition of $\Wc^T$ 
\begin{equation} \label{eq:jl-gamu -notin-W} 
\forall u\notin \Wc_T, \quad \gamma_u^T <\thrjul.
\end{equation}


\begin{definition} Let $r_{\ti}^T$ be the number of items with item type $j$ that have been rated by time $T$:
\[r_{j}^T=|\{i: \tau_I(i)=j, a_{u,t}=i, u\in[N], t\leq T\}|.\]
\end{definition}


The total number of items recommended (ever seen by the algorithm) by time $T$ is $f_T + g_T\,.$   Also, for any user $u$, $T$ items from $\Fc_T\cup\Gc_T$ with types in $\Gamma_u^T$ (defined in  Definition \ref{def:jl-gamma-U}) are recommended by time $T$. Hence, $T\leq \sum_{\ti\in\Gamma_{u}^T} r_{\ti}^T\,.$
This implies $\gamma_*^T := \min_{u\notin \Wc_T} \gamma_u^T \geq \frac{T}{\max_{j}r_{j,T}}\,.$ 

Note that the prior distribution of type of each item is uniform on $[\qi]$ independently of other items. So, $r_{\ti}^{T}$ is $\mathsf{Bin}(f_T + g_T , \frac{1}{\qi})\,.$ We provide two different deviation bounds for the random variable $\max_{\ti\in\qi}r_{\ti}^T$ as a function of $f_T + g_T$:
\begin{itemize}
\item  When $f_T + g_T\geq 6\qi\log\qi$, using the Chernoff bound in Lemma \ref{l:Chernoff} with $\epsilon=1,$  
\begin{equation}\label{eq:jl-maxr1}
\Pr[\max_{\ti\in\qi}r_{\ti}^T\geq 2\frac{f_T+g_T}{\qi}]\leq \qi\exp\left(-\frac{f_T+g_T}{3\qi}\right) \leq  \frac{1}{\qi}\,,
  \end{equation}
  where the last inequality is due to the fact that $f_T+g_T \geq 6\qi\log\qi\,.$ This implies that
\begin{equation}\label{eq:jl-gammaTlowerbd1}
\Pr[\gamma_*^T\geq \frac{T\qi}{2(f_T + g_T)}]\geq 1/2
\end{equation}  
  and we always have $\gamma_*^T\geq 1$.
\item  When $f_T + g_T < 6\qi\log\qi$, using the Chernoff bound in Lemma \ref{l:Chernoff} with $$\epsilon=\frac{18\qi \log\qi}{f_T + g_T}-1 >2,$$  gives
\begin{equation}\label{eq:jl-maxr2}
\Pr[\max_{\ti\in\qi}r_{\ti}^T\geq 18\log \qi]\leq \qi\exp\left(-(\frac{18\qi \log\qi}{f_T + g_T}-1 )^2\frac{f_T+g_T}{2\qi}\right) \leq  \frac{1}{\qi}\,,
  \end{equation}
  where the last inequality is due to the fact that $f_T+g_T < 6\qi\log\qi\,.$ This implies that 
\begin{equation}\label{eq:jl-gammaTlowerbd2}
\Pr[\gamma_*^T\geq  \frac{T}{18\log \qi}]\geq 1/2
\end{equation}  
  and we always have $\gamma_*^T\geq 1$.
\end{itemize}
The above two cases show that 
\begin{equation}\label{eq:jl-gammaTlowerbd3}
\Pr[\gamma_*^T\geq  \min\{\frac{T}{36\log \qi},\frac{T\qi}{6(f_T+g_T)}\}]\geq 1/2
\end{equation}  
and we always have $\gamma_*^T\geq 1$.
  
\begin{claim}\label{cl:jl-wT-neq-one}
If $w_T\neq 1,$ for $\delta=\qi \exp(-\frac{T}{3\qi})$ we have
\begin{equation}
\bad(T) \geq (1-\delta) \frac{T\qi}{3\thrjul}
\end{equation}
\end{claim}

\begin{proof}

Plugging Equation~\eqref{eq:jl-gammaTlowerbd1} into Equation~\eqref{eq:jl-gamu -notin-W}, if $w_T\neq 1, $ then $\gamma_*^T\leq \thrjul$ and 
\begin{equation*}
g_T \geq \frac{T \qi}{2\thrjul} - f_T
\end{equation*}
Plugging this into Equation~\eqref{eq:jl-bad-gT-fT} shows that if $w_T\neq 0,$ with probability $1-\delta,$
\begin{equation}
 \sum_{t=1}^T \sum_{u=1}\Bsf{1}(u,t) +\Bsf{2}(u,t) \geq \frac{T \qi}{2\thrjul} + f_T (\thrjil -2) > \frac{T \qi}{2\thrjul}\,.
\end{equation}
Using definition of $\bad(T)$ given in Equation~\eqref{eq:jl-def-bad} gives the statement of the claim.
\end{proof}
 
\begin{definition}\label{def:jl-theta-U}
 Let $\Theta_{\tu}^T$ be the set of item types that are rated by any user of type $\tu$ by time $T$.
\[\Theta_{\tu}^T=\{\ti\in[\qi]: \sum_{t\in[T]\atop i:\tau_I(i)=\ti}\ident[\sum_{u: \tau_U(u)=\tu}a_{u,t}=i]\neq 0\}\]

Let $\theta_{\tu}^T = |\Theta_{\tu}^T|$.
\end{definition}

Similarly, for any user type $\tu$, $T$ items from $\Fc_T\cup\Gc_T$ with types in $\Theta_u^T$ (defined in  Definition \ref{def:jl-theta-U}) are recommended by time $T$. Hence, $T\leq \sum_{\ti\in\Theta_{\tu}^T} r_{\ti}^T\,.$
This implies $\theta_*^T := \min_{\tu} \theta_{\tu}^T \geq \frac{T}{\max_{j}r_{j,T}}\,.$ 
Similar to the Equation~\eqref{eq:jl-maxr1} and~\eqref{eq:jl-maxr2}:
\begin{itemize}
\item  When $f_T + g_T\geq 6\qi\log\qi$,  
\begin{equation}\label{eq:jl-thetaTlowerbd1}
\Pr[\theta_*^T\geq \frac{T\qi}{2(f_T + g_T)}]\geq 1/2\,.
\end{equation}
we always have $\theta_*^T\geq 1.$
%\begin{equation}\label{jl-eq-one-over-gamma}
%\bad(T)\geq (1-\qi\exp(-\frac{T}{3\qi})) [\frac{T \qi}{2\gamma_*^T}  +f_T(\thrjil-2)]\,.
%\end{equation}
%Also, with probability at least $1/2\,,$
%\begin{equation}\label{eq:jl-gT-gamma-fT}
%g_T  \geq \frac{T \qi}{2\gamma_*^T} - f_T\,.
%\end{equation}
%

\item  When $f_T + g_T < 6\qi\log\qi$ 
\begin{equation}\label{eq:jl-thetaTlowerbd2}
\Pr[\theta_*^T\geq \frac{T}{18\log \qi}]\geq 1/2\,.
\end{equation}
we always have $\theta_*^T\geq 1.$
\end{itemize}
%
The above two cases show that 
\begin{equation}\label{eq:jl-thetaTlowerbd3}
\Pr[\theta_*^T\geq  \min\{\frac{T}{36\log \qi},\frac{T\qi}{6(f_T+g_T)}\}]\geq 1/2
\end{equation}  
and we always have $\theta_*^T\geq 1$.
 % 
%
%\begin{equation}
%\Pr[\theta_*^T \leq \frac{T\qi}{2(f_T + g_T) }]\leq \qi \exp(-\frac{T}{3\qi})\,.
%\end{equation}
%So, with probability at least $1-\delta\,,$
%\begin{equation}
%g_T  \geq \frac{T \qi}{2\theta_*^T} - f_T\,.
%\end{equation}
%
%Plugging this into Equation~\eqref{eq:jl-bad-gT-fT} gives
%\begin{equation}\label{jl-eq-one-over-theta}
%\bad(T)\geq (1-\qi\exp(-\frac{T}{3\qi})) [\frac{T \qi}{2\theta_*^T}  +f_T(\thrjil-2)]\,.
%\end{equation}
%%%%%%%%%%%%%%%
\begin{claim} The number of bad recommendations up to time $T$ satisfies the lower bound:
\begin{equation}\label{eq:jl-wtheta-Ngamma}
\bad(T) \geq\frac{w_T \qu }{4}\theta_*^T+(1-w_T) N \gamma_*^T\,.
\end{equation}
\end{claim}

\begin{proof}
As shown in Equation~\eqref{eq:jl-B1-B3}
\[\Bsf{1}(u,t) +\Bsf{3}(u,t) \geq 
\ident[ d_{u}^t < \thrjul, (\BBjil{u}{i}{t})^c]\]

Taking the summation for $u\notin\Wc_T$ gives
\begin{equation}\label{eq:jl-B1-B3-gamma}
\sum_{t=1}^T\sum_{u\notin\Wc_T}\Bsf{1}(u,t) +\Bsf{3}(u,t) \geq 
(1-w_T) N \gamma_*^T
\end{equation}

Note that if no user from user type $\tau_U(u)$ has rated any item from item type $\tau_I(i)$, then we are sure that no user from user type $\tau_U(i)$ has rated item $i$: $\ident[(\BBjul{u}{i}{t})^c]\geq \ident[(\BBjjl{u}{i}{t})^c] $. We also know that $\ident[d_u^t>\thrjul]\geq \ident[d_u^T>\thrjul]$ Hence, 
\begin{align*}
\Bsf{2}(u,t) +\Bsf{4}(u,t) & = \ident[c_{a_{u,t}}^t < \thrjil, d_{u}^t \geq \thrjul, (\BBjul{u}{i}{t})^c]\\
 &\quad + \ident[c_{a_{u,t}}^t \geq\thrjil, d_{u}^t \geq \thrjul, (\BBjjl{u}{a_{u,t}}{t})^c]\\
& \geq 
\ident[c_{a_{u,t}}^t < \thrjil, d_{u}^T \geq \thrjul, (\BBjjl{u}{i}{t})^c]\\
 &\quad + \ident[c_{a_{u,t}}^t \geq\thrjil, d_{u}^T \geq \thrjul, (\BBjjl{u}{a_{u,t}}{t})^c]\\
 &\geq \ident[d_{u}^T \geq \thrjul, (\BBjjl{u}{a_{u,t}}{t})^c]
\end{align*}

Using the Chernoff bound, with probability $1-\qu\exp(-\frac{N}{3\qu}),$ the maximum number of users with any given user type is less than $2\frac{N}{\qu}\,.$
So, with probability  $1-\qu\exp(-\frac{N}{3\qu}),$ there are at least $\frac{w_T N}{2\frac{N}{\qu}}=w_T \qu /2$ distinct user types among the users in $\Wc_T.$ Counting the total number of item types any given user type with users in $\Wc_T$ has rated (and given Definition \ref{def:jl-theta-U}), with probability $1-\qu\exp(-\frac{N}{3\qu}),$
\begin{equation}
\sum_{t=1}^T\sum_{u\in\Wc_T}\Bsf{2}(u,t) +\Bsf{4}(u,t) \geq 
\frac{w_T \qu \theta_*^T}{2}\,.
\end{equation}
Merging this with Equation~\eqref{eq:jl-B1-B3-gamma} gives
\[\bad(T)\geq [1-\qu\exp(-\frac{N}{3\qu})] \frac{w_T \qu \theta_*^T}{2}+(1-w_T) N \gamma_*^T\] 
We assume $N$ is large enough so that $N>3\qu \log(2\qu)\,.$ which gives the statement of claim.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{l:jl-bad-lower}
For some constant $c>0$, the expected number of bad recommendations defined in Equation~\eqref{eq:jl-def-bad} satisfies the following lower bound:
\begin{align*}
\bad(T) \geq \begin{cases} c\sqrt{T\qi N}, \quad &\text{ if } 3\qi \log(2\qi)\leq T\leq \frac{N\thrjul^2}{\qi}\\
c\sqrt{T\qi \qu} , \quad &\text{ if } \frac{N\thrjul^2}{\qi}\leq T\leq \frac{\qi \qu}{\thrjul^2}\\
cT\thrjil, \quad &\text{ if } \frac{\qi \qu}{\thrjul^2}\leq T\,.
\end{cases}
\end{align*}
\end{lemma}
\begin{proof}

 Equation~\eqref{eq:jl-bad-gT-fT} and plugging Equation~\eqref{eq:jl-thetaTlowerbd3} into Equation~\eqref{eq:jl-wtheta-Ngamma} gives:
 \begin{align*}
2 \bad(T)&\geq  \max\left\{f_T + g_T\, , \, \frac{w_T\qu}{4} \min\{\frac{T}{36\log \qi},\frac{T\qi}{6(f_T+g_T)}\} + (1-w_T) N \gamma_*^T\right\}
 \end{align*}
 If $Tw_T\qu\geq 144\qi(\log\qi)^2$, then 
  \begin{align*}
  2\bad(T)&\geq  \max\left\{f_T + g_T\, , \, \frac{w_T\qu}{4} \frac{T\qi}{6(f_T+g_T)} + (1-w_T) N \gamma_*^T\right\}\\
 &\geq \sqrt{\frac{w_T \qu \qi}{8}T} +(1-w_T) N \gamma_*^T
 \end{align*}
 otherwise, 
  \begin{align*}
2 \bad(T)&\geq \frac{w_T\qu}{4} \frac{T}{36\log \qi}+ (1-w_T) N \gamma_*^T
 \end{align*}

Similarly,  
 Equation~\eqref{eq:jl-bad-gT-fT} and plugging Equation~\eqref{eq:jl-gammaTlowerbd3} into above gives:
 \begin{itemize}
 \item If $Tw_T\qu\geq 144\qi(\log\qi)^2$ and $T(1-w_T)N\geq 216\qi(\log\qi)^2$ 
 \begin{align*}
  2\bad(T)&\geq \sqrt{\frac{w_T \qu \qi}{32}T} +\sqrt{\frac{(1-w_T) N \qi}{6}T}
 \end{align*}
  \item If $Tw_T\qu\geq 144\qi(\log\qi)^2$ and $T(1-w_T)N< 216\qi(\log\qi)^2$ 
 \begin{align*}
  2\bad(T)&\geq \sqrt{\frac{w_T \qu \qi}{32}T} +\frac{(1-w_T) N }{36\log \qi}T
 \end{align*}
 
 \item If $Tw_T\qu< 144\qi(\log\qi)^2$ and $T(1-w_T)N\geq 216\qi(\log\qi)^2$ 
 \begin{align*}
  2\bad(T)&\geq  \frac{w_T\qu}{4} \frac{T}{36\log \qi} +\sqrt{\frac{(1-w_T) N \qi}{6}T}
 \end{align*}
 
 \item If $Tw_T\qu< 144\qi(\log\qi)^2$ and $T(1-w_T)N< 216\qi(\log\qi)^2$ 
 \begin{align*}
  2\bad(T)&\geq  \frac{w_T\qu}{4} \frac{T}{36\log \qi} +\frac{(1-w_T) N }{36\log \qi}T
 \end{align*}
 \end{itemize}
% \begin{align*}
%2 \bad(T)&\geq  \max\left\{f_T + g_T\, , \, \frac{w_T\qu}{4} \min\{\frac{T}{36\log \qi},\frac{T\qi}{6(f_T+g_T)}\} + (1-w_T) N \gamma_*^T\right\}
% \end{align*}
% If $Tw_T\qu\geq \qi(\log\qi)^2$, then 
%  \begin{align*}
%  2\bad(T)&\geq  \max\left\{f_T + g_T\, , \, \frac{w_T\qu}{4} \frac{T\qi}{6(f_T+g_T)} + (1-w_T) N \gamma_*^T\right\}\\
% &\geq \sqrt{\frac{w_T \qu \qi}{8}T} +(1-w_T) N \gamma_*^T
% \end{align*}
% otherwise, 
%  \begin{align*}
%2 \bad(T)&\geq \frac{w_T\qu}{4} \frac{T}{36\log \qi}+ (1-w_T) N \gamma_*^T
% \end{align*}
% 
%\begin{itemize}
%\item When $f_T+g_T \geq 6\qi\log\qi$,% plugging Equations~\eqref{eq:jl-gammaTlowerbd1} and~\eqref{eq:jl-thetaTlowerbd1}  into the statement of Claim \ref{eq:jl-wtheta-Ngamma} gives 
%with probability at least $1/2$
%\[2\bad(T)\geq \sqrt{\frac{w_T \qu \qi}{8}T} +(1-w_T) N \gamma_*^T\]
%
%\item When $f_T+g_T <6\qi\log\qi$,  with probability at least $1/2$
%\[2\bad(T)\geq\frac{w_T \qu }{4}\frac{T}{18\log\qi}+(1-w_T) N \gamma_*^T\]
%\end{itemize}
%
%
%
%Assuming $T\geq 3\qi\log(2\qi)$ and
%using Equation~\eqref{jl-eq-one-over-theta} and  Equation~\eqref{eq:jl-wtheta-Ngamma} give
%\begin{align*}
%4 \bad(T) &\geq \max\left\{\frac{T\qi}{\theta_*^T} + 2f_T(\thrjil-2)\,\, ,\,\, w_T\qu\theta_*^T+ 4(1-w_T)N\gamma_*^T\right\}\\
%&\geq 2 (1-w_T)N\gamma_*^T +  f_T(\thrjil-2) +\sqrt{T w_T\qi\qu}\\
%\end{align*}
%where the last inequality holds for any choice of $\theta_*^T\geq 0.$
%Using this equation and Equation~\eqref{jl-eq-one-over-gamma} gives
%
%\begin{align*}
%4\bad(T)&\geq \max\left\{ 2 (1-w_T)N\gamma_*^T + f_T(\thrjil-2) + \sqrt{T w_T\qi\qu} \,\, , \right.\\
%&\qquad \qquad \left.\,\,\frac{2T \qi}{\gamma_*^T}  +4f_T(\thrjil-2) \right\}\\
%& \geq \frac{\sqrt{T w_T\qi\qu}}{2} + 2f_T(\thrjil-2) + 2\sqrt{NT\qi (1-w_T)}
%\end{align*}
%
%which gives
%\begin{equation}
%\bad(T) \geq \frac{1}{8} \sqrt{T w_T\qi\qu} + \frac{1}{2} \sqrt{NT\qi (1-w_T)}
%\end{equation}
%
%This inequality, in addition to Equations~\eqref{eq:jl-asympt} and~\eqref{eq:jl-wT-N-rU} and statement of Claim \ref{cl:jl-wT-neq-one} gives for some constant $c$,
Some algebraic manipulations shows that for any choice of the parameter $w_T$ by the algorithm, the following lower bound holds:
\begin{align*}
\bad(T) \geq c\begin{cases} \sqrt{T\qi N}, \quad &\text{ if }  T\leq \frac{N\thrjul^2}{\qi}\\
\sqrt{T\qi \qu} , \quad &\text{ if } \frac{N\thrjul^2}{\qi}\leq T\leq \frac{\qi \qu}{\thrjul^2}\\
T\thrjil, \quad &\text{ if } \frac{\qi \qu}{\thrjul^2}\leq T
\end{cases}
\end{align*}
\end{proof}%end of proof of lemma

==> joint-upper.tex <==


In this chapter, a hybrid algorithm is proposed which utilizes the structure in both user and item space. Then, information theoretic lower bound shows that the proposed algorithm achieves almost optimal performance in virtually all regimes of parameters of the model. 

Utilizing both structure in user space and item space provides the benefits of both user-user and item-item algorithm. Similar to item-item algorithm, the hybrid algorithm can start making meaningful recommendation very early on (small cold-start time). The asymptotic slope of regret in hybrid algorithm is also as small as the one in item-item algorithm. Additionally, similar to user-user algorithm, the asymptotic slope is achieved much faster compared to item-item algorithm. The explanation for this observation is that the by learning the structure in user space, the effort of learning the item space is shared among the users of similar types. 
\section{Hybrid algorithm - upper bound}

The algorithm we are proposing based on the joint structure in user space and item space is quite similar to the  proposed item-item algorithm. For small $T\,,$ the algorithm is oblivious to the structure in user space and performing exactly like the item-item algorithm.

 By exploring part of the item space, the structure in user space is known to the algorithm.
 After that, exploring the rest of item space is easier due to collaboration between users. 
  When the number of learned item types in item-item algorithm (the parameter $\ell$ in Algorithm \ref{alg:item-fixed}) is greater than $\thrjuu = \log N\qu^2,$ it is possible to partition users based on their type correctly with high probability. This happens when $T$ is large enough so that  $\ell>\thrjuu$.  The algorithm learns the user structure through partitioning the users (similar to user-user model in Algorithm \ref{alg:user})

Learning user types reduces the cost of item exploration. Knowing the type of users, to learn an item type, instead of recommending it to all users, one needs to recommend it to one user from each user type. This reduces the cost of exploration by a factor of $\frac{\qu}{N}$. 

After all $\qi$ item types are learned, the joint algorithm works similar to item-item algorithm (Algorithm \ref{alg:item-fixed}) again. The user structure becomes irrelevant again. The intuition is that utilizing structure in user space gives asymptotic regret slope of $\frac{\qu}{N}$ whereas the asymptotic regret slope using the structure in item space is $\frac{\log N}{N}$ which is much smaller for $N$ being large. 

The algorithm uses some notation, which we define next. For an item $i$ and time $t>0$, $\rated_t(i) = \{u\in [N]: a_{u,s}= i \text{ for some } s<t\}$ is the set of users that have rated the item before time $t$. We use the notation $\rated(i)$ in the algorithm for $\rated_t(i)$ at the time it is used.
If $\ell\geq \thrjuu$ and a partitioning over users is formed, $\ratedtype_t(i)$ denotes the partitions from which a user has rated item $i$ by time $t$, \textit{i.e.,} $\ratedtype_t(i) = \{\tu\in [\qu]: a_{u,s}= i \text{ for some } s<t , u\in\Pc_{\tu}\}$. 

\begin{algorithm}
\caption{$\textsc{Joint}(T, \qi, \qu, N)$ (fixed time horizon)}\label{alg:joint-fixed}
\begin{algorithmic}[1]

\State $\ell$ chosen as Equation~\eqref{eq:ju-ellchoice}		
		\vspace{1mm}
\State $\thrjuu= 13\log N\qu^2$; $\thrjiu = 10\log N\qi^2$; $M=\lceil T\frac{64\qi}{\ell} \rceil$
\State $\Mcc{1} = M$  random items; $\Mcc{2} = M$  new random items;
		\vspace{1mm}
\State $\R_u\gets\varnothing,\quad u\in[N]$ \quad (items exploitable by user $u$)
\State $\{\R_u\}_{u\in [N]})\gets \textsc{ItemExplore}(\Mcc{1}, \Mcc{2}, \ell)$
\State $\textsc{ItemExploit}(\{\R_u\}_{u\in[N]})$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
	\caption{$\textsc{ItemExplore}(\Mcc{1}, \Mcc{2},\ell)$}\label{alg:joint-itemExplore}
	\begin{algorithmic}[1]
		\State $\S_\ti\gets\varnothing, \quad \ti\in[\qi]$ \quad (initialize sets of items of type $j$)
\vspace{2mm}
		\Statex \emph{Rate items by a few users (preliminary exploration)}
\State Recommend each item in $\Mcc{1}$ and $\Mcc{2}$ to $\thrjiu$ users  (This is done over $\lceil{(|\Mcc{1}|+|\Mcc{2}|)\thrjiu}/{N}\rceil< 2M\thrjiu/N+1$ time-steps, with extra recommendations being random new items.)
		\vspace{2mm}
		\Statex \emph{Partition items and learn item types (joint exploration, oblivious to user structure)}
		\For{$\ti=1,\cdots,\min\{\ell,\thrjuu\}$ \textbf{if} $\Mcc{1}\neq \varnothing$} 
		\State $\rep_\ti \gets$ a random item in $\Mcc{1}$ (representative item)
		\State $a_{u,t}\gets \rep_\ti$ if $u\notin\rated_t(\rep_{\ti})$, otherwise a random item not from $\Mcc{1}$. 
		\State $\widetilde{\S}_{\ti}\gets \{i\in \Mcc{1}: U = \rated(i)\cap \rated(\rep_{\ti}), L_{U, i} = L_{U,\rep_\ti}\}$
			\State $\Mcc{1}\gets\Mcc{1}\setminus \widetilde{\S}_{\ti}$ 
		\EndFor
	\vspace{.2cm}
		\Statex \emph{Partition users and learn item types (joint exploration with user structure)}
	\If{$\ell>\thrjuu$}
	\State Partition users into fewest possible groups such that each group agrees on all items.  Let $\tauh_U(u)\in [\qu]$ be the label of user $u$'s partition.
	\State $\Pc_{\tu}= \{u\in[N]:\tauh_U(u)=\tu\},\quad \forall \tu\in[\qu]$
	\For{$\ti=\thrjuu+1,\cdots,\ell$ \textbf{if} $\Mcc{1}\neq \varnothing$} 
		\State $\rep_\ti \gets$ a random item in $\Mcc{1}$ (representative item)
		\State $a_{u,t}\gets \rep_\ti$ if $\forall u'\in\Pc_{\tauh_U(u)}, u'\notin\rated_t(\rep_{\ti})$. (no user in the same partiotion of $u$ has rated $\rep_{\ti}$ before)
		\State $\widetilde{\S}_{\ti}\gets\{i\in \Mcc{1}: V = \ratedtype(i)\cap \ratedtype(\rep_{\ti}), L_{V, i} = L_{V,\rep_\ti}\}$
		\State $\Mcc{1}\gets\Mcc{1}\setminus \widetilde{\S}_{\ti}$ 
		\EndFor
	\EndIf
\vspace{.1cm}
\For{$\ti=1,\cdots,\ell$}
		\State $\S_\ti \gets \{i\in \Mcc{2}: V = \ratedtype(i)\cap \ratedtype(\rep_{\ti}), L_{V, i} = L_{V,\rep_\ti}\}$ \quad% (users agree on $i$ vs. $\rep_\ti$)
		\State $\Mcc{2}\gets \Mcc{2}\setminus \S_\ti$
		\EndFor
		\State $\R_u = \bigcup_{j:L_{u,\rep_\ti}=+1} \S_j$ for each $u\in [N]$
		\If{$u\in\Pc_{\tu}$ for some $\tu$}
\vspace{.1cm}
\State $\R_u =
		\bigcup_{u'\in\Pc_{\tu}} \bigcup_{j:L_{u',\rep_\ti}=+1} \S_j$ for each $u\in [N]$
		\EndIf
	\end{algorithmic}
\Return $\{\R^{s}_u\}_{u\in [N]}$
\end{algorithm}


\begin{algorithm}
	\caption{$\textsc{Exploit} \{\R_u\}_{u\in [N]}$}\label{alg:jointExploit}
	\begin{algorithmic}[1]
\For{ remaining $ t \leq T $}
\For{$u\in U $}
\If{there is an item $i \in\R_u$ such that $u\notin \rated_t(i)$.} 
\State $a_{u,t}\gets i$ 
\Else  { } $a_{u,t} \gets$ a random item not yet rated by $u$.
\EndIf
\EndFor
\EndFor
	\end{algorithmic}
\end{algorithm}

\section{Performance analysis}

\begin{thm}\label{t:joint-Upper}
Choosing the parameter $\ell$ as follows: 
\begin{align}\label{eq:ju-ellchoice}
\ell=\begin{cases} 
\qi, \quad  & \text{ if }\,\,\sqrt{\frac{200\qi\thrjiu}{\qu}T}> \qi\\ 
\sqrt{\frac{200\qi\thrjiu}{\qu}T}, \quad  & \text{ if }\,\,\thrjuu> \sqrt{\frac{200\qi\thrjiu}{N}T} \,\,\text{ and } \sqrt{\frac{200\qi\thrjiu}{\qu}T} \leq \qi\\
\sqrt{\frac{200\qi\thrjiu}{N}T}, \quad  & \text{ if }\,\, 8\log T\leq  \sqrt{\frac{200\qi\thrjiu}{N}T} \leq \thrjuu\\
8\log T, \quad  & \text{ if }\,\, 8\log T>  \sqrt{\frac{200\qi\thrjiu}{N}T},
\end{cases}
\end{align}
let $\thrjiu = 10\log (N\qi^2)$ and $\thrjuu = 13\log (N\qu^2)$.  Algorithm \ref{alg:joint-fixed} obtains regret per user at time $T$ upper bounded as
\begin{align*}
\reg(T)\leq\begin{cases} 
8 + \thrjuu + \frac{\qu}{N}(\qi-\thrjuu) + 200\frac{\qi\thrjiu}{N}T, \quad  & \text{ if }\,\,\sqrt{\frac{200\qi\thrjiu}{\qu}T}> \qi\\ 
8  + \thrjuu(1-\qu/N) + 2\sqrt{200\frac{\qu\qi\thrjiu}{N}T}, \quad  & \\
\hspace{4cm}\text{ if }\,\,\thrjuu> \sqrt{\frac{200\qi\thrjiu}{N}T}& \text{ and } \sqrt{\frac{200\qi\thrjiu}{\qu}T} \leq \qi\\
8 + 2\sqrt{\frac{200\qi\thrjiu}{N}T}, \quad  & \text{ if }\,\, 8\log T\leq  \sqrt{\frac{200\qi\thrjiu}{N}T} \leq \thrjuu\\
8\log T, \quad  &\text{ if }\,\, 8\log T >  \sqrt{\frac{200\qi\thrjiu}{N}T}\,.
\end{cases}
\end{align*}
\end{thm}


\begin{proof}

The basic error event is misclassification of an item or some users.

\paragraph{Item misclassification:}

 In Algorithm~\ref{alg:joint-itemExplore}, $\S_\ti$ is the set of items which the algorithm posits are of type $j$ (i.e., of the same type as the $j$th representative $\rep_\ti$). 
Let $\EE_i$ be the event that item $i$ was misclassified, 
		\begin{equation}\label{e:ju-EE}
		\EE_i = \{\exists \ti : i\in\S_\ti, \tau_I(i)\neq \tau_I(\rep_\ti)\}\,.
		\end{equation}
		In Lemma \ref{l:ju-item-mis-pr}, we will find an upper bound for probability of $\EE_i$.% and deviation bounds for total number of misclassified items in the algorithm. 
		To do so, one should carefully distinguish slightly different proof techniques for items classified before and after partitioning the user space, as any error in partitioning the user space increases the probability of errors in classification of items. 
		
		\paragraph{User misclassification}
	We bound the probability that the partitioning over  users created by the algorithm is incorrect: Let $\Bcal$  (defined in Equation~\eqref{e:ju-bcal-u-v} and~\eqref{e:ju-bcal}) be the event that the partitioning over the users is correct according to the type of users. Note that if $\ell<\thrjuu,$ the algorithm does not partition the users. In this case, we defined $\Bcal$ in Equation~\eqref{e:ju-bcal} such that $\Bcal$ holds. According to Lemma \ref{l:ju-user-mis-pr} $\Pr[\Bcal^c]\leq 2/N^2$.
	
	Also, according to the model introduced in Section \ref{sec:model}, users of the same type rate all items similarly all the time. So, the only error that can happen in partitioning the users is when two or more distinct user types rate the first $\thrjuu$ representative items similarly. In this case, the users from these user types are not distinguishable from each other. Consequently, users of the same type are always in the same partition whether or not $\Bcal$ holds.
		
		
\paragraph{Categorization of recommendations:}	The amount of time a user $u$ spends in the exploration phase (Step~1 of the algorithm) is denoted by $\Tu(u)$. %Note that $\Tu(u)$ is a random variable which depends on the feedback to the algorithm.

To bound regret (the expected number of bad recommendations), we partition the set of recommendations made by the algorithm according to: 1-whether or not recommendation was in the exploration phase; 2-whether or not the item is in the list of exploitable items $\R_u$; 3-whether or not the item misclassification event $\EE_{a_{u,t}}$ occurs; and 4-whether or not the partitioning over the users is correct ($\Bcal^c$ holds).
\newpage
\begin{align}
N\reg(T) & \leq   \Exp{ \sum_{u=1}^N\sum_{t=1}^{\Tu(u)} \ident[L_{u,a_{u,t}}=-1]}\notag\\
& \quad +   \Exp{ \sum_{u=1}^N\sum_{t=\Tu(u)+1}^T  \ident[L_{u,a_{u,t}}=-1, a_{u,t}\notin\R_u]}\notag\\
& \quad +  \Exp{ \sum_{u=1}^N\sum_{t=\Tu(u)+1}^T  \ident[L_{u,a_{u,t}}=-1, a_{u,t}\in\R_u, \Bcal]}\notag\\
& \quad +  \Exp{ \sum_{u=1}^N\sum_{t=\Tu(u)+1}^T  \ident[L_{u,a_{u,t}}=-1, a_{u,t}\in\R_u, \EE_{a_{u,t}}]}\notag\\
& \quad +  \Exp{ \sum_{u=1}^N\sum_{t=\Tu(u)+1}^T \ident[L_{u,a_{u,t}}=-1, a_{u,t}\in\R_u, \EE_{a_{u,t}}^c, \Bcal^c]} \notag\\
& =: \Asf{1} + \Asf{2} + \Asf{3} +\Asf{4} +\Asf{5} \,. \label{eq:ju-reg-decomp}
\end{align}
%\MK{I didn't change the appearance of summations as I wanted to emphasize that $t\in[\Tu{u}:T]$. We should make it look better at some point. But it's not clear how.}

\begin{itemize}[leftmargin=*]
  \item[--] $\Asf{1}$ is the regret from early time-steps before $\Tu(u)$. We control the value of $\Tu(u)$ by studying the exploration exploitation tradeoff in the design and analysis of the algorithm. Proper choice of the parameter $\ell$ has an important role in bounding this term.
  \item[--] $\Asf{2}$ is the regret due to not having enough items available for the exploitation phase, which is proved to be small with high probability for a good choice of $M$. 
  \item[--] $\Asf{3}$ is the regret due to the error in partitioning the users. This will be small with proper choice of $\thrjuu$.
\item[--] $\Asf{4}$ is the regret due to exploiting the misclassified items. It will be small because few items are misclassified as a result of proper choice of $\thrjiu$. 
\item[--] $\Asf{5}$  is the regret due to exploiting correctly classified items under the correct partitioning of the users and we 
will see that $\Asf{5}=0\,.$
\end{itemize}
In Equation~\eqref{eq:ju-reg-decomp}, we provide an upper bound for regret as we are double counting the recommendations in which not only the partitioning on user structure is incorrect, but also the recommended item is also misclassfieid. The probability of this event is  small so that using this upper bound does not make the analysis less relevant.  

\paragraph{Bounding $\Asf{1}.$}
It takes at most $\lceil\frac{2M\thrjiu}{N}\rceil$ units of time to rate each item in $\Mcc{1}$ and $\Mcc{2}$ by $\thrjiu$ users (since intially $|\Mcc{1}|=|\Mcc{2}|=M$ and later some items are removed from $\Mcc{1}$ and $\Mcc{2}$). 

At each iteration $\ell$  representative items from different item types are rated by either all users (if $\ell<\thrjuu$) or one user from each partition of users (if $\ell\geq \thrjuu$). Let $W_{\tu}$ be the set of users with type $\tu$ and $w_{\tu}=|W_{\tu}|$
\begin{equation}\label{eq:ju-wk-def}
W_{\tu}=\{u:\tau_U(u)=\tu
\}, \quad \text{and}\quad w_{\tu}=|\{u:\tau_U(u)=\tu\}|\,.
\end{equation}

\begin{itemize}
\item So, if $\ell<\thrjuu,$ user $u$ rates at most $\lceil\frac{2M\thrjiu}{N}\rceil$ items in step 2 and $\ell$ items in step 5 of \textsc{ItemExplore} algorithm (Algorithm \ref{alg:joint-itemExplore}) .
\begin{equation}\label{eq:ju-Tou-small-ell}
\Tu(u)\leq  \left\lceil\frac{2M\thrjiu}{N}\right\rceil + \ell \leq \frac{2M\thrjiu}{N}+ (\ell+1)\,. 
\end{equation}


\item If $\ell\geq \thrjuu,$ for given user type $\tu\in[\qu], $ all the users in $W_{\tu}$ rate the first $\thrjuu$ representative items at each iteration they go through. The remaining $\ell-\thrjuu$ representative items are rated by at most one user in $W_{\tu}$. To see this, remember that we showed all the users of the same type end up in the same partition. But if the user partitioning is incorrect, there might be users from more than one user type in a partiotion. Since one user from each partition rate remaining $\ell-\thrjuu$ representative items, at most one user from $W_{\tu}$ rates each of them. Hence, 
\begin{align}
\sum_{u\in W_{\tu}}\Tu(u) & \leq \sum_{u\in W_{\tu}}\left(\left\lceil\frac{2M\thrjiu}{N}\right\rceil + \thrjuu\right) + (\ell-\thrjuu)
\leq  w_{\tu}(\frac{2M\thrjiu}{N}+ 1+\thrjuu) + \ell-\thrjuu\,. \label{eq:ju-Tou-large-ell}
\end{align}
\end{itemize}
%Define $\R_u^{(s)}$ to be the set $\R_u$ by the end of $s-$th time user $u$ goes through Exploration phase of the algorithm. 
Hence, if $u\in\Pc_{\tu},$
\begin{equation}
\label{e:ju-Ru-s}
\R_u=\bigcup_{u': u'\in\Pc_{\tu}}\bigcup_{\ti\in [\ell]\atop L_{u',\rep_{\ti}}=+1} \S_{\ti}
\end{equation}
Note that if $\ell<\thrjuu$ and there is no partitioning, then $\R_u=\cup_{\ti\in [\ell]\atop L_{u,\rep_{\ti}}=+1} \S_{\ti}.$


At $t\leq \Tu(u)\,,$ the algorithm recommends random items to $u$. Since each item $i$ has a uniformly distributed type $\tau_I(i)$, any given user likes item type $\ti$ with probability half. 
For $\ell<\thrjuu,$
\begin{align}
2 \Asf{1} & = 2 \Ex{\sum_{u=1}^N \sum_{t=1}^{\Tu(u)} \ident[L_{u,a_{u,t}}=-1]}\notag = \Ex\sum_{u=1}^N \Tu(u) \notag\\
&{\leq} \bigg(\bigg\lceil\frac{2M\thr}{N}\bigg\rceil+\ell\bigg) N{\leq} 2M\thr + (\ell+1)N \,,\label{eq:ju-bound-A1-ell-small}
\end{align}
where we used Equation~\eqref{eq:ju-Tou-small-ell}.

For $\ell\geq \thrjuu,$
\begin{align}
2\Asf{1} & = \Ex\sum_{u=1}^N \Tu(u)  = \Ex\sum_{k\in[\qu]}\sum_{u\in W_{\tu}} \Tu(u)  \notag\\
&\overset{(a)}{\leq} \Ex\sum_{k\in[\qu]}[ w_{\tu}(\frac{2M\thrjiu}{N}+ 1+\thrjuu) + \ell-\thrjuu]\notag\\
&
\overset{(b)}{\leq} N(\frac{2M\thrjiu}{N}+ 1+\thrjuu) + \qu(\ell-\thrjuu)\label{eq:ju-bound-A1-ell-large}
\end{align}
Here (a) is obtained by Equation~\eqref{eq:ju-Tou-large-ell}. Definition of $w_{\tu}$ in Equation~\eqref{eq:ju-wk-def} gives (b).


\paragraph{Bounding $\Asf{2}$.}
According Algorithm \ref{alg:jointExploit}, user $u$ is recommended a new random item at $t\geq \Tu(u)$ if  there is no available items in $\R_u$ to recommend to it. Hence, for every $u\in[N]$ at these times
$\Pr[L_{u,a_{u,t}}=-1| a_{u,t}\notin \R_u]= \frac{1}{2}\,.$ Also, an item $a_{u,t}\notin \R_u$ is recommended to $u$ in Algorithm  \ref{alg:jointExploit} only when all items in $\R_u$ have been recommended to this user before. So, the total number of times $a_{u,t}\notin \R_u$ is recommended at time interval $\Tu(u)\leq t\leq T\,,$ is at most $(T-|\R_u|)_+$. To observe that, note that if $|\R_u|\geq T\,,$ then there are enough items in $\R_u$ up until time $T$, in which case $\sum_{t=\Tu(u)+1}^T \ident[ a_{u,t}\notin \R_u] = 0$. Alternatively, if $|\R_u| < T\,,$ then there will be at most $(T-|\R_u|)$ times that user $u$ is recommended an item $a_{u,t}\notin\R_u$, which implies that $\sum_{t=\Tu(u)+1}^T \ident[ a_{u,t}\notin \R_u] \leq (T-|\R_u|)_+\,.$ Hence, 
\begin{align*}
\Asf{2} &= \sum_{u\in[N]} {\sum_{t=\Tu(u)+1}^T \Pr[L_{u,a_{u,t}}=-1, a_{u,t}\notin \R_u]} \\
& =  
  \sum_{u\in [N]}  {\sum_{t=\Tu(u)+1}^T \frac{1}{2}\Pr[ a_{u,t}\notin \R_u]}
\leq \sum_{u\in [N]} \frac{1}{2}\Exp{(T -|\R_{u} |)_+}\,.
\end{align*}
Using Lemma \ref{l:ju-exp-R-u}, we get
 \begin{equation}\label{eq:ju-bound-A2}
\Asf{2} \leq 2TN\exp(-\frac{\ell}{8})+ \frac{32 T}{\ell}
\end{equation}
\paragraph{Bounding $\Asf{3}$.}
Term $\Asf{3}$ in Equation \eqref{eq:ju-reg-decomp} is the regret due to the misclassification of users. Using Lemma \ref{l:ju-user-mis-pr}, we know that the probability of having any error in partitioning the users is at most $2/N^2$. Hence,
\begin{align}
	\Asf{3}& = \Ex{\sum_{u=1}^N \sum_{t=\Tu{u}+1}^T \ident[L_{u,a_{u,t}}=-1, a_{u,t}\in\R_u, \BB]} \notag\\
&	\leq  \Ex{\sum_{u=1}^N \sum_{t=\Tu{u}+1}^T \ident[a_{u,t}\in\R_u, \BB]}\, {\leq} \, \frac{2}{N}T\label{eq:ju-bound-A3}
\end{align}
where the last inequality is proved in Lemma \ref{l:ju-user-mis-pr}.

\newpage
\paragraph{Bounding $\Asf{4}$.}
Term $\Asf{4}$ in Equation \eqref{eq:ju-reg-decomp} is the expected number of mistakes made by the algorithm as a result of item misclassifications. Lemma \ref{l:ju-item-mis-pr}  upper bounds the expected number of ``potential item misclassifications'' in the algorithm to provide an upper bound for this value: 
\begin{align}
	\Asf{4}& = \Ex{\sum_{u=1}^N \sum_{t=\Tu(u)+1}^T \sum_{i\in\mathbb{N}} \ident[L_{u,i}=-1, a_{u,t}=i, i\in\R_u, \EE_i]}\notag\\
	& \leq  \Ex{\sum_{u=1}^N \sum_{t=\Tu(u)+1}^T \sum_{i\in\mathbb{N}} \ident[a_{u,t}=i, i\in\R_u, \EE_i]}\notag\\
	& \overset{(a)}{=} \Ex{\sum_{u=1}^N \sum_{t=\Tu(u)+1}^T \sum_{i\in\Mcc{2}} \ident[a_{u,t}=i, i\in\R_u, \EE_i]}\notag\\
	& \overset{(b)}{\leq}  N\Exp{\sum_{i\in\Mcc{2}} \ident[\EEb_{i,U_i}]} \leq N M \max_{i\in\Mcc{2}}\Pr[\EE_{i}]
\overset{(c)}{\leq}  M \frac{3}{\qi}\,.\label{eq:ju-bound-A4}
\end{align}
Here (a) follows because for every user $u\,,$ the set of items $\R_u$ is a subset of $\Mcc{2}$;
(b) is true since each item $i$ is recommended at most $N$ times; (c) is proved in Lemma \ref{l:ju-item-mis-pr} that for any $i\in\Mcc{2}, \Pr[\EE_{i}]<3/(\qi N)$.




\paragraph{Bounding $\Asf{5}$.}
By the definition of event $\EE_i$ given in Equation~\eqref{e:EE}, if an item $i\in\S_{\ti}\,$ is not misclassified, then $\tau_I(i)=\tau_I(\rep_{\ti})$. By definition of the model, user preferences for an item depend only on the type of the item (since $L_{u,i} = \xi_{\tau_U(u),\tau_I(i)}$), so all users rate $i$ the same as $\rep_{\ti}\,.$ If an item $i\in\R_u$ we know that there is some $\ti$ such that $i\in\S_{\ti}$ and $u$ likes item $\rep_{\ti}\,.$
\begin{align}
\Pr[L_{u,i}=-1| i\in\R_u, \EE^c_i] &= \Pr[L_{u,i}=-1| \exists \ti: L_{u,\rep_\ti}=+1, i\in\S_{\ti}, \tau_I(i)= \tau_I(\rep_\ti)]\notag\\
& = \Pr[L_{u,i}=-1| \xi_{u,\tau_I(i)}=+1] =0\notag\\
& \Rightarrow \Asf{5} = 0\,.\label{eq:JU-bound-D}
\end{align}



\paragraph{Combining all the bounds.}
Plugging in Equation~\eqref{eq:IU-bound-A},~\eqref{eq:IU-bound-B},~\eqref{eq:IU-bound-C} and~\eqref{eq:IU-bound-D} into Equation~\eqref{eq:IU-reg-decomp} gives 
for $\ell\leq\thrjuu$
\begin{align*}
\reg(T) & \leq \frac{128 \qi\thrjiu}{\ell N}T+ 1+\ell + 2T\exp(-\frac{\ell}{8})+ \frac{32 }{\ell N}T+\frac{2}{N^2}T+\frac{19}{\ell N}T\\
&\leq \frac{200 \qi\thrjiu}{\ell N}T+ 1+\ell + 2T\exp(-\frac{\ell}{8})\,.
\end{align*}
and for $\ell>\thrjuu$
\begin{align*}
\reg(T) & \leq \frac{128 \qi\thrjiu}{\ell N}T+ 1+\thrjuu + \frac{\qu}{N}(\ell-\thrjuu)+2T\exp(-\frac{\ell}{8})+ \frac{32 }{\ell N}T+\frac{2}{N^2}T+\frac{19}{\ell N}T\\
&\leq \frac{200 \qi\thrjiu}{\ell N}T+ \frac{\qu}{N}\ell+ 2T\exp(-\frac{\ell}{8})+ 1+(1-\frac{\qu}{N})\thrjiu \,.
\end{align*}

The choice of $\ell$ in the algorithm gives the statement of the theorem.

\begin{align*}
\ell=\begin{cases} 
\qi, \quad  & \text{ if }\,\,\sqrt{\frac{200\qi\thrjiu}{\qu}T}\geq \qi\\ 
\sqrt{\frac{200\qi\thrjiu}{\qu}T}, \quad  & \text{ if }\,\,\thrjuu\leq \sqrt{\frac{200\qi\thrjiu}{N}T} \,\,\text{ and } \sqrt{\frac{200\qi\thrjiu}{\qu}T} \leq \qi\\
\sqrt{\frac{200\qi\thrjiu}{N}T}, \quad  & \text{ if }\,\, 8\log T\leq  \sqrt{\frac{200\qi\thrjiu}{N}T} \leq \thrjuu\\
8\log T, \quad  & \text{ if }\,\, 8\log T\geq  \sqrt{\frac{200\qi\thrjiu}{N}T}
\end{cases}
\end{align*}
gives 
\begin{align*}
\reg(T)\leq\begin{cases} 
8 + \thrjuu + \frac{\qu}{N}(\qi-\thrjuu) + 200\frac{\qi\thrjiu}{N}T, \quad  & \text{ if }\,\,\sqrt{\frac{200\qi\thrjiu}{\qu}T}\geq \qi\\ 
8  + \thrjuu(1-\qu/N) + 2\frac{\sqrt{200\qu\qi\thrjiu T}}{N}, \quad  & \text{ if }\,\,\thrjuu\leq \sqrt{\frac{200\qi\thrjiu}{N}T} \,\,\text{ and } \sqrt{\frac{200\qi\thrjiu}{\qu}T} \leq \qi\\
8 + 2\sqrt{\frac{200\qi\thrjiu}{N}T}, \quad  & \text{ if }\,\, 8\log T\leq  \sqrt{\frac{200\qi\thrjiu}{N}T} \leq \thrjuu\\
8\log T, \quad  &\text{ if }\,\, 8\log T \geq  \sqrt{\frac{200\qi\thrjiu}{N}T}\,.
\end{cases}
\end{align*}
\end{proof}%Theorem joint upper bound



%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Error probability in item classification}
For a sequence of labels of learned representative items $X_{1:m}=X_1,\cdots,X_m$, let

\begin{equation}\label{e:ju-EE-m}
	\EE_i(X_{1:m}) = \{\exists \ti\in\{X_{1:m}\} : i\in\S_\ti, \tau_I(i)\neq \tau_I(\rep_\ti)\}
\end{equation}
to be the event that item $i$ is misclassified after learning the first $m$ representative items. According to the definition of $\EE_i$ given in Equation~\eqref{e:ju-EE}, $\EE_i=\EE_i([\qi])\,.$

\begin{lemma}\label{l:ju-item-mis-pr}
Given $N$ large enough so that $\qu>10\thrjiu$,   for every item  $i\in\Mcc{2},$ the probability of mis-classifying item $i$ is upper bounded as $\Pr[\EE_i]\leq \frac{3}{\qi N}\,.$
	\end{lemma}
\begin{proof}
To bound the probability of misclassifying any item,  we look at items that were classified using the partitioning over the users ($i\in\S_{\ti}$ with $\ti\geq \thrjuu$) and the ones that were classified not using the partitioning over the users ($i\in\S_{\ti}$ with $\ti< \thrjuu$) separately. Hence, we study the error events $\EE_{i}([\thrjiu])$ and $\EE_{i}([\qi]\setminus[\thrjiu])$ separately.To do so, first we guarantee that there are enough distinct user types rating each item in the following claim:


%\begin{claim}
%\label{cl:ju-pr-Ei-cl1}
% For any $s,$  the number of distinct user types in $\U_s$ is at least $10\thrjiu$ with probability at least $1-\qu\exp(-\frac{N}{3\qu})$. 
%\end{claim}
%\begin{proof}
%To see that, note that according to the Algorithm \ref{alg:joint-fixed}, the number of users in $\U_s$ is at least $20\thrjiu \frac{N}{\qu}\,.$ Using the Chernoff bound given in Lemma \ref{l:Chernoff}, the maximum number of users with a given type is less than $\frac{2N}{\qu}$  with probability at least $1-\qu\exp(-\frac{N}{3\qu})$. Hence, there are at least $10\thrjiu$ distinct user types in $\U_s$ in any group of $10\thrjiu \frac{N}{\qu}$ users. 
%\end{proof}

\begin{claim}
\label{cl:ju-pr-Ei-cl2}
Given $N$ large enough so that $\qu>10\thrjiu$, the $\thrjiu$ users rating any item in $\Mcc{2}$ belong to at least $\frac{\thrjiu}{2}$ distinct user types with probability at least $1-\frac{1}{\qi N}$. 
\end{claim}
\begin{proof}
The choice of $\thrjiu$ users rating any item in $\Mcc{2}$ is independent of the feedback. For given item $i$ and $m\in[\thrjiu]$ let $X_m$ be a binary valued random variable which denotes whether the $m-$th user which rates item $i$ is from a new user type or not. We are interested to find an upper bound for $\Pr[\sum_{m=1}^{\thrjiu} X_i <\frac{\thrjiu}{2}]$. To do so, note that $\Pr[X_m=1 | \sum_{m'=1}^{m-1} X_{m'}=d]\geq 1-\frac{d}{\qu}$, this is a direct consequence of the uniform prior distribution of user types over users. Since we are interested in $\Pr[\sum_{m=1}^{\thrjiu} X_i <\frac{\thrjiu}{2}]$, we know that the sequence of random variables $X_m$ stochastically dominates an i.i.d. binary-valued random variable with mean $\frac{19}{20}\,.$ Hence, $\Pr[\sum_{m=1}^{\thrjiu} X_i <\frac{\thrjiu}{2}]\leq \exp(-\frac{\thrjiu}{10}) \leq \frac{1}{\qi N}\,.$
\end{proof}

\begin{claim}\label{cl:ju-pr-Ei-cl3}
For item $i\in\S_{\ti}$, such that $\ti<\thrjuu,$ we have $\Pr[\EE_i]\leq \frac{3}{\qi N}$, \textit{i.e.,}
$$\Pr\big[\,\EE_i([\thrjuu])\,\big]\leq \frac{2}{\qi N}\,.$$
\end{claim}

\begin{proof}
For item $i\in\Mcc{2}$ and subset of users $U_i\subseteq [N]\,,$ define 
\begin{equation}\label{e:ju-EEbu-def}
\EEb_{i,U_i} =\{\exists \ti\neq \tau_I(i): L_{u,i}=\xi_{\tau_U(u),\ti}\,, \forall u\in U_i\}
\end{equation} to be the event that the ratings of users in $U_i$ for item $i$ agree with a different type. 
For item $i\in\S_{\ti}$, such that $\ti<\thrjuu,$ we know that item $i$ was added to $\S_{\ti}$ since some groups of users of size $\thrjiu$ have rated $i$ and $\rep_{\ti}$ similarly. 
Let $t$ be the time $i$ was added to $\S_{\ti}$ in the exploration phase. Let $U_i=\rated_t(i)\cap\rated_t(\rep_{\ti})$ be the set of users whose ratings verified that $i$ and $\rep_{\ti}$ are of the same type. All users in $U_{i}$ agree on $i$ vs. $\rep_{\ti}$. Hence, if item $i\in \S_{\ti}$ is misclassified (which implies $\tau_I(i)\neq \tau_I(\rep_{\ti})$ using Equation~\eqref{e:EE}), then $\EEb_{i,U_i}$ holds. So, $\EE_i\subseteq\EEb_{i,U_i}\,.$

Using the statement of Claim\ref{cl:ju-pr-Ei-cl2}, there are at least $\thrjiu/2$ users with distinct user types who rate both item $i\in\S_{\ti}$ and $\rep_{\ti}$.
A set of $\thrjiu/2$ users with distinct types, chosen independently of the feedback, rate item $i$ of type $\tau_{I}(i)$. Any two item types $j\neq j'$ have jointly independent user preferences $(\xi_{u,j})_{u\in [N]}, (\xi_{u,j'})_{u\in [N]}$, so two items of different types are rated in the same way by the $\thrjiu/2$ users of distinct types with probability at most $2^{-\thrjiu/2}$. The choice $\thrjiu=10\log({N\qi^2})$ and a union bound over item types $\ti$  gives  that conditional on the fact that $U_i$ contains at least $\thrjiu/2$ distinct user types, $\Pr[\EEb_{i,U_i}]\leq \frac{1}{\qi N}.$ Plugging in the statement of Claim \ref{cl:ju-pr-Ei-cl2} gives
$\Pr\big[\,\EE_i([\thrjuu])\,\big]\leq \frac{2}{\qi N}\,.$
\end{proof}


\begin{claim} \label{cl:ju-pr-Ei-cl4}
For item $i\in\S_{\ti}$, such that $\ti\geq\thrjuu,$ we have $\Pr[\EE_i]\leq \frac{3}{\qi N}$, \textit{i.e.,}
\[\Pr\big[\,\EE_i([\qi]\setminus[\thrjuu])\,\big]\leq \frac{3}{\qi N}\]
\end{claim}
\begin{proof}
For an item $i\in\Mcc{2}$ and a subset of user types $V_i\subseteq[\qu],$ define 
\begin{equation}
\label{e:ju-EEbv-def}
\EEb_{i,V_i}=\{\exists \ti\neq\tau_I(i): \xi_{\tu,\tau_I(i)} = \xi_{\tu,\ti}, \forall \tu\in V_i\}
\end{equation}
to be the event that the ratings of users with types in $V_i$ for item $i$ agrees with a different type. For item $i\in\S_{\ti}$, such that $\ti\geq\thrjuu$ we know that $i$ was added to $\S_{\ti}$ because  according to the partitioning made over the users, items $i$ and $\rep_{\ti}$ are rated similarly. 

We will provide the upper bound on probability of error $\EE_i$ conditional on $\Bcal$ (the partitioning over the users is correct). Note that in Lemma \ref{l:ju-user-mis-pr} it is shown that $\Pr[\Bcal^c]<2/N^2$. But this bound is provided conditional on statement of Claim \ref{cl:ju-pr-Ei-cl3}. 


Let $\Bcal^c$ holds. 
Let $t$ be the time $i$ was added to $\S_{\ti}$ in the exploration phase. Let $V_i=\ratedtype_t(i)\cap \ratedtype_t(\rep_{\ti})$ be the set of user types whose ratings verified that $i$ and $\rep_{\ti}$ are of the same type. Hence, if item $i\in\S_{\ti}$ is misclassified (which implies $\tau_I(i)\neq \tau_I(\rep_{\ti})$ using Equation~\eqref{e:ju-EE}), then $\EEb_{i,V_i}$ holds. So, $\EE_i\subseteq\EEb_{i,V_i}$ which implies $\Pr[\EE_i]\leq \Pr[\EEb_{i,V_i}]$.

Next, we will show that the probability of $\EEb_{i,V_i}$ is small. To see that, we use Claim \ref{cl:ju-pr-Ei-cl2} that $V_i$ contains at least $\thrjiu/2$ distinct user types with high probability.

The probability of the event $\EEb_{i,V_i}$ is upper bounded as $\Pr[\EEb_{i,V_i}]\leq $
Any two item types $j\neq j'$ have jointly independent user-type preferences $(\xi_{\tu,j})_{\tu\in [\qu]}, (\xi_{\tu,j'})_{\tu\in [\qu]}$, so two items of different types are rated in the same way by the $\thrjiu/2$ distinct user types with probability at most $2^{-\thr/2}$. The choice $\thrjiu=10\log(N{\qi^2})$ and a union bound over item types $\ti$, $\Pr[\EEb_{i,V_i}|\Bcal]\leq \qi 2^{-\thrjiu/10}\leq \frac{1}{\qi N}\,.$ Plugging in Claim \ref{cl:ju-pr-Ei-cl2} gives
\[\Pr[\EE_i]\leq \frac{2}{\qi N}+ \Pr[\Bcal]\,.\]
Using the fact that $\Pr[\Bcal]<2/N^2$ and $\qu=N^\alpha,$ for $N>N_0(\alpha),$  we have $\Pr[\EE_i]<\frac{3}{\qi N}\,.$
\end{proof}

Claims \ref{cl:ju-pr-Ei-cl3} and \ref{cl:ju-pr-Ei-cl4} give the statement of lemma.
\end{proof}
 

\subsection{Error probability in user classification }

\begin{definition}
 For user types $\tu$ and $\tu',$ let \begin{equation}\label{e:ju-bcal-u-v}
	\Bcal_{\tu, \tu'}= 
\left\{\ident[\tauh_U(u)=\tauh_U(v)] = \ident[\tu = \tu'], \text{ for all } u,v \text{ such that } \tau_U(u)=\tu \text{ and } \tau_U(v)=\tu'\right\}
	\end{equation} be the event that user types $\tu$ and $\tu'$ are partitioned correctly with respect to each other in Algorithm \ref{alg:joint-itemExplore}.
	Let \begin{equation}\label{e:ju-bcal}
	\Bcal=\cap \Bcal_{\tu,\tu'}
\end{equation} be the event that the partitioning over the users match the partitioning induced by user types.
\end{definition}


\begin{lemma}
\label{l:ju-user-mis-pr}
Probability of not distinguishing two user types $\tu$ and $\tu'$ in the partitioning over the users made by the algorithm is upper bounded as $\Pr[(\Bcal_{\tu,\tu'})^c]\leq 2/(N\qu^2)^2$. It follows that the partitioning over the users is correct with probability at least $\Pr[\Bcal^c]\leq 2/N^2.$
\end{lemma}

\begin{proof}
Distinct user types $\tu$ and $\tu'$ are distinguished in the partitioning made by the algorithm if there is at least one  item among the first $\thrjuu$ representative items which is rated differently by user types $\tu$ and $\tu'$. Knowing that the elements of matrix $\Xi$ are i.i.d., it would be easy to find the probability of this event happening if the representative items were drawn  uniformly at random.

 But unfortunately, this is not the case: At each step, the choice of the next item type depends on the proportion of number of items of a given item type among the remaining items in $\Mcc{1}$. Hence, item of an item types which are more probable to be misclassified are less likely to be chosen as the representative items (as most items of these types are misclassified and already removed from $\Mcc{1}$). Hence, there is statistical dependence between matrix $\Xi$ and the choice of representative items. 
 
 To solve this problem, let $\Xi_{\tu,\cdot}$ and $\Xi_{\tu',\cdot}$ be the $\tu$ and $\tu'-$th rows of matrix $\Xi$. We bound the probability of choosing any specific sequence of distinct item types as the first $\thrjuu$ representatives conditional on fixed $\Xi_{\tu,\cdot}$ and $\Xi_{\tu',\cdot}$. Then we show that with high probability, there are more than $\qi/3$ item types which distinguish $\tu$ and $\tu'$. Conditional on this property of matrix $\Xi\,,$ with high probability there is at least one item among the first $\thrjuu$ learned representative items which distinguish $\tu$ and $\tu'$.



Let $X_m=\tau_I(\rep_m)$ be the item type of the $m-$th representative item.  For given user types $\tu$ and $\tu'$, we want to find the probability that both user types $\tu$ and $\tu'$ rate all item types $X_1, \cdots, X_{\thrjuu}$ similarly. To do so, given $X_1, \cdots, X_{m-1}$ for $m<\thrjuu$, $\Xi_{\tu,\cdot}$ and $\Xi_{\tu',\cdot}$ we find the conditional probability of choosing item type $X_m$ as the next type to learn.
 

Let $\Lc_{\tu,\tu'}=\{\ti: \xi_{\tu,\ti}\neq\xi_{\tu',\ti}\}$ be the set of item types who are rated differently by user types $\tu$ and $\tu'$. Hence, the event $\Bcal_{\tu,\tu'}$ holds if there is some $m\in[\thrjuu],$ so that $X_m\in\Lc_{\tu,\tu'}$ (there is at least one learned item type among the ones that are  helpful in distinguishing $\tu$ and $\tu'$). Hence, we want to show an upper bound for
\begin{equation}
\label{eq:ju-Bkc-bound}
\Pr[(\Bcal_{\tu,\tu'})^c]= \Pr\big[\,X_m\notin\Lc_{\tu,\tu'}, \text{ for all } m\in[\thrjuu]\,\big]\,.
\end{equation}

Since the elements of matrix $\Xi$ are independently  $\mathrm{Bern}(1/2)$ distributed, using Chernoff bound in Lemma \ref{l:Chernoff},
\begin{equation}\label{eq:ju-Lkkprime-bd}
\Pr[|\Lc_{\tu,\tu'}|<\qu/3 ]\leq \exp(-\qu/18)\,.
\end{equation}
Note that the set $\Lc_{\tu,\tu'}$ is a function of $\Xi_{\tu,\cdot}$ and $\Xi_{\tu',\cdot}$.
Define $\Rb(\ti)$ to be the set of items in $\Mcc{1}$ of type $\ti$
\begin{equation}
\label{eq:ju-Rb2}
\Rb(\ti)= \{i\in\Mcc{1}:\tau_I(i)=\ti\}\,.
\end{equation}

Define the error event $\EEt_i$ for $i\in\Mcc{1}$ similar to the event $\EE_i$ for $i\in\Mcc{2}$ given in Equation~\eqref{e:EE} so that 
\begin{equation}
\label{eq:ju-EEt-m}
	\EEt_i(X_1,\cdots,X_m) = \{\exists \ti\in\{X_1,\cdots,X_m\} : i\in\widetilde{\mathcal{S}}_\ti, \tau_I(i)\neq \tau_I(\rep_\ti)\}\,.
\end{equation}
to be the event item $i\in\Mcc{1}$ is miscategorized into one of the representative item types labeled by $X_1,\cdots,X_m$. Let $\EEt_i = \EEt_i([\qi])$ to be the error event associated with item $i\in\Mcc{1}$.

\begin{definition}\label{def:ju-iuerr}
Let  $\iuerr(X_1,\cdots,X_m)$, be the event such that on this event, for any item type $\ti$, at most $1/10-$th fraction of  items in $\Mcc{1}$ of type $\ti$ are misclassified into partitions corresponding to representative items labeled by $X_1,\cdots,X_m$. We use the notation introduced in Equation \ref{eq:ju-EEt-m} to define:
\begin{equation}
\iuerr(X_1,\cdots,X_m) = \left\{\,\sum_{i\in\Rb(\ti)}\ident[\EEt_i(X_1,\cdots,X_m)]\leq \frac{|\Rb(\ti)|}{10}, \text{ for all } \ti\in[\qi]\,\right\}.
\end{equation}
Let $\iuerr=\iuerr([\qi])$.
\end{definition}


Using the total probability lemma, for any fixed value of $\Xi_{\tu,\cdot}$ and $\Xi_{\tu',\cdot}$: 
\begin{align}
 \Pr\bigg[\sum_{i=1}^{\thrjuu}\ident&\big[\,X_i\in\Lc_{\tu,\tu'}\,\big]< 1 \, \bigg|\, \Xi_{\tu,\cdot},\Xi_{\tu',\cdot}, |\Lc_{\tu,\tu'}|\geq \qi/3\bigg] \notag\\
&\leq \Pr\bigg[\sum_{i=1}^{\thrjuu}\ident[X_i\in\Lc_{\tu,\tu'}]< 1 \, \bigg|\, \iuerr([\thrjuu]), \Xi_{\tu,\cdot},\Xi_{\tu',\cdot}, |\Lc_{\tu,\tu'}|\geq \qi/3\bigg]\notag\\
& \quad+ \Pr\big[\,\iuerr^c([\thrjuu])\,\big|\, \Xi_{\tu,\cdot},\Xi_{\tu',\cdot}, |\Lc_{\tu,\tu'}|\geq \qi/3\,\big]\,.
\end{align}

Application of Claim \ref{cl:ju-err-event-M1} provides an upper bound for the second term on the right hand side of above display. 
Lemma \ref{l:sum-rep-Lkkprime} provides the upper bound for the first term for all $\Xi_{\tu,\cdot}$ and  $\Xi_{\tu',\cdot}$ such that $|\Lc_{\tu,\tu'}|\geq \qi/3$ (remember that $\Lc_{\tu,\tu'}$ is a deterministic function of the $\tu$ and $\tu'-$th rows of matrix $\Xi$). Hence, 
\[\Pr\bigg[\sum_{i=1}^{\thrjuu}\ident\big[\,X_i\in\Lc_{\tu,\tu'}\,\big]< 1 \, \bigg|\, \Xi_{\tu,\cdot},\Xi_{\tu',\cdot}, |\Lc_{\tu,\tu'}|\geq \qi/3\bigg] \leq \frac{1}{N\qu^2}\]

Taking the expectation of the the above inequality with respect to $\Xi_{\tu,\cdot}$ and  $\Xi_{\tu',\cdot}$ condition on $|\Lc_{\tu,\tu'}|\geq \qi/3$ gives 

\[\Pr\bigg[\sum_{i=1}^{\thrjuu}\ident\big[\,X_i\in\Lc_{\tu,\tu'}\,\big]< 1 \, \bigg|\,  |\Lc_{\tu,\tu'}|\geq \qi/3\bigg] \leq \frac{1}{N\qu^2} +\frac{40}{\qi^4 N^{10}}\]
Plugging Equation~\eqref{eq:ju-Lkkprime-bd} gives an upper bound for the right term in Equation~\eqref{eq:ju-Bkc-bound}. Hence,
\[\Pr\big[ (\Bcal_{\tu,\tu'})^c\big] \leq \frac{1}{(N\qu^2)^2}+\frac{40}{\qi^4 N^{10}}\leq \frac{2}{(N\qu^2)^2}\,.\]
Union bound over $\tu,\tu'\in[\qu]$ gives $\Pr[\Bcal^c]\leq \frac{2}{N^2}\,.$
\end{proof}


\begin{claim}\label{cl:ju-err-event-M1}
Let $\iuerr$ be the error defined in Definition \ref{def:ju-iuerr} be the event under which at most $1/10$-th fraction of items in $\Mcc{1}$ from any item types are mislcassified. Then,
\[\Pr\big[\,\iuerr^c([\thrjuu])\,\big|\, \Xi_{\tu,\cdot},\,\Xi_{\tu',\cdot}\,\big]\leq\frac{40}{\qi^4 N^{10}}\]
\end{claim}
\begin{proof}
Similar to the proof of Claim \ref{cl:ju-pr-Ei-cl3}, we defined the potential error event for item $i\in\Mcc{1}$, $\EEt_{i,U_i}$ to be the event that there exists $\ti$ such that $\tau_I(\rep_{\ti})\neq \tau_I(i)$ such that for all the users in $U_i$ agree on $i$ vs. $\rep_{\ti}$. As explained in the proof of Claim \ref{cl:ju-pr-Ei-cl3}, for $i\in\widetilde{\S}_{\ti}$ and $\ti\leq \thrjuu$, we have $\EEt_i([\thrjuu])\subseteq\EEt_{i,U_i}$ for the $U_i=\rated(i)\cap\rated(\rep_{\ti})$ at the time the algorithm added $i$ to $\widetilde{\S}_{\ti}$. Note that according to Claim \ref{cl:ju-pr-Ei-cl2}, there are  users of at least $\thrjiu/2$ distinct user types in $U_i$.

The remaining of the proof is very similar to the proof of Claim \ref{cl:Ftilde}. A set $U_i$ of users of at least $\thrjiu/2$ user types, chosen independently of feedback, rate item $i$. Conditional on the $\tu$ and $\tu'-$th row of matrix $\Xi$ (denoted by $\Xi_{\tu,\cdot}$ and $\Xi_{\tu',\cdot}$), any two item types $\ti\neq \ti'$ have jointly independent user preferences by at least $\thrjiu/2-2$ user types in $U_i$. So, Condition on $\Xi_{\tu,\cdot}$ and $\Xi_{\tu',\cdot}$ the probability of not distinguishing two distinct item types by users in $U_i$  at most $2^{-(\thrjiu/2-2)}$. The choice of $\thrjiu=10\log(\qi N^2)$ and union bounding over item types give

\[\Pr\big[\,\EEt_i([\thrjuu]) \, \big|\, \Xi_{\tu,\cdot}, \Xi_{\tu',\cdot}\,\big] \leq \frac{4}{\qi^4 N^{10}}\,.\]
Using Markov inequality gives
\begin{align*}\Pr\bigg[\,\sum_{i\in\Rb(\ti)}{\ident[\EEt_i([\thrjuu])]}>\frac{|\Rb(\ti)|}{10} \, \big| \, \Xi_{\tu,\cdot}, \Xi_{\tu',\cdot}\,\bigg]& \leq \frac{40}{\qi^4 N^{10}}\,.
\end{align*}
Union bounding over $\ti\in[\qi]$ and tower property of expectation gives the statement of the claim.
\end{proof}


\begin{claim}\label{l:sum-rep-Lkkprime}
For given user types $\tu$ and $\tu'$, let $\Lc_{\tu,\tu'}=\{\ti\in[\qi]: \xi_{\tu,\ti}\neq \xi_{\tu',\ti}\}$. let $X_m = \tau_I(\rep_m)$  and event $\iuerr(X_1,\cdots,X_m)$ as in Definition \ref{def:ju-iuerr}. Then,
\[\Pr\bigg[\sum_{i=1}^{\thrjuu}\ident[X_i\in\Lc_{\tu,\tu'}]< 1 \, \bigg|\, \iuerr([\thrjuu]), \Xi_{\tu,\cdot},\Xi_{\tu',\cdot}, |\Lc_{\tu,\tu'}|\geq \qi/3\bigg] \leq\frac{1}{(N\qu^2)^2}\]
\end{claim}
\begin{proof}
To prove this, we use the statement of Lemma \ref{l:ju-next-rep} which gives a lower bound for the type of next representative item conditional on the type of previous item types, $\Xi_{\tu,\cdot}$ and $\Xi_{\tu',\cdot}$ and the event $\iuerr([\thrjuu])$. Note that $\iuerr([\thrjuu])$ implies $\iuerr([m])$ for all $m\leq\thrjuu$. Assuming $N$ being large enough so that $\thrjuu/\qu < 5/6,$ for $m\leq\thrjuu$ we have
\begin{align*}
\Pr\left[\, X_{m}\notin\Lc_{\tu,\tu'}  \big| X_1,\cdots,X_{m-1}, \Xi_{\tu,\cdot},\Xi_{\tu',\cdot}, \iuerr([m-1]), |\Lc_{\tu,\tu'}| >\frac{\qi}{3}\,\right] &< \frac{81}{100}\frac{\frac{2\qi}{3}}{\qi-(m-1)}\\
&\leq \frac{7}{10}\,.
\end{align*}

Hence, for $m\leq\thrjuu$, condition on $\Xi_{\tu,\cdot},\Xi_{\tu',\cdot}, \iuerr([m-1]), |\Lc_{\tu,\tu'}| >\frac{\qi}{3}\,,$ the random variable $\ident[X_{m}\in\Lc_{\tu,\tu'}]$ stochastically dominates a  $\mathrm{Bern}(7/10)$ random variable. Hence, 
\[\Pr\left[\, \sum_{m=1}^{\thrjuu}\ident[X_{m}\in\Lc_{\tu,\tu'}] =0  \big| \Xi_{\tu,\cdot},\Xi_{\tu',\cdot}, \iuerr([m-1]), |\Lc_{\tu,\tu'}| >\frac{\qi}{3}\,\right] \leq \left(\frac{7}{10}\right)^{\thrjuu}\leq \frac{1}{(N\qu^2)^2} \,.\]
where the choice of $\thrjuu=13\log N\qu^2$ gives the last inequality.
\end{proof}




In the following lemma, we study the probability distribution and dependence of choice of representative items from distinct items types. Note that the item types chosen to be learned are not i.i.d. over time: i) No item type can be chosen twice to be learned; ii) If a given item type has more items in $\Mcc{1},$ it has a higher probability of being picked earlier to be learned; iii)There is a slight dependence between the preference matrix $\Xi$ and the distribution of item types being chosen to learn: If two item types $\ti$ and $\ti'$ are rated similarly by many users and one of them, $\ti$, was chosen to be learned before, there is a high probability that many items of type $\ti'$ is $\Mcc{1}$ were misclassfied by the algorithm to be of type $\ti$. This reduces the probability of choosing $\ti'$ in the next steps to be learned.  

In the following lemma, we will study the effect of all these parameters and show that fixing at most two rows of matrix $\Xi$, at each step, the choice of item types to be learned is close to uniform over the types that have not been learned before. This lemma will be used to bound the probability of error of partitioning the users. It will also be used in providing a lower bound of the number of learned item types which are liked by a given user type.



\begin{lemma}\label{l:ju-next-rep}
Let the sequence of random variables $X_1 = \tau_I(\rep_1), \cdots,  X_{m} = \tau_I(\rep_{m})$ denote the item types of the first $m$ representative items to be learned by the algorithm.

For given distinct user types $\tu$ and $\tu'$, let $\Xi_{\tu,\cdot}$ and $\Xi_{\tu',\cdot}$ to be the $\tu-$th and $\tu'-$th rows of matrix $\Xi$.

Conditional on the $\tu$ and $\tu'-$th row of matrix $\Xi$, given $X_1,\cdots,X_{m-1}$, we are going to find upper and lower bounds for probability of choosing a representative item with a specific type $\ti\notin\{X_1,\cdots, X_{m-1}\}$ is almost uniform (up to a constant) over the set of item types not learned yet by the algorithm.
\begin{equation}\label{eq:ju-nextrep}
\Pr[X_{m}=\ti \big| X_1,\cdots,X_{m-1}, \Xi_{\tu,\cdot},\Xi_{\tu',\cdot},\iuerr([m-1])] > \frac{81}{100}\frac{1}{\qi-(m-1)}
\end{equation}
\end{lemma}

\begin{proof}
To bound the probability of choosing a representative item with a specific type at the next step, we look at the proportion of items the the given type compared to the total number of remaining items in $\Mcc{1}$.

Let $\Rb(\ti)$ to be the set of items in $\Mcc{1}$ of type $\ti$
\begin{equation}\label{ju-Rb2}
\Rb(\ti)= \{i\in\Mcc{1}:\tau_I(i)=\ti\}\,.
\end{equation}
% For given user types $\tu$ and $\tu'$, we want to find the probability that both user types $\tu$ and $\tu'$ rate all item types $X_1, \cdots, X_{\thrjuu}$ similarly. To do so, given $X_1, \cdots, X_m$ for $m<\thrjuu$, $\Xi_{\tu,\cdot}$ and $\Xi_{\tu',\cdot}$ we find the conditional probability of choosing item type $X_m$ as the next type to learn.

 A new item type is chosen randomly among the remaining items in $\Mcc{1}$.
Conditional on the $\tu$ and $\tu'-$th row of matrix $\Xi$ and the event $\iuerr([m-1])$, given $X_1,\cdots,X_{m-1}, \Rb(X_1), \cdots$ and $\Rb(X_{m-1})$, we are going to find upper and lower bounds for probability of choosing a representative item with a specific type $\ti\notin\{X_1,\cdots, X_{m-1}\}:$
\begin{equation}\label{eq:ju-nextrep}
\Pr[\,X_{m}=\ti \,\big|\, X_1,\cdots,X_{m-1}, \Rb(X_1), \cdots,\Rb(X_{m-1}), \Xi_{\tu,\cdot},\Xi_{\tu',\cdot} ,\iuerr([m-1])\,]
\end{equation}
Then, using tower property of expectation and some calculations gives the statement of the lemma.



For $m$, let $t$ be the time the $m$-th representative item is chosen randomly by the algorithm. For $\ti\notin\{X_1,\cdots, X_{m-1}\}$ the probability of choosing representative so that $X_m=\ti$ is equal to the proportion of items of type $\ti$ in the remaining items in $\Mcc{1}$ at time $t-1\,.$ Note that some items of type $\ti$ might have been already miscategorized by time $t-1$. This corresponds to items $i\in\Mcc{1}$ such that $i\in\Rb(\ti)$, but $i\in\widetilde{\mathcal{S}}_{m'}$ for some $m'<m$. It implies $\EEt_i([m-1])=1$. So the total number of items of type $\ti$ in the remaining items in $\Mcc{1}$ might be smaller than $\Rb(\ti)$. 

Define the error event $\EEt_i(X_1,\cdots,X_m)$ for $i\in\Mcc{1}$ as in Equation~\eqref{eq:ju-EEt-m}.
 Remember that we use Definition \ref{def:ju-iuerr} for the event $\iuerr([m-1])$.

The number of items of type $\ti$ in $\Mcc{1}$  by time $t-1$ is
\[|\Rb(\ti)|- \sum_{i\in\Rb(\ti)\cap (\bigcup_{r\in[m-1]}\widetilde{\S}_{X_r})}{\ident\big[\,\EEt_i\,]}= |\Rb(\ti)|- \sum_{i\in\Rb(\ti)}{\ident\big[\,\EEt_i([m-1])\,\big]}\,.\] 
which is lower bounded by $|\Rb(\ti)|$. Conditioning on event $\iuerr([m-1])$, the number of items of type $\ti$ in $\Mcc{1}$  by time $t-1$  is upper bounded by $\frac{9}{10}|\Rb(\ti)|$.

The number of items removed from $\Mcc{1}$ by the time $t$ when $X_m$ is chosen is
 \[\sum_{l=1}^{m-1}|\Rb(X_l)|+ \sum_{\ti\in[\qi]\setminus\{X_1,\cdots,X_{m-1}\}}\sum_{i\in\Rb(\ti)}{\ident\big[\,\EEt_i([m-1])\,\big]}\,,\]
which is upper bounded by $\sum_{l=1}^{m-1}|\Rb(X_l)|$. Conditioning on event $\iuerr([m-1])$, the total number of remaining items in $\Mcc{1}$ is upper bounded by $\frac{9}{10}(M-\sum_{l=1}^{m-1}|\Rb(X_l)|)\,.$
\paragraph{Lower bound for~\eqref{eq:ju-nextrep}.}

 



For $\ti\notin\{X_1,\cdots,X_m\}$, we have
\begin{align}\label{eq:ju-luKj1}
\Pr[X_m=\ti|X_1,\cdots,X_{m-1}, \Rb(\cdot), \Xi_{\tu,\cdot},\Xi_{\tu',\cdot},\iuerr([m-1])]
\geq \frac{9}{10} \frac{|\Rb(\ti)|}{M - \sum_{l=1}^{m-1}|\Rb(X_l)|}\,.
\end{align}

\paragraph{Upper bound for~\eqref{eq:ju-nextrep}.}
 For $\ti\notin\{X_1,\cdots,X_m\}$, we have
\begin{align}\label{eq:ju-luKj2}
\Pr[X_m=\ti|X_1,\cdots,X_{m-1}, \Rb(\cdot), \Xi_{\tu,\cdot},\Xi_{\tu',\cdot},\iuerr([m-1])]
\geq \frac{10}{9} \frac{|\Rb(\ti)|}{M - \sum_{l=1}^{m-1}|\Rb(X_l)|}\,.
\end{align}
%Remember that the probability of choosing $X_m=\ti$ for some $\ti\notin\{X_1,\cdots,X_{m-1}\}$ is proportional to the number of items with type $\ti$ in the remaining items in $\Mcc{1}$. The minimum number of remaining items in $\Mcc{1}$ is the number of items in types $[\qi]\setminus\{X_1,\cdots,X_{m-1}\}$ minus the number of possible mistakes which removed some items from them and categorized them as $i\in\widetilde{S}_{\ti}$ for $\ti<m\,.$
%
%\begin{align*}
%\Pr[X_m=\ti|&X_1,\cdots,X_{m-1}, \Rb(\cdot), \EEt, \Xi_{\tu,\cdot},\Xi_{\tu',\cdot}]\\
%& \leq \frac{|\Rb(\ti)|}{M - \sum_{l=1}^{m-1}|\Rb(X_l)| - \sum_{i\in\Mcc{1}\setminus (\cup_{l=1}^{m-1}\Rb(X_l) \cap (\cup_{\ti<m}\widetilde{S}_{\ti}) }{\ident[\EEt_i]}} 
%\end{align*}
%
%For $i\in\cup_{\ti<m}\widetilde{S}_{\ti}$ using Claim \ref{cl:ju-pr-Ei-cl3},
%%Using Equation~\eqref{eq:ju-EETbd}, for 
%\[\sum_{i\in\Mcc{1}\setminus (\cup_{l=1}^{m-1}\Rb(X_l) \cap (\cup_{\ti<m}\widetilde{S}_{\ti}) }{\Pr[\EEt_i]}\leq \frac{12}{\qi N}(M - \sum_{l=1}^{m-1}|\Rb(X_l)|) \]
%
%Using Markov Inequality, conditional on $X_1,\cdots,X_{m-1}, \Rb(\cdot), \Xi_{\tu,\cdot}$ and $\Xi_{\tu',\cdot}$ with probability at least $1-\frac{24}{\qi N}$
%\[\sum_{i\in\Mcc{1}\setminus (\cup_{l=1}^{m-1}\Rb(X_l) \cap (\cup_{\ti<m}\widetilde{S}_{\ti}) }{\ident[\EE_i]} < \frac{M - \sum_{l=1}^{m-1}|\Rb(X_l)|}{2} \]
%Given the above holds and conditional on  $X_1,\cdots,X_{m-1}, \Rb(\cdot), \Xi_{\tu,\cdot}$ and $\Xi_{\tu',\cdot}$ the probability $X_m = \ti$ is less than 
%\begin{align*}
% \frac{2|\Rb(\ti)|}{M - \sum_{l=1}^{m-1}|\Rb(X_l)|}
%\end{align*}
%Using the total probability lemma,
%
%\begin{align}\label{eq:ju-luKj2}
%\Pr[X_m=\ti|&X_1,\cdots,X_{m-1}, \Rb(\cdot), \Xi_{\tu,\cdot},\Xi_{\tu',\cdot}]
%\leq  2\frac{|\Rb(\ti)|}{M - \sum_{l=1}^{m-1}|\Rb(X_l)|} + \frac{24}{\qi N}
%\end{align}

Taking the expectation of $|\Rb(\ti)|$ conditional on $$X_1,\cdots,X_{m-1}, \Rb(X_1),\cdots,\Rb(X_{m-1}),\Xi_{\tu,\cdot},\Xi_{\tu',\cdot},\iuerr([m-1])$$ for any $\ti\notin\{X_1,\cdots,,X_m\}$ is invariant to choice of $\ti$. So, there exists a constant $C$
$$C = \Exp{\frac{|\Rb(\ti)|}{M - \sum_{l=1}^{m-1}|\Rb(X_l)|}  \bigg|X_1,\cdots,X_{m-1}, \Rb(X_1),\cdots,\Rb(X_{m-1}),\Xi_{\tu,\cdot},\Xi_{\tu',\cdot},\iuerr([m-1])}$$ which is independent of $\ti$ as long as $\ti\notin\{X_1,\cdots,X_m\}$. Using tower property of expectation on Equation~\eqref{eq:ju-luKj1} and~\eqref{eq:ju-luKj2} along with the definition of $C$ above gives
\begin{align*}
\frac{9}{10}C &< \Pr[X_m=\ti|X_1,\cdots,X_{m-1}, \Rb(X_1),\cdots,\Rb(X_{m-1}),\Xi_{\tu,\cdot},\Xi_{\tu',\cdot},\iuerr([m-1])]
 <\frac{10}{9}C\,.
\end{align*}
Since there are $\qi - (m-1)$ types $\ti$ such that $\ti\notin \{X_1,\cdots,X_{m-1}\}$ taking the summation over $\ti$'s, the second inequality of the above display gives  $C\geq\frac{9}{10}\frac{1}{\qi-(m-1)}$. The left inequality of the above display gives for all $\ti\notin\{X_1,\cdots,,X_m\}$,
\begin{align*}
\Pr[X_m=\ti|X_1,\cdots,X_{m-1}, \Rb(X_1),\cdots,\Rb(X_{m-1}),\Xi_{\tu,\cdot},\Xi_{\tu',\cdot},\iuerr([m-1])] &>\frac{81}{100}\frac{1}{\qi-(m-1)}\,.
\end{align*}
Using $\epsilon=\frac{1}{\qi N}$ and $N>32$,
\[\Pr\big[\,X_m=\ti|X_1,\cdots,X_{m-1}, \Xi_{\tu,\cdot},\Xi_{\tu',\cdot},\iuerr([m-1])\,\big]  \geq  \frac3{8(\qi-(m-1))}\,.\]

\end{proof}



%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\subsection{Probability of not finding enough exploitable items}
\begin{lemma}\label{l:ju-exp-R-u}
For user $u\in[N],$
\[\Pr[|\R_u|\leq T] \leq 3\exp(-\frac{\ell}{18})+ \frac{64}{\ell N}\]
And, 
\[\Exp{(T- |\R_u |)_+}\leq 3T\exp(-\frac{\ell}{8})+ \frac{64 T}{\ell N}\,.\]
\end{lemma}

\begin{proof}
Roughly speaking, any user $u$ likes about half of the  $\ell$ item types learned by the algorithm. The total number of items in $\Mcc{2}$ is $T\frac{64\qi}{\ell}$. Hence, there are about $T\frac{64}{\ell}$ items from each of the item types in $\Mcc{2}$. So, with high probability $\R_u$ being the items in $\Mcc{2}$ which user $u$ is expected is more than $T$. 

Making this argument rigorous requires careful reasoning for the following reasons: i) $\R_u$ is the union of $\S_{\ti}$'s with $L_{u,\rep_{\ti}}=+1$. But, for a specific $\ti$ such that $L_{u,\rep_{\ti}}=+1$,   due to misclassification of items, there might be some items of the same type as  $\rep_{\ti}$ which have been misclassified and removed from $\S_{\ti}$. This issue is addressed carefully in the remaining of this proof.
ii) The choice of item types learned by the algorithm at each step is statistically dependent of number of remaining items in each item type in  $\Mcc{1}$.  Again, due to the misclassification, this could be different from the actual number of items of each given type. Additionally, the probability of misclassifying an item of a given type depends on the ratings of a users for that item. Hence, the choice of next item type to be learned is not statistically independent of the rating of a given user $u$ for a given item type. The effect of this dependency should be studied carefully. This phenomenon is addressed carefully in the proof of Claim \ref{cl:JU-lukbd}.

For $u\in\Pc_{\tu}\,,$ we define 
\begin{equation}\label{eq:JU-Ruk}
\Rt_{u}=\{i\in\Mcc{2}: \tau_I(i)=\tau_I(\rep_{\ti}), \text{ for some }\ti\in[\ell] \text{ such that } L_{v,\rep_{\ti}}= +1, \text{ for some } v\in\Pc_{\tu}\}
\end{equation} to be the items in $\Mcc{2}$ whose types are similar to one of the $\rep_{\ti}$'s which are liked by $u$. If there is no error in the classification of items, $\Rt_{u}$ is equal to $\R_u$. It will be easier to bound $\Rt_u$.

Note that if an item $i\in \Rt_{u}$ is correctly classified by the algorithm, then $i\in \R_u$; so $i\in \Rt_u\setminus \R_u$ implies $\EE_i$ (misclassification defined in Equation~\eqref{e:ju-EE}). Hence, \begin{equation}\label{eq:JU-Rubound}
|\R_u|\geq |\Rt_{u}| - \sum_{i\in\Mcc{2}}\ident[\EE_i]\,.
\end{equation}

Observing from Claim \ref{cl:ju-pr-Ei-cl3}, $\Pr[\EE_i]\leq 2/(\qi N)\,.$ Hence,
\begin{align}
\Pr[|\R_u|\leq T]& \leq \Pr[|\Rt_{u}| - \sum_{i\in\Mcc{2}}\ident[\EE_{i}]\leq T]\notag\\
&\leq \Pr[|\Rt_{u}|<\frac 32 T]+\Pr[\sum_{i\in\Mcc{2}}\ident[\EE_{i}]\geq \frac T2]\label{eq:JU-Rubound}
\end{align}
and
\begin{equation}
\Exp{(T-|\R_u|)_+} \leq \Exp{(T-|\Rt_{u}|)_+} + \Exp{\sum_{i\in\Mcc{2}} \ident[\EE_{i}]}\,.\label{eq:JU-Rubound2}
\end{equation}
We bound the second expectation of Equation~\eqref{eq:JU-Rubound2} using Claim \ref{cl:ju-pr-Ei-cl3} 
\begin{equation}\label{eq:JU-Ftildebound}
\Exp{\sum_{i\in\Mcc{2}} \ident[\EE_{i}]}\leq |\Mcc{2}| \epsilon = \frac{64T}{N\ell} 
\end{equation}
and by Markov Inequality for any $s>0$
\begin{equation}\label{eq:JU-Ftildebound2}
\Pr[\sum_{i\in\Mcc{2}} \ident[\EE_{i}]\geq sT] \leq \frac{64}{s \ell N}\,.
\end{equation}


We now bound tail probability of $|\Rt_u|$. 
Remember $\Rt_u$ is the set of items in $\Mcc{2}$ with types the same as representatives which are liked by some user in the same partition as user $u$.

 Let $\Rt(\ti)$ be the set of items in $\Mcc{2}$ whose types are the same as $\rep_{\ti}\,:$
\begin{equation} \label{eq:JU-Rj}
\Rt(\ti) =\{i\in\Mcc{2}: \tau_I(i)=\tau_I(\rep_{\ti})\}\,.
\end{equation}
Note that the sets $\Rt(\ti)$ are mutually exclusive. Let \begin{equation}
\label{eq:JU-Luk}
\Lc_{\tu}^{(\ell)}=\{\tau_I(\rep_\ti): \ti\in[\ell], \xi_{\tu,\tau_I(\rep_\ti)}=+1\}
\end{equation}
 be the set of learned item types in $[\ell]$ which are liked by user $u$. Note that the algorithm guarantees that each representative corresponds to a different item type.
%Using Equation~\eqref{eq:JU-Ruk},  for $u\in\Pc_{\tu},$
% $$\Rt_u = \cup_{\ti\in[\ell], v\in\Pc_{\tu}\atop L_{v,\rep_{\ti}}=+1} \Rt(\ti)\,.$$
Hence, if the partitioning over the users is correct,
\begin{equation*}
|\Rt_u| = \sum_{i\in\Mcc{2}} \ident\big[\,\tau_I(i)\in\Lc_{\tau_U(u)}^{(\ell)}\,\big].
\end{equation*}


Note that  according to the definition of $\Lc_{\tu}^{(\ell)}$ given in Equation~\eqref{eq:JU-Luk}, $\Lc_{\tu}^{(\ell)}$ is determined by: i)$\tu$-th row of matrix $\Xi$ (denoted by $\Xi_{\tu,.}$) which determines whether for all $v$ such that $\tau_U(v)=\tau_U(u)$, $L_{v,\rep_{\ti}}= \xi_{\tu,\tau_{I}(\rep_{\ti})}=+1$ or not; ii) the items in $\Mcc{1}$, their types and some randomness in the algorithm which determines the choice of $\rep_{\ti}$ and $\tau_I(\rep_{\ti})\,.$ Hence, the set $\Lc_{\tu}^{(\ell)}$ is statistically independent of all items $i\in\Mcc{2}$ and their item type. Hence, conditional on any given $\Lc_{\tu}^{(\ell)}\,,$ the types $\tau_I(i)$ for $i\in\Mcc{2}$ is uniformly and independently distributed   over $[\qi]\,.$ So, given $\Lc_{\tu}^{(\ell)}$ with size $\ell_{\tu}^{(\ell)}=|\Lc_{\tu}^{(\ell)}|\,,$ condition on the partiotioning over the users being correct, $|\Rt_u|$ is the sum of $|\Mcc{2}|$ i.i.d. binary random variables; it is a Binomial random variable with mean $M\frac{\ell_{\tu}}{\qi}=64T \frac{\ell_{\tu}}{\ell}$. Using Chernoff bound given in Lemma \ref{l:Chernoff}, condition on $\ell_{\tu}\geq\frac{\ell}{30}$, 
\[\Pr\left[|\Rt_u| < \frac 32 T \big|\ell_{\tu}^{(\ell)}\geq {\ell}/{30}, \Bcal\right]\leq \exp(-T/11)\,.\]


The above inequality and the statement of Claim \ref{cl:JU-lukbd} and Lemma \ref{l:ju-user-mis-pr} give
\begin{align*}
\Pr[|\Rt_u|\leq \frac 32 T ]& < \Pr\left[|\Rt_u| < \frac 32 T \big|\ell_{\tu}^{(\ell)}\geq {\ell}/{30}, \Bcal\right] + \Pr\left[\ell_{\tu}^{(\ell)}< {\ell}/{30}, \Bcal \right] + \Pr[(\Bcal)^c]\\
& < \Pr\left[|\Rt_u| < \frac 32 T \big|\ell_{\tu}^{(\ell)}\geq {\ell}/{30}, \Bcal\right] + \Pr\left[\ell_{\tu}^{(\ell)}< {\ell}/{30} \right] + \Pr[(\Bcal)^c]\\
&\leq \exp(-{T}/{11}) +  \exp(-{\ell}/{15}) + \exp(-{\qi}/{18}) + \frac{20}{N}\,.
\end{align*}

Plugging this and Equation~\eqref{eq:JU-Ftildebound2} into Equation~\eqref{eq:JU-Rubound} gives 
\[\Pr[|\R_u| < T]\leq \exp(-{T}/{11}) +  \exp(-{\ell}/{15}) + \exp(-{\qi}/{18}) + \frac{20}{N} +\frac{128}{\ell N} \,.\]

Since $\ell<T$ and $\ell<\qi\,,$
\[\Pr[|\R_u| < T]\leq 3\exp(-\frac{\ell}{18})+ \frac{148}{ N} \,.\qedhere\]
\end{proof}

\begin{claim}\label{cl:JU-lukbd}
For any $u\in[N]\,,$ and $\ell_{\tu}^{(\ell)}=|\Lc_{\tu}^{(\ell)}|$ with $\Lc_{\tu}^{(\ell)}$ defined in Equation~\eqref{eq:JU-Luk} to be the set of learned item types which $u$ likes, 
\begin{equation*}
\Pr[\ell_{\tu}^{(\ell)} < {\ell}/{30}] < \exp(-{\ell}/{15}) + \exp(-{\qi}/{18})+ \frac{20}{N}\,.
\end{equation*}
\end{claim}

\begin{proof}
For given user type $\tu$, the parameter $\ell_{\tu}^{(\ell)}$ denotes the number of learned item types liked by user type $\tu$. The set of item types learned by the algorithm is a function of the number of items of a given item type in $\Mcc{1}$ at each step; misclassifying items in previous steps changes the number of items of a given type at a given time. Also, the probability of misclassifying  an item from a given type depends on the preference  of users for that item type. Hence, whether or not user type $u$ likes an item type is statistically dependent on whether or not that item type is chosen as one of the learned item types. We will show that the effect of this dependency is small; subsequently, we find upper bounds for probability of $\ell_{\tu}^{(\ell)}<\ell/30$.

Let $\Lc_{\tu}$ be the item types in $[\qi]$ which are liked by user type $\tu$. 
\begin{equation}
	\Lc_{\tu}= \{\ti\in[\qi]: \xi_{\tu,\ti}=+1 \}
\end{equation}

Since the elements of matrix $\Xi$ (determining $\Lc_{\tu}$) are independetly  $\mathrm{Bern}(1/2)$ distributed, using Chernoff bound in Lemma \ref{l:Chernoff} gives \begin{equation}
\label{eq:JU-Lcubd}
	\Pr[|\Lc_{\tu}|< {\qi}/{3}]< \exp(-{\qi}/{18})\,.
\end{equation}

We will show that 
\begin{equation}\label{eq:JU-ell-condLu}
	\Pr\big[\ell^{(\ell)}_{\tu} \leq {\ell}/{30} \,\big|\, |\Lc_{\tu}|> {\qi}/{3}\big] \leq \exp(-{\ell}/{5}) + \frac{20}{N}
\end{equation}

To do so, let the sequence of random variables $X_1 = \tau_I(\rep_1), X_2 = \tau_I(\rep_2), \cdots$ denote the item types chosen to be learned by the algorithm. Then, $|\Lc^{(\ell)}_{\tu}| = \sum_{\ti\in[\ell]}\ident[X_{\ti}\in \Lc_{\tu}]$. Note that the set $\Lc_{\tu}$ is a one-to-one function of $\tu-$th row of matrix $\Xi$ (denoted by $\Xi_{\tu,\cdot}$).
Define $\Rb(\ti)$ to be the set of items in $\Mcc{1}$ of type $\ti$
\begin{equation}\label{JU-Rb2}
	\Rb(\ti)= \{i\in\Mcc{1}:\tau_I(i)=\ti\}\,.
\end{equation}


%%%%%%%%%%%%%%%

Define the error event $\EEt_i$ for $i\in\Mcc{1}$, defined in Equation~\eqref{eq:ju-EEt-m},
 be the event item $i\in\Mcc{1}$ is miscategorized into one of the representative item types labeled by $X_1,\cdots,X_m$.  Also, let $\EEt_i = \EEt_i([\qi])$ be the error event associated with item $i\in\Mcc{1}$ similar to before.

Using Definition \ref{def:ju-iuerr}
for event  $\iuerr(X_1,\cdots,X_m)$, applying the total probability lemma, for any fixed value of $\Xi_{\tu,\cdot}$: 
\begin{align}
 \Pr\bigg[\sum_{i=1}^{\ell}\ident\big[\,X_i\in\Lc_{\tu}&\,\big]< \ell/30 \, \bigg|\, \Xi_{\tu,\cdot}, |\Lc_{\tu}|\geq \qi/3\bigg] \notag\\
&\leq \Pr\bigg[\sum_{i=1}^{\ell}\ident\big[\,X_i\in\Lc_{\tu}\,\big]< \ell/30 \, \bigg|\, \iuerr([\ell]), \Xi_{\tu,\cdot}, |\Lc_{\tu}|\geq \qi/3\bigg]\notag\\
&\quad+ \Pr\big[\,(\iuerr([\ell]) )^c\,\big|\,\iuerr([\ell]) \Xi_{\tu,\cdot} |\Lc_{\tu}|\geq \qi/3\,\big]\,. \label{eq:ju-decom-size-ellk}
\end{align}
Considering $\Pr\big[\,(\iuerr([\ell]) )^c\,\big|\, \Xi_{\tu,\cdot} |\Lc_{\tu}|\geq \qi/3\,\big]\leq \Pr\big[\,\iuerr^c\,\big|\, \Xi_{\tu,\cdot} |\Lc_{\tu}|\geq \qi/3\,\big]$, using the tower property of expectation on the result of Claim \ref{cl:ju-err2-event-M1} provides an upper bound for the second term on the right hand side of above display:
\begin{equation}
\Pr\big[\,(\iuerr([\ell]) )^c\,\big|\, \Xi_{\tu,\cdot} |\Lc_{\tu}|\geq \qi/3\,\big]\leq \frac{20}{N}\,.
\end{equation}
Lemma \ref{l:sum-rep-Lk} provides the upper bound for the first term for all $\Xi_{\tu,\cdot}$  such that $|\Lc_{\tu}|\geq \qi/3$ (remember that $\Lc_{\tu}$ is a deterministic function of the $\tu-$th rows of matrix $\Xi$). Hence, 
\[\Pr\bigg[\sum_{i=1}^{\ell}\ident\big[\,X_i\in\Lc_{\tu}\,\big]< \ell/30 \, \bigg|\, \Xi_{\tu,\cdot}, |\Lc_{\tu}|\geq \qi/3 \bigg] \leq \exp(-\ell/15)\,.\]

Plugging this into Equation~\eqref{eq:ju-decom-size-ellk} gives

\[\Pr\bigg[\sum_{i=1}^{\ell}\ident\big[\,X_i\in\Lc_{\tu}\,\big]< \ell/30 \, \bigg|\, \Xi_{\tu,\cdot}, |\Lc_{\tu}|\geq \qi/3\bigg] \leq  \exp(-\ell/15) + \frac{20}{N}\]


Taking the expectation of this with respect to $\Xi_{\tu,\cdot}$  condition on $|\Lc_{\tu}|\geq \qi/3$ and lugging Equation~\eqref{eq:JU-Lcubd} gives the statement of claim.
\end{proof}


\begin{claim}\label{cl:ju-err2-event-M1}
Let $\iuerr$ be the error defined in Definition \ref{def:ju-iuerr} be the event under which at most a fraction of $1/10$-th of items in $\Mcc{1}$ from any item types are mislcassified. Then,
\[\Pr\big[\,\iuerr^c\,\big|\, \Xi_{\tu,\cdot}\,\big]\leq\frac{21}{N}\,.\]
\end{claim}
\begin{proof}

We use 
\[\Pr\big[\,\iuerr^c\,\big|\, \Xi_{\tu,\cdot}\,\big] \leq \Pr\big[\,\iuerr^c\,\big|\, \Xi_{\tu,\cdot},\Bcal\,\big]+ \Pr[\Bcal^c\,|\, \Xi_{\tu,\cdot} ]\,.\]

The exact same steps in the proof of Lemma \ref{l:ju-user-mis-pr} shows that $\Pr[\Bcal^c\,|\, \Xi_{\tu,\cdot} ]\leq 2/N^2\,.$ 

To bound the first term in the above display, for any $i\in\Mcc{1}$ define 

\begin{equation}\label{e:ju-EEtu-def}
\EEt_{i,U_i}=\{\exists \ti\neq \tau_I(i): L_{u,i}=\xi_{\tau_U(u),\ti}\,, \forall u\in U_i\}
\end{equation}

Condition on the partitioning over users being correct, the event $\EEt_i\subseteq \EEt_{i,U_i}$ for the set of users $U_i$ which are used in classifying item $i$. Exactly similar to the proof of Claim \ref{cl:ju-pr-Ei-cl2}, Given $N$ large enough so that $\qu>10\thrjiu$, the $\thrjiu$ users rating any item in $\Mcc{1}$ belong to at least $\frac{\thrjiu}{2}$ distinct user types with probability at least $1-\frac{1}{\qi N}$. Conditioning on $\Xi_{\tu,\cdot}$ implies that there are at least ${\thrjiu}/{2}-1$ distinct user types (chosen independent of feedback and matrix $\Xi$) are used as witnesses in categorizing item $i$. Hence, the probability that there is another item type $\ti\neq\tau_I(i)$ which is rated the same by these ${\thrjiu}/{2}-1$ user types is $2^{-({\thrjiu}/{2}-1)}\leq 2/(N\qi^2)^5\,.$ Hence,  
\[\Pr\big[\,\EEt_i\,\big|\, \Xi_{\tu,\cdot},\Bcal\,\big] \leq  \frac{1}{N\qi}+\frac{2}{(N\qi^2)^5}\leq\frac{2}{N\qi}\,.\]
Using Definition \ref{def:ju-iuerr} for $\iuerr$ gives
\[\Pr\big[\,\iuerr^c\,\big|\, \Xi_{\tu,\cdot},\Bcal\,\big] \leq \frac{20}{N}\,.\]
The above two inequalities give the statement of the Claim.
\end{proof}



\begin{lemma}\label{l:sum-rep-Lk}
Let the sequence of random variables $X_1 = \tau_I(\rep_1), X_2 = \tau_I(\rep_2), \cdots$ denote the item types chosen to be learned by the algorithm. Then,
\[\Pr\bigg[\sum_{i=1}^{\ell}\ident[X_i\in\Lc_{\tu}]<\ell/30 \, \bigg|\, \iuerr([\ell]), \Xi_{\tu,\cdot}, |\Lc_{\tu}|\geq \qi/3 \bigg] < \exp(-\ell/15)\,.\]
\end{lemma}

\begin{proof}
We use the statement of Lemma \ref{l:ju-next-rep} to show that for any $\tu\in[\qu]$ and any $\ti\notin\{X_1,\cdots,X_{m-1}\}$
\begin{equation}\label{eq:JU-nextrep-lk2}
\Pr[X_{m}=\ti \big| X_1,\cdots,X_{m-1}, \Xi_{\tu,\cdot}, \iuerr([m-1])] > \frac{81}{100}\frac{1}{\qi-(m-1)}
\end{equation}

Hence, for $\Xi_{\tu,\cdot}$ such that $|\Lc_{\tu}|\geq \qi/3,$ 
\[\Pr[X_{m}\in\Lc_{\tu} \,\big| \sum_{m'=1}^{m-1}\ident[X_{m'}\in\Lc_{\tu}]<s , \Xi_{\tu,\cdot},|\Lc_{\tu}|\geq \qi/3 , \iuerr([m-1])] > \frac{81}{100}\frac{\frac{\qi}{3}-s}{\qi-(m-1)} > \frac{1}{5}\,.\]
where the last inequality holds for $s\leq\ell/30$ and $m\leq\ell\leq \qi\,.$
So the random variable $\sum_{m'=1}^{\ell}\ident[X_{m'}\in\Lc_{\tu}]$ conditional on $\Xi_{\tu,\cdot},|\Lc_{\tu}|\geq \qi/3 $ and $\iuerr([m-1])$, stochastically dominates a  $\mathrm{Bin}(\ell,1/5)$ random variable. Hence,

\[\Pr[\sum_{m'=1}^{\ell}\ident{[X_{m'}\in\Lc_{\tu}]}<\frac{\ell}{30}\,\big| \Xi_{\tu,\cdot},|\Lc_{\tu}|\geq \qi/3 , \iuerr] > \exp(-\ell/15) \,.\]
 
\end{proof}


==> logLowerBound.tex <==

%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%

\newpage
\subsection{The log lower bd. Version 3}
For any $u\in[N]$, define the number of item types \textit{rated} by $u$ up to time $t$ and

\begin{align}
d_u^t &:=
\sum_{\ti=1}^{\qi}\ident\b\{\tau_I(a_{u,s})=\ti\text{ for some } s<t\b\}
\,. 
\end{align}

For any $u\in[N]$, define the number of item types \textit{rated and liked} by $u$ up to time $t$ and


\begin{align}
\liked u t & =
\sum_{\ti=1}^{\qi}\ident\b\{\tau_I(a_{u,s})=\ti, L_{u,a_{u,s}}=+1\text{ for some } s<t\b\}
\,. 
\end{align}



Roughly speaking, $\liked{u}t$ is $\mathsf{Bin}(d_u^t,1/2)$ as long as user $u$ does not exploit the information in the user structure (users are not categorized).

\guy{needs interpretation / discussion}

\guy{can we use $1/3$ instead of $2/5$?}

\begin{lemma}
Fix given user $u\in[N]$. Then,
\begin{align}\label{e:duTbound}
\Pr\left[\liked{u}T\leq 
\begin{cases}
0, & \quad \text{ if }\quad d_u^T \leq \min\{\log T,\tul\}\\
d_u^T, & \quad \text{ otherwise}
\end{cases}
\,\Big|\,\Omega\right]\geq \frac{1}{T}
\end{align}

\begin{align}
\Pr\left[\liked{u}T/d_u^T\leq 
 \ident\big\{d_u^T > \min\{\log T,\tul\}\big\}
\,\Big|\,\Omega\right]\geq \frac{1}{T}
\end{align}

for any $a\leq \tul$, and any $t$
\begin{align*}
\Pr\left[\liked{u}t = 0\,\Big|\, 
d_u^t, d_u^t \leq a,\, \Omega\right]
\geq \frac{1}{3^a}
\end{align*}


for any $s\leq \tul$, and any $t$
\begin{align*}
%\label{eq:duplusMainBound}
\Pr\left[\liked{u}t = 0\,\Big|\, 
d_u^t= s,\, \Omega\right]
\geq \frac{1}{3^s}
\end{align*}


\begin{align*}
\Pr\left[\liked{u}t \leq  d_u^t  
\right]
=1
\end{align*}
\end{lemma}

Let $\E Kt$ be the event in \eqref{e:duTbound} modified a little, 
\begin{align}\label{e:Edef}
\bigg\{\liked{u}t\leq 
\begin{cases}
0, & \quad \text{ if }\quad d_u^t \leq \min\{K,\tul\}\\
d_u^t, & \quad \text{ otherwise}
\end{cases}
\bigg\}
\end{align}
Then
\begin{align*}
\sum_{k=0}^{K}\Pr(E|d_u^t=k)\Pr(d_u^t=k) + \Pr(E|d_u^t>K)\Pr(d_u^t>K)
\end{align*}

Note that $E_K = E_{\tul}$ if $K \geq \tul$. Hence we can assume that
$K\leq \tul$. 
\begin{align*}
&\sum_{k=0}^{K}\Pr(E_K|d_u^t=k)\Pr(d_u^t=k) + \Pr(E_K|d_u^t>K)\Pr(d_u^t>K)
\\ &
\geq 
\sum_{k=0}^{K}\frac1{3^k}\Pr(d_u^t=k) + \Pr(d_u^t>K) 
\\& \geq
\frac{1}{3^K} 
\sum_{k=0}^{K}\Pr(d_u^t=k) + \frac{1}{3^K} \Pr(d_u^t>K)
 \geq
\frac{1}{3^K} 
\end{align*}

Note that $\Pr(E_K|d_u^t>K)=1$ since $\liked{u}t \leq  d_u^t$ with probability one.

\begin{proof}

\MK{Write an exposition on how we use this bound in the lower bound of regret. }

We use proposition~\ref{p:badUncertain} for $b=1$ and $3$.

\begin{align*}
\Pr\b(L_{u,a_{u,t}} = -1 |\Bsf{b}_{u,t}, \Omega\b)\geq 1/3
\end{align*}
Combining these yields
\begin{align}
 \label{eq:bdprobnNewUserT}
\Pr\b(L_{u,a_{u,t}} = -1 |d_{u}^t < \tul, (\BBjil{u}{a_{u,t}}{t})^c, \Omega\b)\geq 1/3
\end{align}

\begin{align}
 \label{eq:bdprobnNewUserT}
\Pr\b(L_{u,i} = -1 |d_{u}^t < \tul, (\BBjil{u}{i}{t})^c, \Omega\b)\geq 1/3
\end{align}
\guy{change this to allow us to condition on any value, should still be true}

Note that
\[d_{u}^t  = \sum_{s=1}^t \ident\{(\BBjil{u}{a_{u,s}}{s})^c\} \]

\[\liked{u}t  = \sum_{s=1}^t \ident\{L_{u,a_{u,t}} = +1 , (\BBjil{u}{a_{u,s}}{s})^c\} \]

Define $T_1=1$ and
\begin{align*}
T_k &= \min\{t >T_{k-1}: d_u^t>d_{u}^{t-1} \}\\
& = \min\{t: d_u^t \geq k\}
\end{align*}
$T_k$ is the time that the $k$-th new item type is recommended to user $u$. So $d_u^{T_k}=k$. The $T_k$'s are stopping times with respect to $(d_u^t)$, and observe that $k^*=  \max\{k: T_k\leq t\} = d_u^t$ is the total number of item types recommended by the algorithm by the end of time $t$. Also, $\liked{u}{T_{k^*}}=\liked{u}t$.

For any $s\leq \tul$, and any $t$, we want to show that 
\begin{align}
\label{eq:duplusMainBound}
\Pr\left[\liked{u}t = 0\,\Big|\,
d_u^t= s,\, \Omega\right]
\geq \frac{1}{3^s}
\end{align}

\begin{align*}
\Pr\left[\liked{u}t = 0\,\Big|\, 
d_u^t= s,\, \Omega\right]
&=
\Pr\left[\sum_{r=1}^t \ident\{L_{u,a_{u,r}} = +1 , (\BBjil{u}{a_{u,s}}{r})^c\} =0 \,\Big|\, 
d_u^t= s,\, \Omega\right]
\\&=
\Pr\left[\ident\{L_{u,a_{u,r}} = +1 , (\BBjil{u}{a_{u,r}}{r})^c\} =0  \text{ for all } r\leq t\,\Big|\, 
d_u^t= s,\, \Omega\right]
\\&=
\Pr\left[\bigcap_{r=1}^t\{L_{u,a_{u,r}} = -1 \cup (\BBjil{u}{a_{u,r}}{r})\}\,\Big|\, 
d_u^t= s,\, \Omega\right]
%\\&=
%\Pr\left[L_{u,a_{u,r}} = -1 ,  \text{ for all } r\leq t\,\Big|\, 
%d_u^t= s,\, (\BBjil{u}{a_{u,r}}{r})^c , \,\Omega\right]
\end{align*}

% \[
% d_{u}^t  = \sum_{s=1}^t \ident\{(\BBjil{u}{a_{u,s}}{s})^c\}
% = 
% \]


%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\newpage
\subsection{martingale -- Mina's version}


For any $u\in[N]$, define the number of item types \textit{rated} by $u$ up to time $t$ and

\begin{align}
d_u^t &:=
\sum_{\ti=1}^{\qi}\ident\b\{\tau_I(a_{u,r})=\ti\text{ for some } r<t\b\}
\\ & = 
\sum_{r=1}^{t-1} \ident\b\{ (\BBjil{u}{a_{u,r}}{r})^c \b\}
\,. \notag
\end{align}

For any $u\in[N]$, define the number of item types \textit{rated and liked} by $u$ up to time $t$ and


\begin{align}
\liked u t & =
\sum_{\ti=1}^{\qi}\ident\b\{\tau_I(a_{u,r})=\ti, L_{u,a_{u,r}}=+1\text{ for some } r<t\b\}
\\ & = 
\sum_{r=1}^{t} \ident\b\{ (\BBjil{u}{a_{u,r}}{r})^c, L_{u,a_{u,r}} = +1 \b\}
\,. \notag
\end{align}
\MK{I defined $\liked{u}{t}$ to include the item type at $t$}

\begin{lemma}
    Fix $s< \tul$. Then,
\[\Pr[ \text{for all } t \text{ such that } d_u^t <s, \liked u t = 0 ] \geq 1/3^s \,.\]
Hence, setting $s=\min\b\{ \log T - \log \log T,\tul \b\}$ and using the trivial inequality $\liked u t\leq d_u^t$,
\begin{align}
\Pr\left[\liked{u}{T}/d_u^T\leq 
 \ident\big\{d_u^T > \min\{\log T,\tul\}\big\}
\right]\geq \frac{\log T}{T}
\end{align}

\begin{align}
\Pr\left[\liked{u}{T}\leq 
 T \ident\big\{d_u^T > \min\{\log T,\tul\}\big\}
\right]\geq \frac{\log T}{T}
\end{align}
\MK{I think I want to bound $\liked{u}{T}\leq 
T \ident\big\{d_u^T > \min\{\log T,\tul\}\big\}$. This will be easier since $\liked{u}{T}$ could potentially be $d_u^T+1$}
\end{lemma}

\begin{align}
    \bad(T) &\geq T\ind{\liked{u}{t}=0}
    \\
    \bad(T)&\geq d_u^T\\
    \Pr(\bad(T) &\geq T\ind{d_u^T<s})\geq  3^{-s}
    \\
d_u^T + \log 
    \\
    E&=\{\liked{u}{T}/d_u^T\leq 
 \ident\big\{d_u^T > \min\{\log T,\tul\}\}
 \\
 \Ex[\bad(T)] &\geq  \Ex[\bad(T)|E] \Pr(E)\\
 &\geq \Ex[d_u^T + T \big\{d_u^T > \min\{\log T,\tul\}\} | E] \logT /T
 \\
 \Ex[\bad(T)] & = \Ex[\Ex[\bad(T)| d_u^T]]
\end{align}

If $d_u^T> \min\{\log T,\tul\} $ then $E$ holds a.s. We want 
$
\Pr(E|d_u^T)
$.

\newpage

\begin{proof}
 Define $X_t = \ident\{L_{u,a_{u,t}} = -1 \}$, $K_t = (\BBjil{u}{a_{u,t}}{t})^c$, $D_t = \sum_{i< t} \ident\{K_i\}$ and $\Fc_{t} = \sigma(X_1, \cdots, X_t, K_1, K_2, \cdots, K_{t+1})$.


With this notation, $D_t = d_{u}^{t}$. Also,  if for all $i<t$ such that $K_i$ occurs, $X_i=1$ then $\liked{u}{t}=0$.


With this definition, $\Fc_{t}\in \sigma (\H_{t}, \tI, \zeta_{u,t})$. So applying tower property on the statement of  Lemma~\ref{l:jl-bdA5statement} shows that $\Pr(X_t = 1|\Fc_{t-1}, K_t, D_t= s) \geq 1/3$ almost surely for any $s\leq s^*$, then for any $s\leq s^*$.

We apply lemma~\ref{lem:stopped} to get the desired statement. 
\end{proof}

\MK{I checked Lemma~\ref{l:jl-bdA5statement} and it's correct.}
\begin{lemma}
\label{l:jl-bdA5statement}
For any $s< \tul$,
    \begin{align}
        \Pr[ L_{u,a_{u,t}} = -1  | \H_{t-1}, \tI ,(\BBjil{u}{a_{u,t}}{t})^c, d_u^t =s] \geq 1/3\,.
        \label{eq:jl-bdA5statement}
    \end{align}
\end{lemma}

%%%%%%%%%%%%%%%%%%%%
\begin{proof}
The proof is similar to the proof of Prop.~\ref{p:badUncertain} with $b=3$.


 Let $\bj_u\in \sigma(\H_{t-1},\tau_I)$ is the set of item types previously rated by user $u$ and row vector $\bx_u\in \sigma(\H_{t-1},\tau_I)$ is the $\pm 1$ feedback. 



Let
\begin{align}
\hist{5}=
\big\{
& \text{realizations of }
\big(\H_{t-1}, \,\Xi, \, \tI, \tUnu \big)
\text{ such that }
\notag
\\&\quad
 \,d_u^t =s,\, \big(\BBjil{u}{i}{t}\big)^c,\, \Xi \in \Omega
%\notag \\ &
\text{ and } a_{u,r}\neq i \text{ for all } r\leq t-1
\, \big\} 
\label{eq:defA5Event}
\end{align}
be the set of possible realizations of the model parameters and history up to time $t-1$  consistent with the event conditioned upon in~\eqref{eq:jl-bdA5statement}. This set is well-defined for the same reason $\hist{3}$ is well-defined in the proof of Prop.~\ref{p:badUncertain} with $b=3$



Let $\bj_u$ and $\bx_u$ be as defined in Lemma~\ref{l:A3propbound}.
Note that $\bj_u$ is  a deterministic function of realization of $\H_{t-1}$ and $\tI$.
Given any realization of $\H_{t-1}$ and $\tI$ in $\hist{5}$, the type of user $u$ is uniform on $\Lambda_{\bx_u}(\Xi_{\bullet \bj_u})$ and $|\bj_u|= d_u^{t}=s < \tul$. 
 
 So for any realization of 
 $\big(\H_{t-1}, \,\Xi, \, \tI, \tUnu\big)
\in\hist{5}
$,
 \begin{align*}
\Pr\Big[L_{u,i}=+1 \,\big|\, \H_{t-1}, \,\Xi, \, \tI, \tUnu \Big]
& \overset{(a)}{=}
 \frac{|\Lambda_{\bx_u^+,}(\Xi_{\bullet (\bj_u,\tau_I(i))})|}
 {|\Lambda_{\bx_u}(\Xi_{\bullet \bj_u})|}
\overset{(b)}{\leq }
\frac{(1+\eta)2^{|\bj_u|}}
{(1-\eta) 2^{|\bj_u|+1}} 
 \overset{(c)}{\leq }
3/5\,,
\end{align*}
where (a) uses the statement of Lemma~\ref{l:A3propbound} which shows that
\begin{align*}
\Pr\big(L_{u,i}=+1 \,\big|\, \H_{t-1}, \,\Xi, \, \tI, \tUnu, (\BBjil{u}{i}{t})^c \big)
&=
  \frac{|\Lambda_{\bx_u^+,}(\Xi_{\bullet (\bj_u,\tau_I(i))})|}
 {|\Lambda_{\bx_u}(\Xi_{\bullet \bj_u})|}\,.
\end{align*}
(b) uses the column regularity of matrix $\Xi$ ($ \Xi \in \rgl_{\tul,\eta}$ as in Definition~\ref{def:ul-reg}) and $|w_{u}|=s<\tul$. (c) uses
$\eta<1/11$. \MK{double check $\eta<1//11$.}

The tower property of expectation over above display gives 
\begin{align*}
   \Pr[ L_{u,a_{u,t}} = +1 \, \big|\, \H_{t-1}, \tI ,(\BBjil{u}{a_{u,t}}{r})^c, d_u^t =s, \Omega]\leq 3/5 \,.
\end{align*} 
Since $\Pr[\Omega] \geq 1/100$, we have 
\begin{align*}
   \Pr&[ L_{u,a_{u,t}} = +1  | \H_{t-1}, \tI ,(\BBjil{u}{a_{u,t}}{r})^c, d_u^t =s]
  \\
  & \leq 
      \Pr[ L_{u,a_{u,t}} = +1  | \H_{t-1}, \tI ,(\BBjil{u}{a_{u,t}}{r})^c, d_u^t =s, \Omega]
      + \Pr[\Omega^c] \leq 2/3\,. \hfill\qedhere
\end{align*}
\end{proof}
%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%



\begin{lemma}\label{lem:stopped}
    Consider a discrete-time process $X_1,X_2,\dots$ with each $X_i\in \{0,1\}$ adapted to filtration $\Fc_t$ and a
    sequence of predictable events $K_1,K_2,\dots$, where $K_t\in \Fc_{t-1}$. Let $D_t = \sum_{i< t} \ind{K_i}$.
    If $\Pr(X_t = 1|\Fc_{t-1}, K_t, D_t= s) \geq 1/3$ almost surely for any $s< s^*$, then for any $s\leq s^*$
    % $$
    % \Pr(X_i = 1 \text{ for all } i\leq t \text{ such that } K_i \text{ occurs}|D_t)\geq 1/3^{D_t} \cdot \ind{D_t\leq s^*}\,.
    % $$
    $$
   \Pr( \text{ for all } t \text{ such that } D_t< s \text{ and all } i\leq t \text{ such that } K_i \text{ occurs}, X_i = 1  ) \geq 1/3^s
    \,.$$
\end{lemma}

% We first quickly show that Lemma~\ref{lem:stopped} follows from Lemma~\ref{lem:dt-mg}. 


\begin{proof}
Take $X_t, K_t$, and $D_t$ as in Lemma~\ref{lem:stopped}.
Define $$K'_t = K_t\cap \{D_{t} \leq s^*-1\}$$ and note that this is still a predictable event (i.e. in $\Fc_{t-1}$), and moreover, that $D_t< s^*$ on $K'_t$. 
Additionally define $X'_t = \max(X_t, \ind{{K'_t}^c})$, so that $X'_t=1$ automatically whenever $K_t'$ does not occur. 

We now show that $\Pr(X_t' = 1|\Fc_{t-1}) \geq 1/3$ almost surely. To start,
$$
 \Pr(X_t' = 1|\Fc_{t-1}, K_t^c)  = 1$$
 and
\begin{align*}  
 \Pr(X_t' = 1|\Fc_{t-1}, K_t) &=  
    \sum_{s=0}^{s^*-1} \Pr(X_t' = 1|\Fc_{t-1}, K_t, D_t= s)  \Pr( D_t= s|\Fc_{t-1}, K_t) 
   \\&\quad  +\sum_{s=s^*}^{\infty} \Pr(X_t' = 1|\Fc_{t-1}, K_t, D_t= s)  \Pr( D_t= s|\Fc_{t-1}, K_t) 
    \\
    & \geq \sum_{s=0}^{s^*-1}\frac{1}{3} \Pr( D_t= s|\Fc_{t-1}, K_t) 
    +\sum_{s=s^*}^{\infty}  \Pr( D_t= s|\Fc_{t-1}, K_t) \geq \frac{1}{3}\,.
\end{align*}
Here we used the lemma statement's assumption $\Pr(X_t = 1|\Fc_{t-1}, K_t, D_t= s) \geq 1/3$ a.s. for any $s< s^*$, together with the fact that $X_t'\geq X_t$ a.s., to bound the first term. We also used the fact that for $s\geq s^*$, $D_t= s$ implies ${K'_t}^c$ holds and hence $X_t' = 1$.
From $X_t'\geq \ind{{K'_t}^c} \geq \ind{{K_t}^c}$ follows that
$$
     \Pr(X_t' = 1|\Fc_{t-1}) 
      = \Pr(X_t' = 1|\Fc_{t-1}, K_t)  \Pr(K_t|\Fc_{t-1}) + \Pr(X_t' = 1|\Fc_{t-1}, K_t^c)  \Pr(K_t^c|\Fc_{t-1}) \geq \frac{1}{3}\,.
$$
     
We now apply Lemma~\ref{lem:dt-mg} to $X'_t$ and $K'_t$ and  $D'_t = \sum_{i\leq t} \ind{K'_i}$ to obtain that for any $s$, \MK{Note that to use the stopping time, I am making $D't$ to include $K'_t$ whereas $D_t$ does not.}
\begin{align*}
           \Pr( \text{ for all } t \text{ such that } D_t'< s \text{ and all } i\leq t \text{ such that } K_i' \text{ occurs}, X_i' = 1  ) \geq 1/3^s\,.
\end{align*}
Note that for all $s\leq s^*$, $\{D_{t+1}=s\} = \{D'_{t}=s\}$ so
\[
\{t:D_t<s\}
\subseteq \{t: D_t' <s\}\,.
\]

Additionally, if $D_t\leq s^*-1$, then
$$\{i\in [t]:K_i'\text{ occurs}\}= \{i\in [t]:K_i\text{ occurs}\}
\,,$$
so on event $\{D_t=s\}$ for any $s\leq s^*-1$, we have 
\[\big\{X'_i = 1 \text{ for all } i\leq t \text{ such that } K'_i \text{ occurs} \big\} = 
\big\{X_i = 1 \text{ for all } i\leq t \text{ such that } K_i \text{ occurs}\big\}\,. \]
Hence, for any $s\leq s^*$
\begin{align*}
       \Pr&( \text{for all } t \text{ such that } D_t< s \text{ and all } i\leq t \text{ such that } K_i \text{ occurs}, X_i = 1  )
       \\&\geq 
          \Pr( \text{for all } t \text{ such that } D_t'< s \text{ and all } i\leq t \text{ such that } K_i' \text{ occurs}, X_i' = 1  ) \geq 1/3^s\,. 
          \hfill\qedhere
\end{align*}
\end{proof}


\begin{lemma}
\label{lem:dt-mg}
  Consider a discrete-time process $X_1', X_2',\dots$ with each $X_i'\in \{0,1\}$ adapted to filtration $\Fc_t$ and a
    sequence of predictable events $K_1',K_2',\dots$, where $K_t'\in \Fc_{t-1}$. Let $D_t' = \sum_{i\leq t} \ind{K_i'}$.
    If $\Pr(X_t' = 1|\Fc_{t-1}) \geq 1/3$ almost surely, then for any $s$
    % $$
    % \Pr(X_i = 1 \text{ for all } i\leq t \text{ such that } K_i \text{ occurs}|D_t)\geq 1/3^{D_t} \cdot \ind{D_t\leq s^*}\,.
    % $$
    $$
   \Pr( \text{ for all } t \text{ such that } D_t'< s \text{ and all } i\leq t \text{ such that } K_i' \text{ occurs}, X_i' = 1  ) \geq 1/3^s
    $$

        $$
   \Pr\b(\bigcap_{t} \{( D_t'< s)^c \cup (M_t>0)\}  \b) \geq 1/3^s
    $$

    We want 
    $$ 
    \Pr\b( M_t>0\,\b|\,  D_t'< s  \b) \geq 3^{-s}$$
\end{lemma}

For any fixed $s$, define the stopping times
$$T=\inf\{t:M_t=0\}\quad \text{and} \quad
S=\inf\{t:D_t'=s\}\,.
$$

$$
\{ D_t'< s\} = \{t<S\}\quad \text{and} \quad \{M_t>0\} = \{t<T\}
$$
so we want to bound
$$
\Pr( t< T| t< S)
$$

Strategy: define a different process, so that if $t\geq S$, then process is somehow stuck at $t<S$. But value of process should be the same. 
Let $D_t'' = \min(\sum_{i\leq t} \ind{K_i'},s-1)$ and 
$$
M_t'' = \prod_{i\leq t:\atop D_{i}'' - D_{i-1}''=1} 3 X_i'\,.
$$
Claim: On the event $\{t<S\}$, $M_t$ can be coupled to $M_t''$.

Now by the optional stopping theorem\footnote{OST applies because for all $t$, $|M_{t\wedge S\wedge T}|\leq 3^s$.} applied to stopping time $t\wedge T\wedge S$,
$$
1\leq \Ex M_{t\wedge T\wedge S} = \Pr(T\leq S)\cdot 0 + \Pr(T>S)\Ex[3^{D_S'}|T> S] = \Pr(T>S) \cdot 3^s\,.
$$

\begin{proof}
    

% Let 
% $D_t' = D'_{t-1} +(D_t' - D_{t-1}') = D'_{t-1} +\ind{K_t'}$, which is still a predictable sequence because $D_t$ is predictable.


 
 % Now 
 % $\Ex[3X_t|\Fc_{t-1}]\geq 1$ almost surely and hence
 % $$M_t = 3^t X_1\cdots X_t$$
 % is a (sub)martingale.

% Let $T=\min\{t:Y_t=0\}$ be the first $0$. Then 
% $$
% 1 \leq  \Ex M_{n\wedge T} = \Pr(T>n) 3^n\,,
% $$
% where we used the fact that if $T\leq n$, then $M_{n\wedge T}=0$.

% Now let $H_t$ be a predictable sequence. This is going to be our rule for if we toss a coin at time $t$ and is a function of outcomes at times $t-1$ and earlier. We set $H_t=1$ if we toss the coin at time $t$ and $0$ otherwise. The martingale transform
% $$
% D_t =(H\circ M)_t = \sum_{i=1}^t H_i (M_i - M_{i-1}) =  \sum_{i=1}^t H_i (3 X_i - 1)M_{i-1}
% $$
% is also a martingale. 
% Let $D_t-D_{t-1}\in\{0,1\}$ be the times at which we toss the coin and suppose that $D_t$ is predictable, i.e., $D_t\in \mathcal{F}_{t-1}$. 

% Let 
% $D_t' = D'_{t-1} +\ind{D_{t-1}\leq s^*-1}(D_t - D_{t-1})$, which is still a predictable sequence because $D_t$ is predictable.

% We impose the constraint that $D_t\leq n$, i.e. the coin is tossed at most $n$ times (i.e., if needed, we can redefine $D_t' = D'_{t-1} +\ind{D_{t-1}\leq n}(D_t - D_{t-1})$, which is still predictable). 

% \guy{need to be careful about MG w.r.t. which filtration, and stopping times w.r.t. same filtration, in order to use OST. We might need separate filtrations for $D_t$ and $M_t$...}
We claim that 
$$
M_t = \prod_{i\leq t:\atop D_{i}' - D_{i-1}'=1} 3 X_i'
$$
is a submartingale, where $M_0=1$. Using the fact that $D_t'$ is a predictable sequence and that $\Pr(X_t' = 1|\Fc_{t-1}) \geq 1/3$ almost surely,
$$
\Ex[M_t|\Fc_{t-1}] =\Ex[ 3 X_t'|\Fc_{t-1}] M_{t-1}\ind{D_{t}'-D_{t-1}'=1}
+ M_{t-1}\ind{D_{t}'-D_{t-1}'=0}\geq M_{t-1}\,.
$$

For any fixed $s$, define the stopping times
$$T=\inf\{t:M_t=0\}\quad \text{and} \quad
S=\inf\{t:D_t'=s\}\,.
$$

\MK{Fix $S$ in terms of $M_t$.}


Note that since $X_i'\in \{0,1\}$, either $M_t=0$ or $M_t = 3^{D_t'}$.
Now by the optional stopping theorem\footnote{OST applies because for all $t$, $|M_{t\wedge S\wedge T}|\leq 3^s$.} applied to stopping time $T\wedge S$,
$$
1\leq \Ex M_{T\wedge S} = \Pr(T\leq S)\cdot 0 + \Pr(T>S)\Ex[3^{D_S'}|T> S] = \Pr(T>S) \cdot 3^s\,.
$$
The event $\{T>S\}$ is precisely the statement that at the first $t$ with $D_t'=s$, it is the case that $M_t\neq 0$, i.e.,
$X_i' = 1$ for all $i$ such that $K_i'$ occurs.

By definition, $t<  S$ if and only if $D_t'< s$ and  $t< T$ if and only if $M_t>0$. The event $\{S<T\}$ is the same as $\{t: t< S\}\subsetneq \{t:t<T\}$. In words, $\{S<T\}$ implies that for all $t$ such that $D_t'<  s$, $M_t>0$.
\begin{align*}
1/3^s\leq  \Pr(T>S) &= \Pr( \{t: t< S\}\subsetneq \{t:t<T\}) \\&\leq 
    \Pr(M_t>0  \text{ for all } t \text{ such that } D_t'<  s)\,.
\end{align*}
This proves the lemma. 
\end{proof}





%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\newpage
\MK{Old version which I think does not work}

\begin{lemma}\label{lem:stopped}
    Consider a discrete-time process $X_1,X_2,\dots$ with each $X_i\in \{0,1\}$ adapted to filtration $\Fc_t$ and a
    sequence of predictable events $K_1,K_2,\dots$, where $K_t\in \Fc_{t-1}$. Let $D_t = \sum_{i\leq t} \ind{K_i}$.
    If $\Pr(X_t = 1|\Fc_{t-1}, K_t, D_t= s) \geq 1/3$ almost surely for any $s\leq s^*$, then for any $s\leq s^*$
    % $$
    % \Pr(X_i = 1 \text{ for all } i\leq t \text{ such that } K_i \text{ occurs}|D_t)\geq 1/3^{D_t} \cdot \ind{D_t\leq s^*}\,.
    % $$
    $$
   \Pr( \text{ for all } t \text{ such that } D_t< s \text{ and all } i\leq t \text{ such that } K_i \text{ occurs}, X_i = 1  ) \geq 1/3^s
    \,.$$
\end{lemma}

% We first quickly show that Lemma~\ref{lem:stopped} follows from Lemma~\ref{lem:dt-mg}. 


\begin{proof}
Take $X_t, K_t$, and $D_t$ as in Lemma~\ref{lem:stopped}.
Define $$K'_t = K_t\cap \{D_{t-1} \leq s^*-1\}$$ and note that this is still a predictable event (i.e. in $\Fc_{t-1}$), and moreover, that $D_t\leq s^*$ on $K'_t$. 
Additionally define $X'_t = \max(X_t, \ind{{K'_t}^c})$, so that $X'_t=1$ automatically whenever $K_t'$ does not occur. 

We now show that $\Pr(X_t' = 1|\Fc_{t-1}) \geq 1/3$ almost surely. To start,
$$
 \Pr(X_t' = 1|\Fc_{t-1}, K_t^c)  = 1$$
 and
\begin{align*}  
 \Pr(X_t' = 1|\Fc_{t-1}, K_t) &=  
    \sum_{s=0}^{s^*} \Pr(X_t' = 1|\Fc_{t-1}, K_t, D_t= s)  \Pr( D_t= s|\Fc_{t-1}, K_t) 
   \\&\quad  +\sum_{s=s^*+1}^{\infty} \Pr(X_t' = 1|\Fc_{t-1}, K_t, D_t= s)  \Pr( D_t= s|\Fc_{t-1}, K_t) 
    \\
    & \geq \sum_{s=0}^{s^*}\frac{1}{3} \Pr( D_t= s|\Fc_{t-1}, K_t) 
    +\sum_{s=s^*+1}^{\infty}  \Pr( D_t= s|\Fc_{t-1}, K_t) \geq \frac{1}{3}\,.
\end{align*}
Here we used the lemma statement's assumption $\Pr(X_t = 1|\Fc_{t-1}, K_t, D_t= s) \geq 1/3$ a.s. for any $s\leq s^*$, together with the fact that $X_t'\geq X_t$ a.s., to bound the first term. We also used the fact that for $s>s^*$, $D_t= s$ implies ${K'_t}^c$ holds and hence $X_t' = 1$.
It follows that
$$
     \Pr(X_t' = 1|\Fc_{t-1}) 
      = \Pr(X_t' = 1|\Fc_{t-1}, K_t)  \Pr(K_t|\Fc_{t-1}) + \Pr(X_t' = 1|\Fc_{t-1}, K_t^c)  \Pr(K_t^c|\Fc_{t-1}) \geq \frac{1}{3}\,.
$$
     
We now apply Lemma~\ref{lem:dt-mg} to $X'_t$ and $K'_t$ and  $D'_t = \sum_{i\leq t} \ind{K'_i}$ to obtain that for any $s$,
\begin{align*}
           \Pr( \text{ for all } t \text{ such that } D_t'< s \text{ and all } i\leq t \text{ such that } K_i' \text{ occurs}, X_i' = 1  ) \geq 1/3^s\,.
\end{align*}
Note that for all $s\leq s^*$, $\{D_t=s\} = \{D'_t=s\}$. Additionally, if $D_t\leq s^*$, then
$$\{i\in [t]:K_i'\text{ occurs}\}= \{i\in [t]:K_i\text{ occurs}\}
\,,$$
so on event $\{D_t=s\}$ for any $s\leq s^*$, we have 
\[\big\{X'_i = 1 \text{ for all } i\leq t \text{ such that } K'_i \text{ occurs} \big\} = 
\big\{X_i = 1 \text{ for all } i\leq t \text{ such that } K_i \text{ occurs}\big\}\,. \]
Hence, for any $s\leq s^*$
\begin{align*}
       \Pr&( \text{for all } t \text{ such that } D_t< s \text{ and all } i\leq t \text{ such that } K_i \text{ occurs}, X_i = 1  )
       \\&\geq 
          \Pr( \text{for all } t \text{ such that } D_t'< s \text{ and all } i\leq t \text{ such that } K_i' \text{ occurs}, X_i' = 1  ) \geq 1/3^s\,.
\end{align*}
% \MK{old version:}
% \begin{align*}
%        \Pr(X_i = 1 \text{ for all }& i\leq t \text{ such that } K_i \text{ occurs}|D_t=s)
%      \\  &=
%         \Pr(X'_i = 1 \text{ for all } i\leq t \text{ such that } K'_i \text{ occurs}|D'_t=s)\geq 1/3^s\,.
% \end{align*}
\end{proof}


\begin{lemma}
\label{lem:dt-mg}
  Consider a discrete-time process $X_1', X_2',\dots$ with each $X_i'\in \{0,1\}$ adapted to filtration $\Fc_t$ and a
    sequence of predictable events $K_1',K_2',\dots$, where $K_t'\in \Fc_{t-1}$. Let $D_t' = \sum_{i\leq t} \ind{K_i'}$.
    If $\Pr(X_t' = 1|\Fc_{t-1}) \geq 1/3$ almost surely, then for any $s$
    % $$
    % \Pr(X_i = 1 \text{ for all } i\leq t \text{ such that } K_i \text{ occurs}|D_t)\geq 1/3^{D_t} \cdot \ind{D_t\leq s^*}\,.
    % $$
    $$
   \Pr( \text{ for all } t \text{ such that } D_t'< s \text{ and all } i\leq t \text{ such that } K_i' \text{ occurs}, X_i' = 1  ) \geq 1/3^s
    $$
\end{lemma}

\begin{proof}
    

% Let 
% $D_t' = D'_{t-1} +(D_t' - D_{t-1}') = D'_{t-1} +\ind{K_t'}$, which is still a predictable sequence because $D_t$ is predictable.


 
 % Now 
 % $\Ex[3X_t|\Fc_{t-1}]\geq 1$ almost surely and hence
 % $$M_t = 3^t X_1\cdots X_t$$
 % is a (sub)martingale.

% Let $T=\min\{t:Y_t=0\}$ be the first $0$. Then 
% $$
% 1 \leq  \Ex M_{n\wedge T} = \Pr(T>n) 3^n\,,
% $$
% where we used the fact that if $T\leq n$, then $M_{n\wedge T}=0$.

% Now let $H_t$ be a predictable sequence. This is going to be our rule for if we toss a coin at time $t$ and is a function of outcomes at times $t-1$ and earlier. We set $H_t=1$ if we toss the coin at time $t$ and $0$ otherwise. The martingale transform
% $$
% D_t =(H\circ M)_t = \sum_{i=1}^t H_i (M_i - M_{i-1}) =  \sum_{i=1}^t H_i (3 X_i - 1)M_{i-1}
% $$
% is also a martingale. 
% Let $D_t-D_{t-1}\in\{0,1\}$ be the times at which we toss the coin and suppose that $D_t$ is predictable, i.e., $D_t\in \mathcal{F}_{t-1}$. 

% Let 
% $D_t' = D'_{t-1} +\ind{D_{t-1}\leq s^*-1}(D_t - D_{t-1})$, which is still a predictable sequence because $D_t$ is predictable.

% We impose the constraint that $D_t\leq n$, i.e. the coin is tossed at most $n$ times (i.e., if needed, we can redefine $D_t' = D'_{t-1} +\ind{D_{t-1}\leq n}(D_t - D_{t-1})$, which is still predictable). 

% \guy{need to be careful about MG w.r.t. which filtration, and stopping times w.r.t. same filtration, in order to use OST. We might need separate filtrations for $D_t$ and $M_t$...}
We claim that 
$$
M_t = \prod_{i\leq t:\atop D_{i}' - D_{i-1}'=1} 3 X_i'
$$
is a submartingale, where $M_0=1$. Using the fact that $D_t'$ is a predictable sequence and that $\Pr(X_t' = 1|\Fc_{t-1}) \geq 1/3$ almost surely,
$$
\Ex[M_t|\Fc_{t-1}] =\Ex[ 3 X_t'|\Fc_{t-1}] M_{t-1}\ind{D_{t}'-D_{t-1}'=1}
+ M_{t-1}\ind{D_{t}'-D_{t-1}'=0}\geq M_{t-1}\,.
$$

For any fixed $s$, define the stopping times
$$T=\inf\{t:M_t=0\}\quad \text{and} \quad
S=\inf\{t:D_t=s\}\,.
$$
Note that since $X_i'\in \{0,1\}$, either $M_t=0$ or $M_t = 3^{D_t'}$.
Now by the optional stopping theorem\footnote{OST applies because for all $t$, $|M_{t\wedge S\wedge T}|\leq 3^s$.} applied to stopping time $T\wedge S$,
$$
1\leq \Ex M_{T\wedge S} = \Pr(T\leq S)\cdot 0 + \Pr(T>S)\Ex[3^{D_S}|T> S] = \Pr(T>S) \cdot 3^s\,.
$$
The event $\{T>S\}$ is precisely the statement that at the first $t$ with $D_t'=s$, it is the case that $M_t\neq 0$, i.e.,
$X_i' = 1$ for all $i$ such that $K_i'$ occurs.

By definition, $t<  S$ if and only if $D_t'< s$ and  $t< T$ if and only if $M_t>0$. The event $\{S<T\}$ is the same as $\{t: t< S\}\subsetneq \{t:t<T\}$. In words, $\{S<T\}$ implies that for all $t$ such that $D_t'<  s$, $M_t>0$.
\begin{align*}
1/3^s\leq  \Pr(T>S) &= \Pr( \{t: t< S\}\subsetneq \{t:t<T\}) \\&\leq 
    \Pr(M_t>0  \text{ for all } t \text{ such that } D_t'<  s)\,.
\end{align*}
This proves the lemma. 
\end{proof}




% \subsection{martingale}

% % \begin{lemma}\label{lem:dt-mg}
% %     Consider a discrete-time process $X_1,X_2,\dots$ with each $X_i\in \{0,1\}$ adapted to filtration $\Fc_t$ and a
% %     sequence of predictable events $K_1,K_2,\dots$, where $K_t\in \Fc_{t-1}$. Let $D_t = \sum_{i\leq t} \ind{K_i}$.
% %     If $\Pr(X_t = 1|\Fc_{t-1}) \geq 1/3$ almost surely, then
% %     $$
% %     \Pr(X_i = 1 \text{ for all } i\leq t \text{ such that } K_i \text{ occurs}|D_t=s)\geq 1/3^s\,.
% %     $$
% % \end{lemma}


% \begin{lemma}\label{lem:stopped}
%     Consider a discrete-time process $X_1,X_2,\dots$ with each $X_i\in \{0,1\}$ adapted to filtration $\Fc_t$ and a
%     sequence of predictable events $K_1,K_2,\dots$, where $K_t\in \Fc_{t-1}$. Let $D_t = \sum_{i\leq t} \ind{K_i}$.
%     If $\Pr(X_t = 1|\Fc_{t-1}, D_t= s) \geq 1/3$ almost surely for any $s\leq s^*$, then for any $s\leq s^*$
%     % $$
%     % \Pr(X_i = 1 \text{ for all } i\leq t \text{ such that } K_i \text{ occurs}|D_t)\geq 1/3^{D_t} \cdot \ind{D_t\leq s^*}\,.
%     % $$
%     $$
%    \Pr( \text{ for all } t \text{ such that } D_t< s \text{ and all } i\leq t \text{ such that } K_i \text{ occurs}, X_i = 1  ) \geq 1/3^s
%     $$
% \end{lemma}
% % We first quickly show that Lemma~\ref{lem:stopped} follows from Lemma~\ref{lem:dt-mg}. 

% Take $X_t, K_t$, and $D_t$ as in Lemma~\ref{lem:stopped}.
% Define $$K'_t = K_t\cap \{D_{t-1}\leq s^*-1\}$$ and note that this is still a predictable event (i.e. in $\Fc_{t-1}$), and moreover, that $D_t\leq s^*$ on $K'_t$. 
% Additionally define $X'_t = \max(X_t, \ind{{K'_t}^c})$, so that $X'_t=1$ automatically whenever $K_t'$ does not occur, and hence $\Pr(X_t' = 1|\Fc_{t-1}) \geq 1/3$ almost surely. 

% \MK{I added the reasoning for this in the following display:}
% \begin{align*}
%     \Pr(X_t' = 1|\Fc_{t-1}) 
%     & = \sum_{s=0}^{s^*} \Pr(X_t' = 1|\Fc_{t-1}, D_t= s)  \Pr( D_t= s|\Fc_{t-1}) 
%    \\&\quad  +\sum_{s=s^*+1}^{\infty} \Pr(X_t' = 1|\Fc_{t-1}, D_t= s)  \Pr( D_t= s|\Fc_{t-1}) 
%     \\
%     & \geq \sum_{s=0}^{s^*}\frac{1}{3} \Pr( D_t= s|\Fc_{t-1}) 
%     +\sum_{s=s^*+1}^{\infty}  \Pr( D_t= s|\Fc_{t-1}) \geq \frac{1}{3}\,.
% \end{align*}
% where we used $\Pr(X_t = 1|\Fc_{t-1}, D_t= s) \geq 1/3$ almost surely for any $s\leq s^*$ to bound the first term. We also used the fact that for $s>s^*$, $D_t= s$ implies ${K'_t}^c$ holds and hence $X_t' = 1$.


% We now apply Lemma~\ref{lem:dt-mg} to $X'_t$ and $K'_t$ and  $D'_t = \sum_{i\leq t} \ind{K'_i}$. 
% % Now, we have the containment of events
% This implies that for any $s$,
% \begin{align*}
%            \Pr( \text{ for all } t \text{ such that } D_t'< s \text{ and all } i\leq t \text{ such that } K_i' \text{ occurs}, X_i' = 1  ) \geq 1/3^s\,.
% \end{align*}
% Note that for all $s\leq s^*$, $\{D_t=s\} = \{D'_t=s\}$. Additionally, if $D_t\leq s^*$, then
% $$\{i\in [t]:K_i'\text{ occurs}\}= \{i\in [t]:K_i\text{ occurs}\}
% \,,$$
% so on event $\{D_t=s\}$ for any $s\leq s^*$, we have 
% \[\big\{X'_i = 1 \text{ for all } i\leq t \text{ such that } K'_i \text{ occurs} \big\} \subseteq 
% \big\{X_i = 1 \text{ for all } i\leq t \text{ such that } K_i \text{ occurs}\big\}\,. \]
% Hence, for any $s\leq s^*$
% \begin{align*}
%        \Pr&( \text{ for all } t \text{ such that } D_t< s \text{ and all } i\leq t \text{ such that } K_i \text{ occurs}, X_i = 1  )
%        \\&\geq 
%           \Pr( \text{ for all } t \text{ such that } D_t'< s \text{ and all } i\leq t \text{ such that } K_i' \text{ occurs}, X_i' = 1  ) \geq 1/3^s
% \end{align*}

% \MK{old version:}
% \begin{align*}
%        \Pr(X_i = 1 \text{ for all }& i\leq t \text{ such that } K_i \text{ occurs}|D_t=s)
%      \\  &=
%         \Pr(X'_i = 1 \text{ for all } i\leq t \text{ such that } K'_i \text{ occurs}|D'_t=s)\geq 1/3^s\,.
% \end{align*}


% \MK{I added this lemma}

% \begin{lemma}
% \label{lem:dt-mg}
%   Consider a discrete-time process $X_1', X_2',\dots$ with each $X_i'\in \{0,1\}$ adapted to filtration $\Fc_t$ and a
%     sequence of predictable events $K_1',K_2',\dots$, where $K_t'\in \Fc_{t-1}$. Let $D_t' = \sum_{i\leq t} \ind{K_i'}$.
%     If $\Pr(X_t' = 1|\Fc_{t-1}) \geq 1/3$ almost surely, then for any $s$
%     % $$
%     % \Pr(X_i = 1 \text{ for all } i\leq t \text{ such that } K_i \text{ occurs}|D_t)\geq 1/3^{D_t} \cdot \ind{D_t\leq s^*}\,.
%     % $$
%     $$
%    \Pr( \text{ for all } t \text{ such that } D_t'< s \text{ and all } i\leq t \text{ such that } K_i' \text{ occurs}, X_i' = 1  ) \geq 1/3^s
%     $$
% \end{lemma}

% \begin{proof}
    

% Let 
% $D_t' = D'_{t-1} +(D_t' - D_{t-1}') = D'_{t-1} +\ind{K_t'}$, which is still a predictable sequence because $D_t$ is predictable.

%  Note that $\Pr(X_t = 1|\Fc_t)\geq 1/3$. 
 
%  % Now 
%  % $\Ex[3X_t|\Fc_{t-1}]\geq 1$ almost surely and hence
%  % $$M_t = 3^t X_1\cdots X_t$$
%  % is a (sub)martingale.

% % Let $T=\min\{t:Y_t=0\}$ be the first $0$. Then 
% % $$
% % 1 \leq  \Ex M_{n\wedge T} = \Pr(T>n) 3^n\,,
% % $$
% % where we used the fact that if $T\leq n$, then $M_{n\wedge T}=0$.

% % Now let $H_t$ be a predictable sequence. This is going to be our rule for if we toss a coin at time $t$ and is a function of outcomes at times $t-1$ and earlier. We set $H_t=1$ if we toss the coin at time $t$ and $0$ otherwise. The martingale transform
% % $$
% % D_t =(H\circ M)_t = \sum_{i=1}^t H_i (M_i - M_{i-1}) =  \sum_{i=1}^t H_i (3 X_i - 1)M_{i-1}
% % $$
% % is also a martingale. 
% % Let $D_t-D_{t-1}\in\{0,1\}$ be the times at which we toss the coin and suppose that $D_t$ is predictable, i.e., $D_t\in \mathcal{F}_{t-1}$. 

% % Let 
% % $D_t' = D'_{t-1} +\ind{D_{t-1}\leq s^*-1}(D_t - D_{t-1})$, which is still a predictable sequence because $D_t$ is predictable.

% % We impose the constraint that $D_t\leq n$, i.e. the coin is tossed at most $n$ times (i.e., if needed, we can redefine $D_t' = D'_{t-1} +\ind{D_{t-1}\leq n}(D_t - D_{t-1})$, which is still predictable). 

% % \guy{need to be careful about MG w.r.t. which filtration, and stopping times w.r.t. same filtration, in order to use OST. We might need separate filtrations for $D_t$ and $M_t$...}
% We claim that 
% $$
% M_t = \prod_{i\leq t:\atop D_{i}' - D_{i-1}'=1} 3 X_i'
% $$
% is a submartingale, where $M_0=1$:
% $$
% \Ex[M_t|\Fc_{t-1}] =\Ex[ 3 X_t'|\Fc_{t-1}] M_{t-1}\ind{D_{t}'-D_{t-1}'=1}
% + M_{t-1}\ind{D_{t}'-D_{t-1}'=0}\geq M_{t-1}\,.
% $$
% It's justified based on the assumption in the lemma.
% % Here we used that
% % $$
% % \Ex[ 3 X_t'|\Fc_{t-1}] M_{t-1}\ind{D_{t}'-D_{t-1}'=1} \geq M_{t-1}\ind{D_{t}'-D_{t-1}'=1}\,,
% % $$
% % because either both sides are zero, or $D_{t}-D_{t-1}=1$ which implies that $D_{t-1}\leq s^*-1$ and hence $D_t' \leq s^*$ and $\Pr(X_t=1|\Fc_{t-1})\geq 1/3$.

% Note that since $X_i'\in \{0,1\}$ either $M_t=0$ or $M_t = 3^{D_t'}$.

% Given $s$, define the stopping times
% $$T=\inf\{t:M_t=0\}\quad \text{and} \quad
% S=\inf\{t:D_t=s\}\,.
% $$
% Now by the optional stopping theorem applied to stopping time $T\wedge S$,\guy{based on (105) you seem to want to condition on $S=t$}
% $$
% 1\leq \Ex M_{T\wedge S} = \Pr(T\leq S)\cdot 0 + \Pr(T>S)\Ex[3^{D_S}|T> S] = \Pr(T>S) \cdot 3^s\,.
% $$
% Now event $\{T>S\}$ is precisely the statement that at the first $t$ with $D_t'=s$, it is the case that $M_t\neq 0$, i.e.,
% $X_i' = 1$ for all $i$ such that $K_i'$ occurs.

% By definition, $t< S$ if and only if $D_t'<s$ and  $t< T$ if and only if $M_t>0$. On the event $\{S<T\}$, for all $t\leq S<T$,  $D_t'< s$ and $M_t>0$ hence:
% \[1/3^s\leq  \Pr(T>S) \leq \Pr(M_t>0  \text{ for all } t \text{ such that } D_t'< s)\,.\]
% % We claim that for any martingale $M_t$, the sequence $(M_{D'_t})_{t\geq 0}$ is also a martingale with respect to filtration $\Fc_{D'_t}$:
% % $$
% % \Ex[M_{D'_t}|\Fc_{D'_{t}-1}]
% % $$
% % If that is true, we note that $M_{n\wedge t}$ is a martingale, and hence so is $M_{n\wedge D_{ t}}$. Define the stopping times
% % $$T=\inf\{t:M_t=0\text{ and } D_t-D_{t-1}=1\}$$
% % and
% % $$
% % \tau=\inf\{t:D_t=s\}\,.
% % $$
% % Now we use the optional stopping theorem (check that conditions hold!) to get
% % \begin{align}
% %    1 \leq \Ex M_{ D_{ T\wedge \tau}} 
% %    &= \Pr(T\leq \tau) \cdot 0 
% %    % \\&\quad + \Pr(T> \tau, H_{T\wedge \tau} > n) \cdot 3^{n} + \Pr(T\leq  \tau, H_{T\wedge \tau} > n) \cdot 3^{n} 
% %        + \Pr(T> \tau)  \cdot \Ex[3^{D_\tau}|T> \tau] 
% %     \\&\leq 
% %      \Pr(T > \tau) 3^s
% % \end{align}
% \end{proof}

% \MK{Guy had the following proof.}
% \begin{proof}
    
% % Note that $\Pr(X_t = 1|\Fc_t)\geq 1/3$. 
% % Now 
% % $\Ex[3X_t|\Fc_{t-1}]\geq 1$ almost surely and hence
% % $$M_t = 3^t X_1\cdots X_t$$
% % is a (sub)martingale.

% % Let $T=\min\{t:Y_t=0\}$ be the first $0$. Then 
% % $$
% % 1 \leq  \Ex M_{n\wedge T} = \Pr(T>n) 3^n\,,
% % $$
% % where we used the fact that if $T\leq n$, then $M_{n\wedge T}=0$.

% % Now let $H_t$ be a predictable sequence. This is going to be our rule for if we toss a coin at time $t$ and is a function of outcomes at times $t-1$ and earlier. We set $H_t=1$ if we toss the coin at time $t$ and $0$ otherwise. The martingale transform
% % $$
% % D_t =(H\circ M)_t = \sum_{i=1}^t H_i (M_i - M_{i-1}) =  \sum_{i=1}^t H_i (3 X_i - 1)M_{i-1}
% % $$
% % is also a martingale. 
% % Let $D_t-D_{t-1}\in\{0,1\}$ be the times at which we toss the coin and suppose that $D_t$ is predictable, i.e., $D_t\in \mathcal{F}_{t-1}$. 

% Let 
% $D_t' = D'_{t-1} +\ind{D_{t-1}\leq s^*-1}(D_t - D_{t-1})$, which is still a predictable sequence because $D_t$ is predictable.

% % We impose the constraint that $D_t\leq n$, i.e. the coin is tossed at most $n$ times (i.e., if needed, we can redefine $D_t' = D'_{t-1} +\ind{D_{t-1}\leq n}(D_t - D_{t-1})$, which is still predictable). 

% % \guy{need to be careful about MG w.r.t. which filtration, and stopping times w.r.t. same filtration, in order to use OST. We might need separate filtrations for $D_t$ and $M_t$...}
% We claim that 
% $$
% M_t = \prod_{i\leq t:\atop D_{i} - D_{i-1}=1} 3 X_i
% $$
% is a submartingale:
% $$
% \Ex[M_t|\Fc_{t-1}] =\Ex[ 3 X_t|\Fc_{t-1}] M_{t-1}\ind{D_{t}-D_{t-1}=1}
% + M_{t-1}\ind{D_{t}-D_{t-1}=0}\geq M_{t-1}\,.
% $$
% Here we used that
% $$
% \Ex[ 3 X_t|\Fc_{t-1}] M_{t-1}\ind{D_{t}-D_{t-1}=1} \geq M_{t-1}\ind{D_{t}-D_{t-1}=1}\,,
% $$
% because either both sides are zero, or $D_{t}-D_{t-1}=1$ which implies that $D_{t-1}\leq s^*-1$ and hence $D_t \leq s^*$ and $\Pr(X_t=1|\Fc_{t-1})\geq 1/3$.
% Define the stopping times
% $$T=\inf\{t:M_t=0\}\quad \text{and} \quad
% S=\inf\{t:D_t=s\}\,.
% $$
% Now by the optional stopping theorem applied to stopping time $T\wedge S$,\guy{based on (105) you seem to want to condition on $S=t$}
% $$
% 1\leq \Ex M_{T\wedge S} = \Pr(T\leq S)\cdot 0 + \Pr(T>S)\Ex[3^{D_S}|T> S] = \Pr(T>S) \cdot 3^s\,.
% $$
% Now event $\{T>S\}$ is precisely the statement that at the first $t$ with $D_t=s$, it is the case that $M_t\neq 0$, i.e.,
% $X_i = 1$ for all $i$ such that $K_i$ occurs.

% By definition, $t< S$ if and only if $D_t<s$ and  $t< T$ if and only if $M_t>0$. On the event $\{S<T\}$, for all $t\leq S<T$,  $D_t< s$ and $M_t>0$ hence:
% \[ \Pr(T>S) \leq \Pr(M_t>0  \text{ for all } t \text{ such that } D_t< s)\,.\]
% % We claim that for any martingale $M_t$, the sequence $(M_{D'_t})_{t\geq 0}$ is also a martingale with respect to filtration $\Fc_{D'_t}$:
% % $$
% % \Ex[M_{D'_t}|\Fc_{D'_{t}-1}]
% % $$
% % If that is true, we note that $M_{n\wedge t}$ is a martingale, and hence so is $M_{n\wedge D_{ t}}$. Define the stopping times
% % $$T=\inf\{t:M_t=0\text{ and } D_t-D_{t-1}=1\}$$
% % and
% % $$
% % \tau=\inf\{t:D_t=s\}\,.
% % $$
% % Now we use the optional stopping theorem (check that conditions hold!) to get
% % \begin{align}
% %    1 \leq \Ex M_{ D_{ T\wedge \tau}} 
% %    &= \Pr(T\leq \tau) \cdot 0 
% %    % \\&\quad + \Pr(T> \tau, H_{T\wedge \tau} > n) \cdot 3^{n} + \Pr(T\leq  \tau, H_{T\wedge \tau} > n) \cdot 3^{n} 
% %        + \Pr(T> \tau)  \cdot \Ex[3^{D_\tau}|T> \tau] 
% %     \\&\leq 
% %      \Pr(T > \tau) 3^s
% % \end{align}
% \end{proof}
% \guy{discussion about what we want to prove vs what we have proved}
% Let 
% $$
% E_t=\{X_i = 1 \text{ for all } i\leq t \text{ such that } K_i \text{ occurs}\}\,.
% $$
% If our aim is (105) then we want to lower bound $\Pr(E_t|D_t=s)$.
% What we seem to have proved is
% $$
% \Pr(\bigcup_{t\geq 1} (\{S = t\}\cap E_t))\geq 1/3^s\,.
% $$

% Let $S_s$ be the obvious thing. We apparently want to bound $P(T>t| S_s\leq t< S_{s+1})$

% % \subsection{Mina's product argument:}
% % \begin{align*}
% %     \Pr[d_u^t = a , \liked{u}t = b
% %     & = 
% %     \Pr \left[ \sum_{s=1}^t \ident\{ (\BBjil{u}{a_{u,s}}{s})^c\} =a ,
% %     \,\,\sum_{s=1}^t \ident\{L_{u,a_{u,t}} = +1 , (\BBjil{u}{a_{u,s}}{s})^c\} =b \right]
% %     \\ & = 
% %     \sum_{L\in {t \choose a}}
% %     \sum_{M\in {a \choose b}}
% % \end{align*}

\subsection{Incorporating it into regret}



% Here we combine the statements of Lemmas~\ref{l:BoundBad1},~\ref{l:BoundBad2},~\ref{l:BoundBad3},~\ref{l:BoundBad4}, and ~\ref{l:BoundBad5}  to to get a minimax statement as a lower bound for number of bad recommendations.

\MK{Notes for Mina to figure things out}
\begin{align*}
    \bad(T)
    &\geq 
    \sum_{u\in [N]} \left[ \min\{d_u^T , \tul\} + 
    (T-d_u^T)\ind{\liked{u}{t} = 0} + n_T(\min_u d_u^T)\right]
    \end{align*}
    
    \begin{align*}
    &\Ex\left[\min\{d_u^T , \tul\} + 
    (T-d_u^T)\ind{\liked{u}{t} = 0} + n_T(\min_u d_u^T)\right]
    \\
    &\geq 
      \Ex\left[\min\{d_u^T , \tul\} + 
    (T-d_u^T)\ind{\liked{u}{t} = 0} + n_T(\min_u d_u^T)
    \, \Big|\, d_u^T <s\right] \Pr(d_{u}^T<s)
         \\&+ 
     \Ex\left[\min\{d_u^T , \tul\}
    (T-d_u^T)\ind{\liked{u}{t} = 0} + n_T(\min_u d_u^T)\, \Big|\, d_u^T \geq s\right] \Pr(d_{u}^T\geq s)
\end{align*}

\MK{Wild idea: Write $n_T(d^*) = \sum_{r=1}^{\infty} \ind{n_T(d^*) \geq r}$ so we can talk about some of indicator variables and use linearity of expectation!!!!!!}




\MK{I added this paragraph:}
\paragraph{Disliked Item Types to Weakly Explored Users}


\begin{lemma}
\label{l:BoundBad5}
The  number of bad recommendations $\bad(T)$,  defined in Equation~\eqref{eq:jl-def-bad}, satisfies 
\begin{align*}
\bad(T)
\geq \sum_{\substack{t\in[T]\\ u\in[N]}}
\ind{\Bsf{1}_{u,t}}
\geq
\sum_{\substack{ u\in[N]}}
 (T- d_u^{T+1})\ind { d_u^T <\tul, \liked{u}{T} = 0} 
\end{align*}
\end{lemma}
\begin{proof}
For any $u$,
\begin{align*}    
 %   \label{e:B5}
    \sum_{t=1}^T\ind{\Bsf{5}_{u,t}}
   & \geq \sum_{t=1}^T \ind { d_u^t <\tul, \liked{u}{t} = 0, \BBjil{u}{a_{u,t}}{t}} 
    \\
    &\geq \sum_{t=1}^T \ind { d_u^T <\tul, \liked{u}{T} = 0, \BBjil{u}{a_{u,t}}{t}} 
\\
  &  \geq (T- d_u^{T+1})\ind { d_u^T <\tul, \liked{u}{T} = 0} 
 \,.
\end{align*}
The event $\liked{u}{T} = 0$, implies that the user $u$ has disliked all the item type she's been recommended up to and including time $T$.
 $\Bsf{5}_{u,t}$ is the event on which a previously rated, and \textit{disliked} item type is recommended to a user with unknown user type.  On event $\liked{u}{T} = 0$, the number of such recommendations is $T- d_u^{T+1}$.

 For any $u\notin \Wc^T$, $d_u^T <\tul$ and $d_{u}^{T+1}\geq \gamma_*^T$ for all $u$. Hence,
 \begin{align*}    
 %   \label{e:B5}
    \sum_{\substack{t\in[T]\\ u\in[N]}}\ind{\Bsf{5}_{u,t}}
   & \geq \sum_{u\notin \Wc^{T}} (T- d_u^{T+1})\ind {\liked{u}{T} = 0} 
   \geq 
  (1-w^T)N (T-\gamma_*^T) \ind {\liked{*}{T} = 0} 
 \,.
\end{align*}

\newpage

For any $\leq d \leq $
\begin{align}
\Pr\left[\liked{u}{T}\leq 
 T \ident\big\{d_u^T > \min\{\log T,\tul\}\big\} | d_u^T = d
\right]\geq \frac{\log T}{T}
\end{align}


$u\notin \Wc_t$, $d_u^T <\tul$
\begin{align*}
     d_u ^{T+1} +  (T- d_u^{T+1})\ind { d_u^T <\tul, \liked{u}{T} = 0} 
\end{align*}
If $\log T < d_u^T <\tul$:







\guy{below is $\tul$}

$u\notin \Wc_t$, $d_u^T \geq \tul$
\begin{align*}
    \tul +  (T- d_u^{T+1})\ind { d_u^T <\tul, \liked{u}{T} = 0} =\tul
\end{align*}

\begin{align}
  \min(d_u^T, \tul) + (T- d_u^{T+1})\ind { d_u^T <\tul, \liked{u}{T} = 0} 
\end{align}

Define event $E:\b\{ \liked{u}{T}\leq 
 T \ident\big\{d_u^T > \min\{\log T,\tul\}\big\}\b\}$. Then, $\Pr(E)\geq \log T/T$

 
Let
$$
s^*:=\min\{\log T,\tul\}-1
$$
and let $d_u^+(a)$ be the number of liked item types out of the first $a$ item types recommended to user $u$. Define
$$
E = \{d_u^+(s^*\wedge d_u^T) = 0\}, \quad F = \{ d_u^T > s^*\}
$$
On $F^c\cap E$, $0=d_u^+(s^*\wedge d_u^T) = d_u^+(d_u^T)$, i.e., all items up to time $T$ are disliked. 
This implies that $$\Ex[\bad(T)|E,F^c]\geq T\,.$$ Hence
 \begin{align}
     \Ex[\bad(T)] &\geq \Ex[\bad(T)|F]\Pr(F) + \Ex[\bad(T)|F^c]\Pr(F^c)
     \\&\geq \min\{\log T,\tul\}\Pr(F) + \Ex[\bad(T)|E,F^c]\Pr(E,F^c) + \Ex[\bad(T)|E^c,F^c]\Pr(E^c,F^c)
     % + \Ex[\bad(T)|E^c,F^c]\Pr(E^c,F^c)
     \\&\geq \min\{\log T,\tul\}\Pr(F) + T \Pr(E|F^c)\Pr(F^c)\,.
     \end{align}
Next, observe that $\Pr(E|F^c) \geq \Pr(d_u^+(d_u^T)=0|F^c)$. By Lemma ???, this is at least $1/3^{s^*}$.


Let $T=s^*$. Then $d_u^T\leq s^*$ and $F$ cannot occur.
 \begin{align}
     \Ex[\bad(S\wedge t)] &=   \Ex[\bad(S\wedge t)|E]\Pr(E) + \Ex[\bad(S\wedge t)|E^c]\Pr(E^c)
     % + \Ex[\bad(T)|E^c,F^c]\Pr(E^c,F^c)
     \\&\geq (t\wedge \Ex[S|E]) \Pr(E) 
     \geq  t 3^{-s} + s \Pr(E^c)  \,.
\\
   t 3^{-s} + s &\geq    \log t
     \end{align}



 \begin{align}
     \bad(t) &= \bad(t-1) + \ind{K_t} X_t + 
     \ind{K_t^c}\ind{\prod_{i< t\atop K_i=1} X_i=1}
     \\
     &= \bad(t-1) + \ind{K_t} X_t + 
     \ind{K_t^c}\ind{E_{t-1}}
     \end{align}

     \begin{align}
     \Pr(X_t| \Fc_{t-1}) &\geq 1/3\,.
     \end{align}




\begin{align}
&\Ex[\min(d_u^T, \tul) + (T- d_u^{T+1})\ind { d_u^T <\tul, \liked{u}{T} = 0} ]
\\ &= \Ex[\min(d_u^T, \tul) + (T- d_u^{T+1})\ind { d_u^T <\tul, \liked{u}{T} = 0}\ident_E \\&\qquad+ (T- d_u^{T+1})\ind { d_u^T <\tul, \liked{u}{T} = 0}\ident_{E^c} ]
\\&\geq  \Ex[\min(d_u^T, \tul) + (T- d_u^{T+1}) \ident\big\{d_u^T \leq \min\{\log T,\tul\}\} \ident_E]
\end{align}

Suppose:
\begin{itemize}
    \item $\Pr(E|d_u^T)\geq \log T / T$ almost surely (i.e., for all $d_u^T$
    \item 
\end{itemize}
Then
\begin{align}
&\Ex[\min(d_u^T, \tul) + (T- d_u^{T+1})\ind { d_u^T <\tul, \liked{u}{T} = 0} ]
\\&=
\Ex[\Ex[\min(d_u^T, \tul) + (T- d_u^{T+1})\ind { d_u^T <\tul, \liked{u}{T} = 0} |d_u^T]]
\\ &= \Ex[\min(d_u^T, \tul) + (T- d_u^{T+1})\ind { d_u^T <\tul, \liked{u}{T} = 0}\ident_E \\&\qquad+ (T- d_u^{T+1})\ind { d_u^T <\tul, \liked{u}{T} = 0}\ident_{E^c} ]
\\&\geq  \Ex[\min(d_u^T, \tul) + (T- d_u^{T+1}) \ident\big\{d_u^T \leq \min\{\log T,\tul\}\} \ident_E]
\end{align}

\begin{align}
\bad&\geq \Ex[\min(d_u^T, \tul) + (T- d_u^{T+1})\ind { d_u^T <\tul, \liked{u}{T} = 0} ]
\\&\geq 
\Ex[\min(d_u^T, \tul) + (T- d_u^{T+1})\ind { d_u^T <\min\{\tul,\log T\}, \liked{u}{T} = 0}]
\\&\geq 
\Ex[\min(d_u^T, \tul) + \frac{T}{2}\ind { d_u^T <\min\{\tul,\log T\}, \liked{u}{T} = 0} ]
\\
\bad&\geq \Ex[n_T(d^*), \qu d^{*}, T\min\{\til,\qu\}]
\\
\bad(T)& \geq \Ex[n_T, \min(d_u^T, \tul) + \frac{T}{2}\ind { d_u^T <\min\{\tul,\log T\}, \liked{u}{T} = 0}]
\end{align}

\newpage
\end{proof}

==> minimax.tex <==

Define 
\begin{align*}
f_1(\gamma) 
&=
\begin{cases}
T\qi / (4\gamma) & \text{ if } \gamma < T/(8\log \qi)
 \\
 1  & \text{ if } \gamma > T/(8\log \qi)
 \end{cases}
 \quad \quad
f_2(\gamma)= \max\big\{ \frac{N}{\Lambda} \gamma,\frac{N}{2}, \min\{\thrjul,\gamma\}\big\}
\\
f_3(\gamma)&=
T \min\big\{\thrjil, \frac{N}{\Lambda }\big\}\,.
 \end{align*}
Then, 
\begin{align*}
\Ex\big[\bad(T)\big]
\geq 
\frac{1}{4}
\min_{\gamma\geq 1}
\max\big\{
f_1(\gamma), f_2(\gamma), f_{3}(\gamma)\big\}\,.
\end{align*}
\begin{figure}[h]
\includegraphics[width=15cm]{figures/LBf}
\caption{The functions}
\label{fig:LBfig}
\centering
\end{figure}
Note that the functions $f_1(\gamma), f_2(\gamma)$ and constant function $f_{3}(\gamma)$ are parameterized by the parameters of the system $\qu, \qi, N$ and $T$. So depending on the realization of these parameters, the above minimax takes different forms. 
To lower bound the minimax term, we observe that $f_{1}(\gamma)$ is a nonincreasing function of $\gamma$; $f_{2}(\gamma)$ is a nondecreasing function of $\gamma$; and $f_{3}(\gamma)$ is a constant function of $\gamma$ (Figure~\ref{fig:LBfig}). 




\newpage
Define 
$f(\gamma) = T\qi / (4\gamma)$ 
and 
$g(\gamma)= \frac{N}{2}\max\big\{ \frac{\gamma}{\Lambda}, \min\{r,\gamma\}\big\}$.
Also, define $\gamma_1$ to be the intersection of the above two curves.  Note that $f(\gamma)$ is decreasing in $\gamma$ and $g(\gamma)$ is nondecreasing in $\gamma$. 

Note that 
\begin{align*}
\Theta_{\qi}(T/\gamma) 
=
\begin{cases}
 f(\gamma) & \text{ if } \gamma > T/(8\log \qi)
 \\
 1  & \text{ if } \gamma < T/(8\log \qi)
 \end{cases}
 \end{align*}
To lower bound regret, we look at two cases

\paragraph{Case I : $\gamma_1\geq\frac{T}{8\log \qi}$:} Alternatively, this condition corresponds to $g(T/(8\log \qi)) \leq f(T/(8\log \qi)) $.
Then, 
\begin{align*}
&\min_{\gamma_*^T}\,\, 
\max\Big\{ \Theta_{\qi}\left(\frac{T}{\gamma_*^T}\right),\,
\frac{N\gamma_*^T}{2\Lambda_{\qu}(N)},\, 
\frac{N}{2}\min\{\gamma_*^T,\, \thrjul\},\,
\Big\}
 \geq 
g(T/(8\log \qi))
\\
&\text{and } 
\Ex\big[\bad(T)\big] \geq 
\max\Big\{ 
g(T/(8\log \qi)) ,  T \min\{\thrjil, \frac{N}{1+\thrjil \Lambda_{\qu}(N) }\}
\Big\}
\end{align*}

\paragraph{Case II : $\gamma_1\leq \frac{T}{8\log \qi}$:}
Then, 

\begin{align*}
\min_{\gamma_*^T}\,\, 
\max\Big\{ \Theta_{\qi}\left(\frac{T}{\gamma_*^T}\right),\,
&
\frac{N\gamma_*^T}{2\Lambda_{\qu}(N)},\, 
\frac{N}{2}\min\{\gamma_*^T,\, \thrjul\},\,
\Big\}
 \geq 
f(\gamma_1)
\\
\text{and } \quad\quad\quad
\Ex\big[\bad(T)\big]&\geq 
\max\Big\{ 
f(\gamma_1),  T \min\{\thrjil, \frac{N}{1+\thrjil \Lambda_{\qu}(N) }\}
\Big\}
\end{align*}

This implies that if
$2\qu\log \qu<N\leq 4\frac{\qi}{\thrjul} \log\qi$, 
\begin{align*}
\Ex\big[\bad(T)\big]
&\geq C
\begin{cases} 
% &\text{if }T \leq \min\{  32\frac{\qi}{\qu}\log\qi,  \frac{N\thrjul^2}{\qi}\}
%\\
\sqrt{T\qi N}
&\text{if } 32\frac{\qi}{\qu}\log\qi < T \leq \frac{N\thrjul^2}{\qi}
\\
 N \thrjul
&\text{if }  \frac{N\thrjul^2}{\qi} < T \leq\frac{N^2\thrjul^2}{\qu\qi} 
\\
\sqrt{T\qi \qu}
&\text{if }  \frac{N^2\thrjul^2}{\qu\qi} < T \leq \qi\qu/(\thrjul^2)
\\
T \thrjil
&\text{if }  \qi\qu/(\thrjul^2) < T
\end{cases}
\end{align*}
Plugging in Equations~\eqref{eq:LBcombineSteps} and~\eqref{eq:ThetaqIdef} for the definition of functions $\Lambda_{\qu}(N)$ and $ \Theta_{\qi}(k)$ in the above two displays gives the statement of Theorem~\ref{t:joint-L}. 

%
%And if $N\leq 2\qu\log \qu$, 
%
%\begin{align*}
%\Ex\big[\bad(T)\big]
%&\geq C
%\begin{cases} 
%% &\text{if }T \leq \min\{  32\frac{\qi}{\qu}\log\qi,  \frac{N\thrjul^2}{\qi}\}
%%\\
%\sqrt{T\qi N}
%&\text{if } 32\frac{\qi}{\qu}\log\qi < T \leq \frac{N\thrjul^2}{\qi}
%\\
% N \thrjul
%&\text{if }  \frac{N\thrjul^2}{\qi} < T \leq\frac{N^2\thrjul^2}{\qu\qi} 
%\\
%\sqrt{T\qi \qu}
%&\text{if }  \frac{N^2\thrjul^2}{\qu\qi} < T \leq \qi\qu/(\thrjul^2)
%\\
%T \thrjil
%&\text{if }  \qi\qu/(\thrjul^2) < T
%\end{cases}
%\end{align*}
%
%
%
%Hence, 
%\begin{align*}
%\gamma_1 &= \min\Big\{\sqrt{\frac{T\qi \Lambda}{2N}},
% \max\{\sqrt{\frac{T\qi }{2N}} , \frac{T\qi}{4 rN}\}\Big\}\,.
% \\
% & = 
% \begin{cases}
% \sqrt{\frac{T\qi }{2N}}, 
% & \text{ if } T \leq 2\frac{N \thrjul^2}{\qi}
% \\\\
%\frac{T\qi }{2\thrjul N}, 
% & \text{ if } 2\frac{N \thrjul^2}{\qi} < T \leq 2\frac{N \Lambda\thrjul^2}{\qi} 
%  \\\\
%\sqrt{\frac{T\qi \Lambda}{2N}}, 
% & \text{ if }  2\frac{N \Lambda\thrjul^2}{\qi}  < T
% \end{cases}
% \end{align*}
% 
% Case 1 ($ N\geq 2\qu\log\qu$):
% \begin{align*}
%\gamma_1 & = 
%  \begin{cases}
% \sqrt{\frac{T\qi }{2N}}, 
% & \text{ if } T \leq 2\frac{N \thrjul^2}{\qi}
% \\\\
%\frac{T\qi }{2\thrjul N}, 
% & \text{ if } 2\frac{N \thrjul^2}{\qi} < T \leq 8\frac{N^2\thrjul^2}{\qi \qu} 
%  \\\\
%\sqrt{\frac{2T\qi }{\qu}}, 
% & \text{ if }   8\frac{N^2\thrjul^2}{\qi \qu}   < T
% \end{cases}
% \end{align*}
% \begin{align}
%\label{eq:ThetaqIdef}
%\Lambda_{q}(N) := \begin{cases} 
%4N/\qu & \text{ if } \quad N\geq 2\qu\log\qu
%\\
%8\log \qu & \text{ if }\quad 2\qu\log\qu > N \geq \qu\,.
%\end{cases}
%\end{align}
%
%\paragraph{Case I : $\gamma_1\geq\frac{T}{8\log \qi}$:} Alternatively, this condition corresponds to $g(T/(8\log \qi)) \leq f(T/(8\log \qi)) $. If $N\thrjul \leq 4\qi\log\qi$, this corresponds to $T\leq 32\frac{\Lambda}{N}\qi\log\qi $.
%If $N\thrjul > 4\qi\log\qi$, this corresponds to $T\leq 32\frac{\qi}{N}\log\qi $.
%
%\begin{itemize}
%\item $2\qu\log \qu\leq N\leq 4\frac{\qi}{\thrjul} \log\qi$ and $T\leq 32\frac{\Lambda}{N}\qi\log\qi $ (which corresponds to $\gamma_1\geq\frac{T}{8\log \qi}$).
%
%\begin{align*}
%\Ex\big[\bad(T)\big] &\geq 
%\max\Big\{ 
%g(T/(8\log \qi)) ,  T \min\{\thrjil, \frac{\qu}{\thrjil  }\}
%\Big\}
%\end{align*}
%\item $N > 4\qi/\thrjul \log\qi$ and $T\leq 32\frac{\qi}{N}\log\qi $ (which corresponds to $\gamma_1\geq\frac{T}{8\log \qi}$).
%
%\item $N\leq 4\frac{\qi}{\thrjul} \log\qi$ and $T> 32\frac{\Lambda}{N}\qi\log\qi $ (which corresponds to $\gamma_1<\frac{T}{8\log \qi}$).
%\begin{align*}
%\Ex\big[\bad(T)\big]&\geq 
%\max\Big\{ 
%f(\gamma_1),  T \min\{\thrjil, \frac{N}{1+\thrjil \Lambda_{\qu}(N) }\}
%\Big\}
%\\
%&\geq C
%\begin{cases} 
%% &\text{if }T \leq \min\{  32\frac{\qi}{\qu}\log\qi,  \frac{N\thrjul^2}{\qi}\}
%%\\
%\sqrt{T\qi N}
%&\text{if } 32\frac{\qi}{\qu}\log\qi < T \leq \frac{N\thrjul^2}{\qi}
%\\
% N \thrjul
%&\text{if }  \frac{N\thrjul^2}{\qi} < T \leq\frac{N^2\thrjul^2}{\qu\qi} 
%\\
%\sqrt{T\qi \qu}
%&\text{if }  \frac{N^2\thrjul^2}{\qu\qi} < T \leq \qi\qu/(\thrjul^2)
%\\
%T \thrjil
%&\text{if }  \qi\qu/(\thrjul^2) < T
%\end{cases}
%\end{align*}
%
%\item $N > 4\qi/\thrjul \log\qi$ and $T> 32\frac{\qi}{N}\log\qi $ (which corresponds to $\gamma_1<\frac{T}{8\log \qi}$).
%\begin{align*}
%\Ex\big[\bad(T)\big]&\geq 
%\max\Big\{ 
%f(\gamma_1),  T \min\{\thrjil, \frac{N}{1+\thrjil \Lambda_{\qu}(N) }\}
%\Big\}
%\geq 
%\end{align*}
%\end{itemize}











%
%\MK{Am I assuming }
%\subsection{Old stuff}
%\textbf{Part I: ($N\geq 2\qu\log\qu$)} 
%In this regime, using the statement of Lemma~\ref{l:BoundminUserSize}, with probability at least $1/2$, we have $\minUser< 4N/\qu$.
%So,
%with probability at least $1/4$, we have 
%
%\begin{align*}
%\bad(T)
%&\geq 
%\,
%\frac{1}{2}
%\max\Big\{
%n_T,\,
%\frac{\qu \gamma_*^T}{4},\, 
%N\min\{\gamma_*^T,
%\thrjul\},
%T \min\{\thrjil, \frac{\qu}{4\thrjil }\}
%\Big\}
%\end{align*}
%Note that $\max\{\frac{\qu \gamma_*^T}{4},\, 
%N\min\{\gamma_*^T,
%\thrjul\}\}$ is a non-decreasing function of $\gamma_*^T$ and hence bounding $\gamma_*^T> \frac{T}{\Theta_{\qi}(n_T)}$, it is a non-increasing function of $n_T$.
% The first term in above display $n_T$ is clearly an increasing function of $n_T$. So, one can find a lower bound for 
%
%\begin{align*}
%\min_{n_T}\max\Big\{
%n_T,\,
%\frac{\qu \gamma_*^T}{4}
%\Big\}
%&\geq
%\min_{n_T}\max\Big\{
%n_T,\,
%\frac{\qu T}{4\Theta_{\qi}(n_T)}
%\Big\}
%\\
%&\geq
%\begin{cases}
%\frac{\qu }{8}T& 
%\text{ if } 
%T \leq \frac{8\sqrt{\qi}}{3\qu}
%\\\\
%\frac{\qu }{32\log \qi}T& 
%\text{ if } 
% \frac{8\sqrt{\qi}}{3\qu}<T\leq
%64\qi (\log\qi)^2 / \qu
%\\\\
%\frac{\sqrt{T\qi\qu}}{4}
%&\text{ if } 64\qi (\log\qi)^2 / \qu<T
%\end{cases}
%\end{align*} 
%
%
%% 
%% 
%%\begin{align*}
%%\min_{n_T} \max\Big\{
%%n_T,\,
%%N\min\{\gamma_*^T,
%%\thrjul\}
%%\Big\}
%%&\geq
%%\min_{n_T} \max\Big\{
%%n_T,\,
%%N\min\{\frac{T}{\Theta_{\qi}(n_T)},
%%\thrjul\}
%%\Big\} 
%%\\
%%&\geq
%%\begin{cases}
%%\frac{NT}{2}
%%&\text{ if } T\leq \frac{2\sqrt{\qi}}{3N}
%%\text{ and } N\thrjul \geq NT/2
%%\\\\
%%\frac{N }{8\log \qi}T& 
%%\text{ if } 
%%\frac{2\sqrt{\qi}}{3N}< T \leq 16\frac{\qi}{N}(\log \qi)^2
%%\text{ and } N\thrjul \geq \frac{N }{8 \log \qi}T
%%\\\\
%%\sqrt{\frac{T\qi N}{4}}
%%&\text{ if } 
%%16\frac{\qi}{N}(\log \qi)^2 <T
%%\text{ and } N\thrjul \geq \sqrt{\frac{T\qi N}{4}}
%%\\\\
%%N\thrjul 
%%&\text{ otherwise}% N\thrjul <\sqrt{\frac{T\qi N}{4}}
%%\end{cases}
%%%
%%\\
%%%
%%&\geq
%%\begin{cases}
%%\frac{NT}{2}
%%&\text{ if } T\leq \min\{\frac{2\sqrt{\qi}}{3N}, 2\thrjul\}
%%\\\\
%%\frac{N }{8\log \qi}T& 
%%\text{ if } 
%%\frac{2\sqrt{\qi}}{3N}< T \leq \min\{16\frac{\qi}{N}(\log \qi)^2,\, 8 \thrjul\log \qi \}
%%\\\\
%%\sqrt{\frac{T\qi N}{4}}
%%&\text{ if } 
%%16\frac{\qi}{N}(\log \qi)^2 <T \leq \frac{4N\thrjul^2}{\qi}
%%\\\\
%%N\thrjul 
%%&\text{ otherwise}% N\thrjul <\sqrt{\frac{T\qi N}{4}}
%%\end{cases}
%%\end{align*}
%%\MK{The last display is wrong!}
%
%\begin{align*}
%\min_{n_T} \max\Big\{
%n_T,\,
%N\min\{\gamma_*^T,
%\thrjul\}
%\Big\}
%&\geq
%\min_{n_T} \max\Big\{
%n_T,\,
%N\min\{\frac{T}{\Theta_{\qi}(n_T)},
%\thrjul\}
%\Big\} 
%%
%\\
%%
%&\geq
%\min\Big\{N\thrjul,\min_{n_T} \max\big\{
%n_T,\,
%\frac{NT}{\Theta_{\qi}(n_T)}
%\big\} 
%\Big\}
%\\
%\min_{n_T} \max\big\{
%n_T,\,
%\frac{NT}{\Theta_{\qi}(n_T)}
%\big\} 
%&\geq
%\begin{cases}
%\frac{NT}{2} 
%&\text{ if } 
%T \leq  \frac{2\sqrt{\qi}}{3N}
%\\\\
%\frac{NT}{8\log \qi} 
%&\text{ if } 
%\frac{2\sqrt{\qi}}{3N} < T \leq 16\frac{\qi}{N} (\log \qi)^2
%\\\\
%\frac{1}{2}\sqrt{NT\qi}
%&\text{ if } 
%16\frac{\qi}{N} (\log \qi)^2< T\,.
%\end{cases}
%\end{align*}
%
%So, overall, there are three possible cases:
%
%\textbf{Case I:} $N\thrjul \leq \sqrt{\qi}/3$
%
%\begin{align*}
%\bad(T)
%&\geq
%\begin{cases}
%\frac{NT}{2} 
%&\text{ if } 
%T \leq  2\thrjul\,,
%\\\\
%N\thrjul
%&\text{ if } 
%2\thrjul <T\leq 
%8\frac{N}{\qu}\thrjul
%\\\\
%\frac{\qu T}{8}
%&\text{ if } 
%8\frac{N}{\qu}\thrjul<T\leq\frac{8\sqrt{\qi}}{3\qu}\,,
%\\\\
%\frac{\qu T}{32\log \qi} 
%&\text{ if } 
%\frac{8\sqrt{\qi}}{3\qu}<T\leq 64\qi (\log\qi)^2 / \qu\,,
%\\\\
%\frac{\sqrt{T\qi\qu}}{4}
%&\text{ if } 64\qi (\log\qi)^2 / \qu<T
%\end{cases}
%\end{align*}
%
%
%\textbf{Case II:} $\sqrt{\qi}/3 < N\thrjul  \leq 2\qi \log\qi$
%
%
%\begin{align*}
%\bad(T)
%&\geq
%\begin{cases}
%\frac{NT}{2} 
%&\text{ if } 
%T \leq  2\thrjul\,,
%\\\\
%\frac{NT}{8\log \qi} 
%&\text{ if } 
%\frac{2\sqrt{\qi}}{3N} < T \leq 8 \thrjul \log \qi
%\\\\
%N\thrjul
%&\text{ if } 
%8 \thrjul \log \qi <T\leq 32\frac{N}{\qu}  \thrjul \log\qi\,,
%\\\\
%\frac{\qu T}{32\log \qi} 
%&\text{ if } 
%32\frac{N}{\qu} \thrjul \log\qi <T\leq 64 N \thrjul \log\qi\frac{32}{\qu}\,,
%\\\\
%\frac{\sqrt{T\qi\qu}}{4}
%&\text{ if } 64\qi (\log\qi)^2 / \qu<T
%\end{cases}
%\end{align*}
%
%
%\textbf{Case III:} $2\qi \log\qi< N\thrjul  $
%
%\begin{align*}
%\bad(T)
%&\geq
%\begin{cases}
%\frac{NT}{2} 
%&\text{ if } 
%T \leq  \frac{2\sqrt{\qi}}{3N}
%\\\\
%\frac{NT}{8\log \qi} 
%&\text{ if } 
%\frac{2\sqrt{\qi}}{3N} < T \leq 16\frac{\qi}{N} (\log \qi)^2
%\\\\
%\frac{1}{2}\sqrt{NT\qi}
%&\text{ if } 
%16\frac{\qi}{N} (\log \qi)^2< T \leq 4\frac{N}{\qi} \thrjul^2
%\\\\
%N\thrjul&\text{ if } 
%4\frac{N}{\qi} \thrjul^2 <T \leq 16\frac{N^2 }{\qi \qu} \thrjul^2
%\\\\
%\frac{\sqrt{T\qi\qu}}{4}&\text{ if } 
% 16\frac{N^2 }{\qi \qu} \thrjul^2 <T
%\end{cases}
%\end{align*}
%
%
%\textbf{Part II: ($N\leq 2\qu\log\qu$)} 

==> prooftheoremLowerBd.tex <==
\subsection{Bad recommendations}
\subsubsection{Regular matrices}
\MK{Done with this subsec.}
The  regularity properties  of the preference matrix, defined below,  allow us to control the posterior probability for an item being liked by a user. 
Roughly speaking, matrix $A$ is column regular when every submatrix constructed by a small subset of columns of $A$ are similar to a matrix with independent uniform elements (each realization of rows of this tall submatrix are almost equally frequent). 
This attribute of the preference matrix quantifies the number of item types which should be recommended to user $u$ to gather enough information about the structure in user space in order to predict the preference of  user $u$ for a new item type $\ti$. 


To elucidate this connection, assume that the preference matrix is column regular. Also assume that $u$ has not rated any item with item type $\ti$ yet. 
Hence, if  $u$ has rated only a few distinct item types, then the columns of matrix $\Xi$ corresponding to the item types previously recommended to user $u$ in addition to the column corresponding to item type $\ti$ is similar to a matrix with independent uniform elements. 
 The historical data implies that the type of  user $u$ is uniform on all the user types consistent with the feedback of past recommendations to $u$.
Therefore,  roughly half of the user types consistent with the historical data of  $u$ like item type $\ti$ and half of them dislike item type $\ti$.
This shows that  $u$ likes or dislikes item type $\ti$ with probability roughly half given historical data. 
We give the details of this argument in the proof of Lemma~\ref{cl:jl-bdA3} in Section~\ref{sec:Pfjl-bdA3}.
Similar heuristics shows that the row-regularity of preference matrix quantifies the number of user types which should be recommended item $i$ to gather enough information about the structure in item space to predict the preference of a new user type $\tu$ for item $i$. 
%
\begin{definition}[$(r,\eta)$-column regularity]\label{def:ul-reg}
	Fix $s$ and $\eta$. Let $A\in \{-1,+1\}^{m \times n}$ and $A_{\cdot j}$ be the $j$th column of $A$. 
	For ordered tuple of distinct (column) indices $w=(j_1,\dots,j_s)\in [n]^s$, let $M=(A_{\cdot j})_{j\in w}\in  \{-1,+1\}^{m \times s}$ be the matrix formed from the columns of $A$ indexed by $w$.
	For given row vector $b\in\{-1,+1\}^s$, let $K_{b,w}(A)\subseteq [m]$ be the  indices of rows in $M$ that are identical to the row $b$. The cardinality of $K_{b,w}(A)$ is denoted by $k_{b,w}(A)$. 
Matrix $A$ is said to be \emph{$(s,\eta)$-column regular} if 
	\[\max_{b,w}\Big|k_{b,w}(A)-\frac{m}{2^{s}}\Big| \leq \eta \frac{m}{2^{s}}\,,\]
	where the maximum is over tuples $w$ of $s$ columns and $\pm 1$ vectors $b$ of size $s$.

	We define $\rgl_{s,\eta}$ to be the set of $(s,\eta)$-column regular matrices. We also define $\Omega_{0,\eta}$ such that $A\in \rgl_{0,\eta}$ for all $A\in \{-1,+1\}^{m \times n}$.
\end{definition}
%\MK{I defined $\rgl_{0,\eta}$}

\begin{definition}[$(s,\eta)$-row regularity]\label{def:row-reg}
The matrix $A\in\{-1,+1\}^{n\times m}$ is said to be $(s,\eta)$-\textit{row regular} if its transpose is $(s,\eta)$-column regular. We write $A^\top \in \rgl_{s,\eta}$,  where $\rgl_{s,\eta}$ is the set of $(s,\eta)$-column regular matrices.
\end{definition}

\begin{claim}\label{cl:ul-smalltregular}If a matrix $A\in\{-1,+1\}^{m\times n}$ is \emph{$(s,\eta)$-column regular}, then it is also \emph{$(s',\eta)$-column regular} for all $s'<s$.\end{claim}
\begin{proof}
Suppose that $A$ is $(s,\eta)$-column regular. By induction it suffices to show that $A$ is $(s-1,\eta)$-column regular. We will check that 
$(1-\eta)\frac{m}{2^{s-1}}\leq k_{b,w}(A) \leq (1+\eta)\frac{m}{2^{s-1}}$ for all size $s-1$ tuples $w$ and vectors $b$. 
For any given $w\in[n]^{s-1}$ and $b\in\{-1,+1\}^{s-1}$, let  $b^+ = [b \, \, 1]\in \{-1,+1\}^{s}$ be obtained from $b$ by appending $+1$. Similarly $b^-$ is obtained from $b$ by appending $-1$. If $w'=(w,\ti)\in[n]^s$ for any $\ti\notin w$, then $K_{b,w}=K_{b^+,w'}\cup K_{b^-,w'}$ and $K_{b^+,w'}\cap K_{b^-,w'}=\varnothing$, so
 $k_{b,w}=k_{b^+,w'}+k_{b^-,w'}$. Since $A$ is $(s,\eta)$-column regular, $(1-\eta)\frac{m}{2^s}\leq k_{b^+,w'},k_{b-,w'} \leq (1+\eta)\frac{m}{2^s}$, hence $(1-\eta)\frac{m}{2^{s-1}}\leq k_{b,w} \leq (1+\eta)\frac{m}{2^{s-1}}$. 
\end{proof}


\begin{lemma}\label{l:ul-regularity}
	Let matrix $A\in\{-1,+1\}^{m \times n}$ have independent uniformly distributed entries on $\{-1,+1\}$. 
	If $\eta<1$, then $A$ is $(s,\eta)$-column regular ($A\in\Omega_{s,\eta}$)  with probability at least $$1-2(2n)^s \exp\left( - \frac{\eta^2}{3}\frac{m}{2^{s}}\right)\,.$$
\end{lemma}
\begin{proof}
For given column tuple $w$ and row vector $b$, the expected number of times the row vector  $b$ appears is $\frac{m}{2^s}$. 
For any given vector of $b$ and $w$, an application of Chernoff bound (Lemma \ref{l:Chernoff}) with $\eta<1$ implies
%
\[\Pr\Big[\big|k_{b,w}(A)-\frac{m}{2^{s}}\big| \geq \eta\frac{m}{2^{s}}\Big] \leq 2 \exp\left( - \frac{\eta^2}{3}\frac{m}{2^{s}}\right)\,.\]
There are no more than $n^s$ possible choices of column tuple $w$, and $2^s$ possible choices of row vector $b$; 
the union bound yields the proof.
\end{proof}

The  proof of the following lemma is similar to the proof of Lemma~\ref{l:ul-regularity}.
\begin{lemma}\label{l:IL-reg-prob}
	Let matrix $A\in\{-1,+1\}^{n\times m}$ have independent uniformly distributed entries on $\{-1,+1\}$.
	 If $\eta<1$, then the matrix $A$ is $(s,\eta)$-row regular, $A^T\in\Omega_{s,\eta}$, with probability at least 
	 $$1-2(2n)^s  \exp\left( - \frac{\eta^2}{3}\frac{m}{2^{s}}\right)\,.$$
\end{lemma}


%%%%%%%%%%%%
%%%%%%%%%%%%5
\subsubsection{Regularity of the preference matrix} \MK{Done with this subsec.}
Throughout this section, we will fix the following parameters.
In Lemma~\ref{cor:regularityprob} we will show that with this choice of parameters the preference matrix is both $(\thrjul,\eta)$-column regular and $(\thrjil,\eta)$-row regular.
\begin{align}\label{eq:jl-thru}
 \thrjul & :=\big\lfloor\log \qu - \log\log \qi -4\log\log N-2\big\rfloor_{+}\,,
\\
\thrjil & :=\big\lfloor 0.99 \log \qi - 5\log\log N - 2\big\rfloor_{+}\,,
\label{eq:jl-thri}
\\
\text{and}\quad 
\eta & :=\frac{1}{\log N}\,.
\label{eq:jl-etaDef}
\end{align}
\MK{add $\big\rfloor_{+}$ in the notation section }
We will use the property $\eta<1/4$ in the proof which is derived by the assumption $N>100$.
\paragraph{Significance of $\thrjil$ and $\thrjul$.}
Roughly speaking, when the preference matrix is row-regular, $\Xi^T \in \Omega_{\thrjil,\eta}$ (or column regular $\Xi \in \Omega_{\thrjul,\eta}$) the parameters $\thrjil$ (and $\thrjul$) quantify a lower bound on the cost of learning the structure in user space (and item space) per user (and per item) respectively.
Note that these parameters can be equal to zero depending on the regime of model parameters $\qi,\qu$, and $N$. 
Heuristically speaking, when $\thrjul=0$, the cost of learning the structure in user space is lower bounded trivially by zero. So the proof is based on the performance limits of an algorithm which has access to the user types of all users and the lower bound is based on the cost of exploring the item space. 
Alternatively, when $\thrjil=0$, the cost of learning the structure in item space is lower bounded trivially by zero. So the proof is based on the performance limits of an algorithm which has access to the item types of all items in this case.

%\MK{Think about this. What does it mean when one of them is zero. I think the lower bound might become trivially equal to zero when $\thrjil=0$. Think about it. }
The next corollary is an implication of Lemmas~\ref{l:ul-regularity} and~\ref{l:IL-reg-prob}.

\begin{lemma}
\label{cor:regularityprob}
With the choice of parameters in~\eqref{eq:jl-thru},~\eqref{eq:jl-thri} and~\eqref{eq:jl-etaDef}, the preference matrix is both $(\thrjul,\eta)$-column regular and $(\thrjil,\eta)$-row regular, \textit{i.e.}, 
$\Xi\in \Omega_{\thrjul,\eta}$ 
and 
$\Xi^T\in \Omega_{\thrjil,\eta}$,
 with probability at least $1-1/N$. 
\end{lemma} 


\begin{proof}
This corollary is derived by plugging in  the choice of parameters  $\thrjul$ and $\thrjil$ in Lemmas~\ref{l:ul-regularity} and~\ref{l:IL-reg-prob}.
\begin{align*}
\log \frac{1}{2}\Pr[\Xi\notin \Omega_{\thrjul,\eta}]
&\overset{(a)}{\leq}
{\thrjul} \log(2\qi)
 - \frac{\eta^2}{3}\frac{\qu}{2^{\thrjul}}
\overset{(b)}{\leq}
{\thrjul} \log(2\qi)- (\log N)^2 \log \qi
 \\
&\overset{(c)}{\leq}
\Big[ \log(2\qi)-  (\log N) (\log \qi)\Big]
\log N
\overset{(d)}{\leq}
-2 \log N\,,
\end{align*}
where (a) uses Lemma~\ref{l:ul-regularity}. (b) uses the definition of $\thrjul$ and $\eta$ in~\eqref{eq:jl-thru} and~\eqref{eq:jl-etaDef}. (c) uses the assumption $\qu\leq N$ and $\thrjul\leq \log N$. (d) holds since $N\geq 100$.
\begin{align*}
\log \frac{1}{2}\Pr[\Xi^T\notin \Omega_{\thrjil,\eta}]
&\overset{(a)}{\leq}
{\thrjil} \log(2\qu)
 - \frac{\eta^2}{3}\frac{\qi}{2^{\thrjil}}
\overset{(b)}{\leq}
% {\thrjil} \log (2N)- (\log N)^3\qi^{.01}
% \\
% &\overset{(c)}{\leq}
\Big[ .99(1+\frac{1}{\log N})\log \qi  
 - (\log N)^2\qi^{.01}\Big]\log N
\\& \overset{(c)}{\leq}
\Big[1.16\log \qi  
 - 44\qi^{.01}\Big]\log N
\overset{(d)}{\leq}
 -2 \log N\,,
\end{align*}
where (a) uses Lemma~\ref{l:IL-reg-prob}. (b) uses the definition of $\thrjil$ and $\eta$ in~\eqref{eq:jl-thri} and~\eqref{eq:jl-etaDef}. (c) uses $N\geq 100$ and (d) holds for any $\qi>1$. 

Hence, $\Pr[\Xi\in \Omega_{\thrjul,\eta},\,\Xi^T\in \Omega_{\thrjil,\eta}]\geq 1-4/N^2 >1-1/N$.
\end{proof}




\subsubsection{Parameters summarizing the history}
\label{sec:LBthrParam}
\MK{Done with this subsec.}

To describe the features of the historical data seen by the algorithm so far (the feedback taken from past recommendations), we will introduce several new notations. 
Later on, these notations will help us characterize and define the notion of `bad' recommendations in Equation~\eqref{eq:jl-def-bad}. 
\begin{definition}\label{def:jl-cit}
Let $c_i^t$ be the number of user types which have rated item $i$ by time $t-1$:
\begin{align*}
c_i^t &:= 
%\Big|\big\{ \tu\in[\qu]: \text{there exists user } u\in[N\text{ with  type } \tau_U(u)=\tu,\, 
%\\
%&\quad \quad \quad\quad \text{ s.t. }\, a_{u,s}=i \text{for some } s<t \big\}\Big|
%\\
%&=
\sum_{\tu=1}^{\qu}
\ident\Big[\sum_{u:\tau_U(u)=\tu}\sum_{s=1}^{t-1}\ident[a_{u,s}=i]>0
\Big]\,.
\end{align*}
\end{definition}
Since $c_i^t$ is nondecreasing in $t$, for any $t\leq T$,
\begin{equation}
\ident[c_i^t \geq \thrjil]
 \leq 
 \ident[c_i^T \geq \thrjil]\,.
\end{equation}


\begin{definition}\label{def:jl-dut}
Let $d_u^t$ be the number of distinct item types that were rated by user $u$ up to time $t-1\,:$
\begin{align*}
d_u^t &:=
% |\{\ti\in[\qi]:  \text{there exists item } i\in\mathbb{N} %\text{with item type } \tau_I(i)=\ti,\,\text{ s.t. }\,  a_{u,s}=i %\text{ for some } s<t \}|\\
%& = 
\sum_{\ti=1}^{\qi}\ident\Big[\sum_{i:\tau_I(i)=\ti}\sum_{s=1}^{t-1}\ident[a_{u,s}=i]>0\Big]
\,. 
\end{align*}
\end{definition}
Since $d_u^t$ is nondecreasing in $t$, for any $t\leq T$,
\begin{equation}
\ident\big[d_u^t \geq \thrjul] \leq \ident[d_u^T \geq \thrjul\big]\,.
\end{equation}


%%%%%
%%%%%
%%%%%
%%%%%
\subsubsection{Characterization of bad recommendations}
\paragraph{Unknown item type and user type.}
Intuitively speaking, when the type of item $i$ and user $u$ are both unknown, recommending $i$ to $u$ is a bad recommendation. 
To formalize this, the following lemma shows that if $c_i^t$ and $d_u^t$ are small and the preference matrix is both row and column-regular, then the outcome of recommending item $i$ to user $u$ at time $t$ is uncertain.
\begin{lemma}\label{cl:jl-bdA1}
For any user $u\in[N],$ and item $i\in\mathbb{N}$, 
\begin{align*}
\Pr
\Big[ 
L_{u,i}=+1 \,\big|\,& a_{u,t}=i,\, c_i^t <\thrjil, \,d_u^t <\thrjul,\, \Xi^T \in \rgl_{\thrjil,\eta}\,, \,\Xi \in \rgl_{\thrjul,\eta}
\Big]
%\\& 
\leq \frac{1+4\eta}{2}\,.
\end{align*}
\end{lemma}

This lemma is proved in Section~\ref{sec:Pfjl-bdA1}.
Multiplying the statement of Lemma~\ref{cl:jl-bdA1}  by $\Pr[ a_{u,t}=i, c_i^t <\thrjil, d_u^t <\thrjul, \Xi^T \in \rgl_{\thrjil,\eta} \,,\Xi \in \rgl_{\thrjul,\eta}]$ and taking summation over $i$ gives 
\begin{align}
\Asf{1} 
&:= 
\Pr\Big[L_{u,a_{u,t}}=+1, c_{a_{u,t}}^t < \thrjil, d_{u}^t < \thrjul,  \Xi^T \in \rgl_{\thrjil,\eta} \,,\Xi \in \rgl_{\thrjul,\eta}\Big]\notag\\
 &\,\,
 \leq \frac{1+4\eta}{2}\,\,
 \Pr\Big[c_{a_{u,t}}^t < \thrjil, d_{u}^t < \thrjul,  \Xi^T \in \rgl_{\thrjil,\eta} \,,\Xi \in \rgl_{\thrjul,\eta}\Big]
 \,.  \label{cor:jl-bdA1}
\end{align}


%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\paragraph{Unknown item type.}
 When the type of user $u$ is known, but the type of item $i$ is unknown, if item  $i$ has not been recommended to any user with the same type as $u$ before, then recommending $i$ to $u$ is a `bad' recommendation. To formalize this, we use the following definition. 
 
 
\begin{definition} \label{def:jl-B-tauU-i} Let $\BBjul{u}{i}{t}$ be  the event that a user with type $\tau_U(u)$ has rated item $i$ by  the end of time $t-1$, i.e.,
\[\BBjul{u}{i}{t} =
 \Big\{{\text{there exists } u'\in[N]: a_{u',s}=i} \text{ for some } s< t \text{ with } \tau_U(u) = \tau_U(u')\Big\}
 \,.\]
\end{definition}



The following lemma shows that if $c_i^t$ is small, the preference matrix is row-regular and no user with type $\tau_U(u)$ has rated $i$ before, then the outcome of recommending item $i$ to user $u$ at time $t$ is uncertain.
\begin{lemma}\label{cl:jl-bdA2}
For any user $u\in[N],$ and any item $i\in\mathbb{N}$, 
\begin{align*}
\Pr
\big[L_{u,i}=+1& \,\big|\, a_{u,t}=i, \,c_i^t <\thrjil,\, d_u^t \geq\thrjul, \,
\big(\BBjul{u}{i}{t}\big)^c,
\, \Xi^T \in \rgl_{\thrjil,\eta}
\big] 
%\\&\,\,
\leq \frac{1+4\eta}{2}\,.
\end{align*}
\end{lemma}
This lemma is proved in Section~\ref{sec:Pfjl-bdA2}.
Multiplying the statement of Lemma~\ref{cl:jl-bdA2} by 
$\Pr\big[ a_{u,t}=i, c_i^t <\thrjil, d_u^t \geq\thrjul, (\BBjul{u}{i}{t})^c, \Xi^T \in \rgl_{\thrjil,\eta}\big]$ 
and summing over $i$ gives
\begin{align}
\Asf{2} :=  
&\Pr\big[L_{u,a_{u,t}}=+1, c_{a_{u,t}}^t < \thrjil, d_{u}^t \geq \thrjul, (\BBjul{u}{a_{u,t}}{t})^c, \Xi^T \in \rgl_{\thrjil,\eta} \big]
\notag\\
 &\hspace{-.1in}\leq 
 \frac{1+4\eta}{2}\,\,\Pr\big[c_{a_{u,t}}^t < \thrjil, d_{u}^t \geq \thrjul, (\BBjul{u}{a_{u,t}}{t})^c, \Xi^T \in \rgl_{\thrjil,\eta} \big]\,.\label{cor:jl-bdA2}
\end{align}

%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\paragraph{Unknown user type.}
When the type of item $i$ is known, but the type of user $u$ is unknown, if user $u$ has not been recommended any item with the same type as $i$ before, then recommending $i$ to $u$ is a `bad' recommendation. To formalize this, we use the following definition. 


\begin{definition} 
%\label{def:jl-B-u-tauI} 
Let $\BBjil{u}{i}{t}$ be  the event that user $u$ has rated an item of the same item type as item $i$ by time $t-1$, i.e.,
\[\BBjil{u}{i}{t} 
= \Big\{
{\text{there exists } i'\in\mathbb{N}: a_{u,s}=i'} \text{ for some } s< t \text{ with } \tau_I(i) = \tau_I(i')
\Big\}
\,.\]
\end{definition}


The following lemma shows that if $d_u^t$ is small, the preference matrix is column-regular and user $u$ has not rated any item of type $\tau_I(i)$, then the outcome of recommending item $i$ to user $u$ at time $t$ is uncertain.
\begin{lemma}\label{cl:jl-bdA3}
 For any user $u\in[N],$ and any  item $i\in\mathbb{N}$, 
\begin{align*}
\Pr
\big[ L_{u,i}=+1& \,\big|\, 
a_{u,t}=i, \,
c_i^t \geq\thrjil,
\, d_u^t <\thrjul,\,
 (\BBjil{u}{i}{t})^c, \,
 \Xi \in \rgl_{\thrjul,\eta}
\big] 
%\\&
\leq \frac{1+4\eta}{2}\,.
\end{align*}
\end{lemma}
This lemma is proved in Section~\ref{sec:Pfjl-bdA3}.
Multiplying the statement of Lemma~\ref{cl:jl-bdA3} by 
$\Pr[ a_{u,t}=i, c_i^t \geq\thrjil, d_u^t <\thrjul, (\BBjil{u}{i}{t})^c, \Xi \in \rgl_{\thrjul,\eta}]$ and summing over $i$ gives
\begin{align}
\Asf{3} 
 & := 
\Pr\big[
L_{u,a_{u,t}}=+1, c_{a_{u,t}}^t \geq\thrjil, d_u^t <\thrjul, (\BBjil{u}{a_{u,t}}{t})^c, \Xi \in \rgl_{\thrjul,\eta}
\big]
\notag\\
&
 \leq 
 \frac{1+4\eta}{2}\,\, \Pr[c_{a_{u,t}}^t \geq\thrjil, d_u^t <\thrjul, (\BBjil{u}{a_{u,t}}{t})^c, \Xi \in \rgl_{\thrjul,\eta}]\,.\label{cor:jl-bdA3}
\end{align}

%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\paragraph{Unknown preference of user type for item type.}
When  the type of item $i$ and  the type of user $u$ are both known, 
 if no user with the same type as $u$ has been recommended any item with the same type as $i$  before, 
 then recommending $i$ to $u$ is a `bad' recommendation. To formalize this, we use the following definition. 
\begin{definition} \label{def:jl-B-tauU-tauI} Let $\BBjjl{u}{i}{t}$ be  the event that a user with type $\tau_U(u)$ has rated an item with type $\tau_I(i)$ by time $t-1$, i.e.,
\begin{align*}
\BBjjl{u}{i}{t} = \Big\{&{\text{there exists } i'\in\mathbb{N}, u'\in[N]: a_{u',s}=i'} 
%\\&
\text{ for some } s< t \text{ with } \tau_I(i') = \tau_I(i), \tau_U(u')=\tau_U(u)
\Big\}\,.
\end{align*}
\end{definition}
The following lemma shows that if no user of type $\tau_U(u)$ has rated any item of type $\tau_I(i)$, then the outcome of recommending item $i$ to user $u$ at time $t$ is uncertain.
\begin{lemma}\label{cl:jl-bdA4}
 For any user $u\in[N],$ and any item $i\in\mathbb{N}$, 
\[
\Pr\big[L_{u,i}=+1 | a_{u,t}=i, c_i^t \geq\thrjil, d_u^t \geq\thrjul, (\BBjjl{u}{i}{t})^c\big] = \frac{1}{2}\]
\end{lemma}
This lemma is proved in Section~\ref{sec:Pfjl-bdA4}.
Multiplying the statement of Lemma~\ref{cl:jl-bdA4}  by $\Pr[ a_{u,t}=i, c_i^t \geq\thrjil, d_u^t \geq\thrjul, (\BBjjl{u}{i}{t})^c]$ and summing over $i$ gives
\begin{align}
\Asf{4} &:=
 \Pr[L_{u,a_{u,t}}=+1, c_{a_{u,t}}^t \geq\thrjil, d_{u}^t \geq \thrjul, (\BBjjl{u}{a_{u,t}}{t})^c ]
 \notag\\&
  = \frac{1}{2}\,\Pr[c_{a_{u,t}}^t \geq\thrjil, d_{u}^t \geq \thrjul, (\BBjjl{u}{a_{u,t}}{t})^c ]\,.\label{cor:jl-bdA4}
\end{align}
%%%%%%%%%%%%%
%%%%%%%%%%%%%
%%%%%%%%%%%%%
%%%%%%%%%%%%%
\paragraph{Definition of bad recommendations.}
Define
\begin{align}
\Bsf{1}(u,t) &:=\ident[c_{a_{u,t}}^t < \thrjil, d_{u}^t < \thrjul]\,,\label{eq:jl-def-B1}\\
\Bsf{2}(u,t) &:=\ident[c_{a_{u,t}}^t < \thrjil, d_{u}^t \geq \thrjul, (\BBjul{u}{
a_{u,t}}{t})^c]\,,\label{eq:jl-def-B2}\\
\Bsf{3}(u,t) &:=\ident[c_{a_{u,t}}^t \geq \thrjil, d_{u}^t < \thrjul, (\BBjil{u}{a_{u,t}}{t})^c]\,,\label{eq:jl-def-B3}\\
\Bsf{4}(u,t) &:= \ident[c_{a_{u,t}}^t \geq\thrjil, d_{u}^t \geq \thrjul, (\BBjjl{u}{a_{u,t}}{t})^c]\,.\label{eq:jl-def-B4}
\end{align}
Next, define the set of bad recommendations up until time $T$ to be:
\begin{align}\label{eq:jl-def-bad}
\bad(T)& := \sum_{t=1}^T \sum_{u=1}^N \Bsf{1}(u,t)+\Bsf{2}(u,t)+\Bsf{3}(u,t)+\Bsf{4}(u,t) \,.
\end{align}


% \paragraph{Regret in terms of number of bad recommendations:}
% \begin{lemma}\label{l:jl-reg-lower}
% For the set of bad recommendations defined in Equation~\eqref{eq:jl-def-bad}, the following lower bound for regret holds:
% \[\reg(T)\geq  \frac{1-4\eta}{2N}\,\Exp{\bad(T)}- \frac{1}{N}T\,.\]
% \end{lemma}
% This lemma is proved in Section~\ref{sec:proof-lowerBD-regret}.
% Theorem~\ref{t:joint-L} is a direct consequence of Lemmas~\ref{l:jl-reg-lower} and~\ref{l:jl-bad-lower}.  


